Membrane: Accelerating Database Analytics with Bank-Level DRAM-PIM Filtering

In-memory database query processing frequently involves substantial data transfers between the CPU and memory, leading to inefficiencies due to Von Neumann bottleneck. Processing-in-Memory (PIM) architectures offer a viable solution to alleviate this bottleneck. In our study, we employ a commonly used software approach that streamlines JOIN operations into simpler selection or filtering tasks using pre-join denormalization which makes query processing workload more amenable to PIM acceleration. This research explores DRAM design landscape to evaluate how effectively these filtering tasks can be efficiently executed across DRAM hierarchy and their effect on overall application speedup. We also find that operations such as aggregates are more suitably executed on the CPU rather than PIM. Thus, we propose a cooperative query processing framework that capitalizes on both CPU and PIM strengths, where (i) the DRAM-based PIM block, with its massive parallelism, supports scan operations while (ii) CPU, with its flexible architecture, supports the rest of query execution. This allows us to utilize both PIM and CPU where appropriate and prevent dramatic changes to the overall system architecture. With these minimal modifications, our methodology enables us to faithfully perform end-to-end performance evaluations using established analytics benchmarks such as TPCH and star-schema benchmark (SSB). Our findings show that this novel mapping approach improves performance, delivering a 5.92x/6.5x speedup compared to a traditional schema and 3.03-4.05x speedup compared to a denormalized schema with 9-17% memory overhead, depending on the degree of partial denormalization. Further, we provide insights into query selectivity, memory overheads, and software optimizations in the context of PIM-based filtering, which better explain the behavior and performance of these systems across the benchmarks.

==> Membrane/Sections/Abstract.tex <==
%% This is the old abstract

%\ks{Hasn't been updated since HPCA. Needs to be rewritten to reflect new story!} \textbf{ This paper explores application of processing-in-memory (PIM) techniques to Online Analytical Processing (OLAP) database workloads. }
%\textbf{We explore how to map queries onto subarray-level PIM, which enables parallelism across subarrays and banks. We systematically explore mapping strategies and trade-offs between bit-serial \/ element-parallel and bit-parallel/element-serial designs adapted from the prior Sieve and Fulcrum architectures, respectively. We find that join operations do not map well to subarray-level PIM architectures, and thus we need to use a software pre-join denormalization method to transform join operations to selection/filter operations. We also learn that certain operations, such as aggregation, remain better served using the CPU. Thus, we propose a cooperative approach for analytic query processing between  CPU and PIM. We then explore several dimensions in the design space of PIM architectures, including different ways to perform filter operations, and a new way to return data to the CPU. We conclude that a traditional columnar-database layout with a scalar processing element in the PIM-enabled subarrays (Membrane-H) for the table scan, combined with a rank-level unit (RLU) for gathering the selected elements, is the best configuration. An evaluation of an end-to-end query processing on the popular analytic benchmark SSB at scale factor 100 (a 60GB database) yields a 45.39$\times$ geometric-mean speedup over a hand-optimized AVX-512 implementation of SSB.}


%% New abstract

%\textbf{Query processing in in-memory databases often entails significant data transfers between the CPU and memory, which leads to inefficiencies due to the Von Neumann bottleneck. Processing-in-Memory (PIM) architectures present a promising solution to mitigate this bottleneck. However, DRAM-based PIM systems face limitations, such as the inability to support large caches or complex arithmetic logic units (ALUs), due to prioritizing DRAM capacity. However, query processing typically benefits from having large caches for operations like JOINs and aggregates. In our research, we adopt a software-based database strategy that simplifies JOIN operations into a sequence of selection or filtering tasks through pre-join denormalization. This study investigates the DRAM design spectrum to assess the effectiveness of executing these filtering tasks at different DRAM levels. Our findings also conclude that certain tasks, particularly aggregates, are more efficiently performed on the CPU. Consequently, we suggest a collaborative query processing model that leverages both the CPU and PiM, offering dual advantages: it minimizes area demands on DRAM without compromising capacity significantly and also, utilizes both CPU and PIM resources for query processing without necessitating significant alterations to the existing system architecture. By implementing minimal modifications, our approach allows for faithful estimation of end-to-end performance analysis using well-established analytics benchmarks like TPCH and the star-schema benchmark (SSB). Our results reveal that this innovative mapping technique significantly enhances performance, achieving a ABC/DEF/GHI (min/max/geomean) speedup while only imposing a MN/OP memory overhead from denormalization. Additionally, we demonstrate that software modifications to database engines can further amplify these performance gains when tailored for PIM-assisted query execution.}

% \ks{Need to update. Also, why is this bold - is this part of the template?}
% \textbf{For in-memory databases, the extensive data movement between the CPU and memory during query processing poses a significant challenge, exacerbating the limitations imposed by the Von Neumann bottleneck and adversely impacting the performance of database systems. To circumvent these constraints, DRAM-based Processing-In-Memory (PIM) architectures have been advocated, aiming to minimize costly data movements by integrating compute elements close to data storage. Nevertheless, the implementation of such PIM architectures necessitates a careful balance between the area overhead of compute elements and the preservation of DRAM storage capacity. This paper introduces Membrane, a novel PIM architecture designed to embed lightweight compute elements within DRAM specifically for enhancing scan operation efficiency in query processing. Given the widespread adoption of database denormalization to enhance performance—characterized by tables with an expanded number of columns to reduce JOIN operations and increase scan efficiency—Membrane leverages the substantial parallelism and bandwidth inherent in DRAM to significantly accelerate scan operations on these denormalized databases, thereby boosting overall workload performance.}

% \textbf{Contrary to strategies that fully offload workloads to PIM, our approach advocates for a cooperative processing paradigm between PIM and the host CPU, strategically distributing portions of the query execution pipeline to exploit the unique advantages of each architecture. Through an extensive exploration of the design space across multiple dimensions, including PIM logic placement (hardware-side) and variations in database sizes and schemas (software-side), we aim to identify an optimal PIM architecture. This architecture is characterized by minimal modifications to the existing system architecture, significant end-to-end application speedup, and minimal PIM area overhead within DRAM. Our co-design of hardware and software for query processing on denormalized databases concludes that Membrane's PIM architecture not only achieves considerable end-to-end speedup (represented by max/min/geomean rates of ABC/DEF/GHI) but also maintains a PIM logic overhead of XY at the DRAM bank level, demonstrating a viable solution to the longstanding challenge of data movement in in-memory database systems.}

% Query processing in in-memory databases often entails significant data transfers between the CPU and memory, which leads to inefficiencies due to the Von Neumann bottleneck. Processing-in-Memory (PIM) architectures present a promising solution to mitigate this bottleneck by placing compute elements on the side of the memory bus. In this work, we explore Membrane family of PIM architectures that tailored to the needs of analytics query processing workloads. Rather than offloading the entire query processing to PIM components, we advocate for a cooperative processing between PIM and CPU to execute portions of the workloads which can take advtanage of each others architectural strengths.  Since, in-memory analytics databases tend to run on DDR-based main memory, we conduct a design space exploration on the DRAM side and analyze the kernels on the application side to propose a low area overhead design that offers a good performance improvement without dramatically altering the main memory. 

% In order to make the workload more PIM-amenable, we propose

%We've analyzed query processing parts that benefit from PIM acceleration and found the filter kernel most suitable. We've explored DRAM design to determine the best place to execute filter operations. Our goal is to achieve a lower area overhead and a larger holistic effect on the end-to-end speedup, not solely on the kernel speedup. We've also proposed denormalization, a software technique to make databases more PIM-friendly. However, denormalization comes with a larger memory overhead, so we suggest different levels to balance performance and memory overhead. 

%Our evaluations show that Membrane, our PIM system, achieves a speedup of A/B/C compared to a host running a normalized schema and D/E/F against the same host running a denormalized schema. Our light-weight filtering elements have an area overhead of XYZ. We also suggest software-hardware co-optimizations to the database engine to unlock more performance when PIM-capable hardware is detected. Additionally, we provide insights on query selectivity, data size, and schema denormalization's impact on system performance.

Database analytics workloads  process large volumes of data and are typically memory-bound. In fact, in typical queries, the filtering step (aka, table scan) selects only a small subset of records; most records do not meet the query predicate(s) and are not used further, and we find that filtering, combined with pre-joining or denormalizing the database schema, is an excellent candidate for near-data or processing-in-memory (PIM) architectures that place compute elements on the other side of the memory bus. This work develops a bank-level PIM architecture that makes only minor changes to main memory and achieves substantial end-to-end query speedup in DuckDB, with negligible area overhead.  However, because denormalization techniques can introduce significant storage overhead, we propose three levels of denormalization that users can choose from to balance memory overheads and desired performance.  
%a area overhead of less than 1\% compared to the chip area, based on our RTL evaluations.

Using the widely-accepted SSB and TPC-H benchmarks, our bank-level PIM architecture obtained an 5.92x/6.5x speedup compared to a traditional schema and 3.03-4.05x speedup compared to a denormalized schema with 9-17\% memory overhead, depending on the degree of partial denormalization. Further, we provide insights into query selectivity, memory overheads, and software optimizations in the context of PIM-based filtering, which better explain the behavior and performance of these systems across the benchmarks. %\ks{fill in numbers}

==> Membrane/Sections/Architecture.tex <==


% overall architecture setup 
    % host + DRAM (optional: TODO depends on Membrane cost) + Membrane
    % what does the Membrane store: full WT or partial WT?
        % how does it make a decision to store selected 
        % we explore two flavors of PIM with different tradeoffs, point to the subsections
        % <,>,=, etc...
        % no 'like' string fuzzy matching yet
    % Mode one high-level idea
    % Mode two high-level idea
    % possibly Mode 1.5

% Membrane-H
    % architecture description
    % data layout  (leveraging data morphine?)
    % other architecture description
    % how to support mode one and mode two

% Membrane-V
    % architecture key ideas
    % why a Sieve/DRAM-CAM-based approach
    % circuit dict-encoding preserves order
    % data layout 
    % how to support mode two

\vspace*{-0.06in}
\subsection{Membrane-V}


% TODO: remove the second inverter, change to 1-bit filter logic

%Contrary to Membrane-H, the key design choice of [Cut to avoid comparison to something we haven't defined yet]
Membrane-V performs query predicate filtering in an \textit{ele\-ment-parallel} but \textit{bit-serial} manner. This operation can be carried out by laying the data vertically (column-major) along the bitlines of DRAM chips. Filtering is performed as a series of row activations, with each activation processing a given bit position ({\em bit slice} across many bitlines, i.e., data items. To support database query filtering,
%(AKA table scan)
only simple bit-wise relational operations are needed. DRAM-based PIM architectures that process data bit-serially, leveraging a vertical data layout, come in two categories: one utilizes a charge sharing (i.e., analog) triple-row-activation (TRA) operation, which does not require additional logic at the row buffer level, and one that integrates digital  logic into the row buffer and can process data using normal DRAM single-row-activation (SRA). 

Prior works such as Ambit~\cite{ambit}, SIMDRAM~\cite{simdram}, ComputeDRAM~\cite{computeDRAM}, and DRISA~\cite{drisa} adopt the TRA-based approach.  While the TRA-based DRAM-PIM is more area-efficient due to the lack of additional digital logic along the width of the row boffer~\cite{ambit}, other than the additional row decoders, it is more energy-intensive and slower than the sequential single-row activation with digital circuits integrated at the row buffer ~\cite{sieve,DRAMCAM}. The TRA overhead is primarily due to: (a) raising each additional wordline increases the activation energy by 22\%~\cite{ambit}, and (b) there is an overhead of multiple row-wide copy operations to move data operands to the PIM-capable rows~\cite{simdram,ambit}. Furthermore, each TRA can only accomplish a bitwise  AND/OR/NOT/MAJ operation, and a series of TRA operations must be chained to support more complex operations such as those needed for table scan~\cite{simdram}). 

Alternatively, we can integrate bitwise digital relational logic directly into the local row buffers at the DRAM subarray level. For example, Sieve~\cite{sieve} and DRAM-CAM~\cite{DRAMCAM} embed a matcher after each sense amplifier for bit-serial exact pattern matching. We can extend this architecture by replacing the matcher hardware with a one-bit comparator that can support inequality to enable table scans (Fig.~\ref{fig:membrane_v}). 
%Note that the reference patterns in the original DRAM-CAM and Sieve literature are analogous to the WideTable entries in the Membrane device. The query patterns are the predicate values that a query filters on. Prior works~\cite{sieve,DRAMCAM} have shown that SRA-based DRAM-PIM offers significant performance and energy efficiency advantages over the TRA-based DRAM-PIM for comparison operations, because the desired comparison can be implemented directly.  Because TRA-based PIM is based on charge sharing, it is limited to a few basic operation such as Majority~\cite{simdram}, and thus requires several expensive row accesses to synthesize a comparison.
%, and the area overhead of the SRA-based DRAM-PIM can be comparable to a TRA-based one. 
%Therefore, in this project, we pursue an SRA-based Membrane-V.

\begin{figure*}
    \centering
    \includegraphics[width=0.5\textwidth]{Membrane/Arch_Figures/ComputeSliceDSE.pdf}
    \caption{Membrane Design Space Exploration: 1. Compute Slice at the Subarray-level 2. Compute Slice at the Rank-level 3. Compute Slice at the Bank-level }
    \label{fig:membrane_dse}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{Membrane/Arch_Figures/DRAM_organization.pdf}
    \caption{DRAM Organization with Membrane PIM compute slices at the subarray-level}
    \label{fig:membrane_subarray}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{Membrane/Arch_Figures/membrane-bank.pdf}
    \caption{DRAM Organization with Membrane PIM compute slices at the bank-level}
    \label{fig:membrane_bank}
\end{figure}

\textbf{SRA-based Membrane-V Architecture.} 
Fig.~\ref{fig:membrane_v} illustrates the overall architecture of Membrane-V, including the vertical data layout and the circuit design to enable predicate table scans. The form factor required to integrate Membrane-V into the host system can be flexible.  Each Membrane-V chip comprises multiple banks, similar to a commodity DRAM chip. However, within each bank, Membrane-V has an additional layer of hierarchy called \textit{Subarray Groups}. 

\textbf{Subarray Groups.} Similar to Sieve Type-2~\cite{sieve}, in Mem\-brane-V, a subset of adjacent subarrays within a bank are connected through high-bandwidth links (isolation transistors) to form a subarray group. No modifications are made to a subarray in Membrane-V, except the last subarray's row buffer in each subarray group is extended with a filter logic array, mainly consisting of a row of 1-bit comparators with auxiliary bit-latches (described below).  Subarray groups within a bank can independently scan their stored wide table entries by sequentially activating rows of a subarray, transferring them into the last subarray's filter logic array using the LISA mechanism~\cite{lisa}, and performing the bit-serial comparison between attributes of the wide table entries (e.g., d\_year) and the target values (e.g., 1994).  The LISA mechanism enables the intra-subarray-group row-wide data relay by sequentially activating the local row buffers between the source and last subarray~\cite{sieve}. The latency of making one ``hop" from one row buffer to the next consists of enabling the isolation transistors (link) and the activation of the sense amplifiers, which is only $1/8$ of a regular row activation~\cite{sieve}. 

\textbf{Data Layout.} To support table scan in Membrane-V, we adopt a column-major bit layout similar to that proposed in~\cite{simdram,bitweaving}.
%several PIM proposals, namely Sieve \cite{sieve}, DRAM-CAM \cite{DRAMCAM}, SIMDRAM\cite{simdram}, ComputeDRAM \cite{computeDRAM}, Ambit \cite{ambit}
The dictionary-encoded WideTable entries are thus transposed onto bitlines for column-wise placement. Each attribute occupies consecutive bits in one column (i.e., spanning multiple rows) in the order of MSB to LSB. Because the transmission delay of the long wordlines prevents a predicate value bit from being dispatched to all comparators in a subarray row during one DRAM row cycle, the whole subarray is further broken down into smaller groups of columns called \textit{pattern groups}. Within each pattern group, a block of WideTable entries is followed by a column of predicate value populated at run-time. All pattern groups work in a lockstep manner by comparing the predicate value with WideTable entries in that pattern group. This is somewhat similar to how a large logical subarray actually consists of smaller mats, each with a wordline amplifier.  After a row is latched into the row buffer of the last subarray through row activation and LISA, the predicate bit is sent to all comparators within a pattern group through a 1-bit bus.

% RESTORE IN CAMERA-READY COPY IF SPACE PERMITS
%For numerical attributes, we preserve their relative order when we perform the %dictionary encoding, i.e., smaller original values are encoded with smaller binary %values than larger values. Therefore, we can safely support relational comparison %in Membrane-V. For attributes with string values, currently, Membrane-V only %supports equality checking using the dictionary-encoded binary, which is sufficient %to support all 13 queries in the SSB benchmark suite. We leave fuzzy string %matching for future work.


\textbf{Filter Array.} The crux of the Membrane-V architecture is its ability to perform a relational comparison (e.g., $=$, $<$, $>$, etc.) between a block of table attributes (e.g., \textit{d\_year}) and a predicate value (e.g., \textit{1994}) bit-serially. This is handled by a filter array integrated at the last subarray in each group. The filter array consists of a row of 1-bit filter logic, which connects to a sense amplifier and a 1-bit bus for inputs. Fig. \ref{fig:membrane_v} bottom (pre-synthesized gate-level diagram is shown for clarity) shows the hardware logic of the 1-bit comparator that determines if one attribute stored in a bitline is smaller, equal to, or larger than the predicate value by making a comparison at every bit position and capturing the running result in the S\_bit (stop bit) latch and R\_bit (result bit) latch. Each subarray row activation delivers one attribute bit (through the sense amplifier) and one predicate bit (through the 1-bit bus) to each filter. If after $n$ sequential row activations, where $n$ is the attribute bit-length, the value of an attribute is $>$/$<$/$=$ to the predicate value, then the R\_bit latch stores $1/0/0$, and the S\_bit latch stores $1/1/0$. The final bits stored in the R\_bit latch and the S\_bit latch are transferred to the Membrane controller to produce the bitmask. To support ranged predicate filtering, such as \textit{1994$<$d\_year$\leq$ 1997}, the Membrane-V runtime would break it down to multiple relational searches (i.e., \textit{1994$<$d\_year}, \textit{d\_year$<$1997}, and \textit{d\_year$=$1997}), execute them separately and aggregate the final results. 
%\ks{@Lingxi - why is a separate search needed for equal. Explain. Lingxi response: See the above explanation. Each comparison yields two bits, one in R\_bit latch and one in S\_bit. If the value of an attribute is evaluated to be $>$/$<$/$=$ to the predicate value, then the R\_bit latch stores $1/0/0$, and the S\_bit latch stores $1/1/0$.}

\textbf{Write Broadcast.} We observed that the latency of writing predicate values to the query regions of the subarrays takes substantially more time than the actual row-activation time spent on matching the predicate (Sec \ref{sec:breakdown}.) Since the predicate value bits written into each subarray are identical and are destined to the same row and column addresses, we propose a simple optimization that broadcasts the predicate bits simultaneously by connecting all participant subarrays' local row buffer to the global data lines, allowing them to accept the predicate bits at the same time. The hardware cost to the Membrane chip is negligible because the wires and the routing for the control signals are already in place \cite{salp}.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{Membrane/Arch_Figures/membrane_h.pdf}
    \caption{Membrane H}
    \label{fig:membrane_h}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{Membrane/Arch_Figures/membrane_v.pdf}
    \caption{Membrane V}
    \label{fig:membrane_v}
\end{figure}

%\vspace*{-.05in}

==> Membrane/Sections/Architecture_2.tex <==
\section{Architecture \bold{(NEW!)}}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{Membrane/Arch_Figures_2/DRAM Design Space Exploration.pdf}
    \caption{Membrane Design Space Exploration: 1. Compute Slice at the Subarray-level 2. Compute Slice at the Rank-level 3. Compute Slice at the Bank-level }
    \label{fig:membrane_dse}
\end{figure}

\subsection{PiM Design Space Exploration at DRAM hierarchy}
%\begin{enumerate}
%    \item \hl{Introduce SCAN capability at subarray-level, bank-level, rank-level}
%    \item \hl{Assumptions of the experiment}
%	\item \hl{Single DRAM read triggers a PiM computation}
%	\item \hl{Subarrays are sensitive data placement (optimistic and pessimistic)}
%	\item \hl{LISA mechanism utilized for subarray-level processing}
%    \item \hl{Beyond bank-level we see diminishing returns }
%    \item \hl{Subarray-level 4.56x/5.92x/8.68x/14.18x (SALP-1/2/4/8) expensive in terms of area and power and improves the end to end execution by only 13\% for (SALP-8) as compared to bank-level }
%    \item \hl{Takeaway - Bank-level offers an optimum parallelism}
%\end{enumerate} 

\hl{The previous section spoke about how the SCAN kernel was the most amenable for PiM acceleration. In this section, we aim to look across the DRAM heirarchy and consider the most suitable location to place our PiM processing elements (PEs).

DRAM is a hierarchical hardware structure which is organized into channels, ranks, bank groups, banks and eventually subarrays. Each memory channel is considered independent for the most part and runs in parallel, while each channel itself is made up of only multiple ranks. Each rank is said to be made of multiple bank groups and banks, and each bank in turn is composed of multiple subarrays. Due to the data path being shared, only one rank, bank group, bank or subarray can be active at any given time. With PiM architectures, we are presented with a choice to avoid this common data path and instead process data nearest to each element. This not only opens up a large degree of parallelism but also opens up significant bandwidth for parallel processing at each level.

Fig-1 presents the results of time taken to perform a scan(or filter) operation on one column of a fact table in Star Schema Benchmark (SSB) at Scale Factor-100. Each column consists of 600,038,146 elements of 32-bits and the overall column size is 2.24 GByte. The experimental setup and methodology for this evaluation is discussed in section - TODO. We consider the DDR4\_8Gb\_x8\_3200 configuration from DRAMSim3 and based on CACTI evaluations we observe that each bank is made up of 16 subarrays per bank with each subarray containing 4096 rows.

All-Bank mode is the mode in which PEs placed in multiple banks/subarrays are processing data parallely at the same time. As we can observe from the graph, the all-bank mode always outperforms the single bank mode since the large parallelism and bandwidth gains increase the scan performance significantly. Note that the rank-level cannot support All-Bank mode since we assume PiM PEs to be placed at the rank-level and only one bank at a time can feed the data into these rank-level units.

The subarray-level PiM design we assume has processing elements placed at each of the subarrays specifically near the row buffers. The subarray design space presents us with two unique  factors to consider while evaluating how the subarray-level architectures viz. (i) Subarray-level Parallelism (SALP) - dictates how many subarrays support compute capability within the same bank and can process data parallelly at the same time (ii) data placement - optimistic data placement is scenario where data is considered to be stored closest to the nearest compute-capable subarray while pessimistic data is where data is considered to be farthest from the compute capable subarrays. The question of data placement arises in a situation where only certain number of subarrays have compute capability and data needs to be moved from each subarray to another to get it processed. We consider the LISA technique for inter-subarray movement within the same bank as it leverages the existing bitline structures to enable faster copying without incurring a large area overhead. Since each row buffer is shared between two subarrays and our design considers 16 subarrays per bank, a maximum of 8 subarrays can be active at any time due to the shared row buffer resource. Thus, in this design, we explored a maximum of SALP-8 and have presented the results.

We can gather from the results that with increasing subarray-level parallelism, the scan performance too increases. In the case of optimistic data placement, the decrease in performance is proportional to the parallelism introduced. However, in the case of pessimistic data placement, we observe that performance degrades exponentially since more number of cycles are spent on moving the data from the farthest subarrays to the compute-capable subarrays. However, overall, SALP-8 provides the best scan performance and since almost every subarray has the compute capability, the issue of data placement does not alter the results in these two scenarios. 

With regards to the bank-level architecture, we envision a PiM Processing Element (PE) to be placed at each bank feeding off the data from the internal data path of each bank. Thus, SALP-1 is equivalent to the bank-level PiM. The SALP-1 in pessimistic data placement scenario is slightly higher than Bank-level since the difference in execution time is accounted for by the LISA movement to shift data between the subarrays. The SALP-1 optimistic data placement scenario is slightly better than the bank-level PiM since when writing the bitmaps back into the subarrays, this is done with a single row activation, where as in the case of bank-level PiM, the bitmap has to be written at the granularity as allowed by the internal data bus of the bank which tends to make it slower in the case of bank-level parallelism.}

\subsection{PiM Design Space from End-To-End Application Perspective}
\hl{However, when the PiM design space is looked at from the end to end application perspective, we observe that a moderate degree of bank-level parallelism is only X% (TODO) faster than the SALP-8. 
We take the results from PiM scan performance analysis and evaluate the entire end to end application execution time for all the SSB queries. The results for the same are presented in Fig-2. 
These observations can be explained by the Amdahl's law wherein the parallelizable portion such as the scan kernel can only speedup the application to a certain extent and there is diminishing returns beyond a certain degree of parallelism. 
Based on these results, we suggest that bank-level parallelism is sufficient in accelerating the scans and that subarray-level PiM although offers a higher degree of parallelism can only accelerate the overall application marginally. Also, subarray-level parallelism suffers from a higher area overhead and tends to alter the DRAM subarray structures significantly. The subarray structures are generally optimized latency and capacity and any in-situ changes to these structures are generally avoided. The bank-level PiM is shown to be more amenable to modifications with frequent changes to its structures across generations and commerically available bank-level PiM already in the market. Hence, bank-level PiM offers us the best choice in terms of where to place the PiM Processing Elements (PEs) across the DRAM hierarchy considering the end-to-end application perspective.}

\subsection{Bank-level Membrane Architecture}
\textbf{Comparator unit (CU).}
\hl{The heart of all versions of Membrane is the \textit{Comparator Unit}, a {\em scalar} unit that can support both equality check (input\_record == a) and range check (x < input\_record < y) on integer or fixed-point values. Each comparison produces a result bit that is and-ed into the bitmap, which is stored in a local {\em bitmap buffer}, or in a row-buffer-like structure called a {\em walker} \cite{fulcrum} --- see below.  When performing a sequence of filtering steps, the CU reads the current value of the bitvector for the current position, and ANDs this with the result from the new comparison.  In this way the bitvector accumulates the final Boolean result. }

\hl{Range checks are implemented using subtraction.  The CU is a scalar unit, supporting operands up to the width of the DRAM global bit lines, i.e. the DRAM device width (e.g., 16 bits).  The CU does not support processing string inputs or regex operations, as these are infrequent and area-prohibitive for PIM implementation. In any case, since we  operate on the denormalized WideTable, which is dictionary-encoded, the comparator unit would not encounter any strings as they are all encoded as integers, making them compatible for PIM CUs. A high-level breakdown of the Comparator Unit (CU) is represented in Fig-TODO. }

\hl{To support data fields that are wider than the burst width (e.g., x8), the CUs are 64 bits, and inputs are read in a bit-sliced, in the sense that they read their inputs in bursts.  For example, reading a 64-bit input in a x8 chip requires 8 reads to assemble the input.  If the database column being processed is less than 64 bits wide, the CU can process multiple values; e.g., the 64-bit input can be made of four 16-bit values and produce 4 output bits in one step.  The advantage of this approach is that  the input dataset may contain records with varying lengths from 8 to 64 bits, and the CU can support this while maintaining full utilization. The Control Unit (discussed later) issues control signals to operate the  CUs in the desired configuration.}

\hl{Scratchpad size (to store bitmaps)}  At the bank and rank level, the CU contains a bitmap of \ks{SIZE} bits. When it is full, it is written back, one burst at a time. At the subarray level, the Compute Slices use a Walker, which the Control Unit flushes when it fills up.

\hl{The \textbf{Control Unit} is responsible for coordinating the control signals to manage the operations of the PIM unit and ensure that it is synchronized with the DRAM portion of the bank. Its primary function is to generating control signals for the bit-sliced CUs to operate in 8, 16, 32, or 64-bit modes, orchestrating the comparison operations within the Compute Slice, and writing the result bitmap back when the bitmap buffer is full. }
    
\hl{Processing data every t\_CCD}
    
\end{enumerate}


==> Membrane/Sections/Architecture_Intro.tex <==
% Design Goals - Given that our main goal was to accelerate the query processing particularly, we wanted to aim for a PIM architecture that is very optimized to handle this specific application only. This not only allows us to ensure the least possible hardware overhead but also ensures a more coherent software-hardware architecture that is co-designed to make complete utilization of the available resources. Oftentimes having large hardware overheads in PIM designs leads to reduced clock speeds to make sure one does not breach the thermal constraints associated with the design. Adversely reduced clock speeds of the PIM architecture also lead to decreased performance of the architecture, which can be quite significant considering that the baseline comparison, i.e., CPU has clock speeds in the range of a few GHz while the memory is usually in the range of a few MHz. Hence, maintaining a very lean architecture super optimized for database application allows us to deliver the best possible performance and also ensure the design is quite manufacturable due to significantly reduced logic being added to the DRAM designs. 

\mrtn{Reviewer comments stressed that the presentation here feels ``split:'' We explore both Membrane-H/-V, but do not link them together as much as desired. This introduction paragraph feels that way; can we explicitly place a comparative analysis (even if it's small) somewhere in this section, so we can talk about -H and -V together in this introduction paragraph?}
In this section, we present two versions of the Membrane PIM architecture. Membrane-V (Vertical) is a bit-serial and element-parallel architecture that extends the exact pattern-matching capabilities of Sieve/DRAM-CAM-style architectures~\cite{sieve,DRAMCAM} to process range queries. Membrane-H (Horizontal) is an element-serial bit-parallel architecture based on Fulcrum~\cite{fulcrum}.  %Figure-\ref{fig:Membrane_arch_overview} \textcolor{blue}{TODO FIX}provides an overview. 
%In this project, we consider Dual-Inline Memory Module (DIMM), and a host can communicate the commands and data with Membrane-V through a modified memory controller (Section-\ref{sec:system integration}). 
%A typical DDR4 DIMM provides around 0.37 Watt/GB~\cite{micronPower} of power delivery and 25 GB/s of bandwidth, which is sufficient for Membrane (see Section \ref{sec:results}).

%\subsection{Operational Modes} \label{sec:op_modes}
%    \begin{figure}
%        \centering
%        \includegraphics[width=0.8\linewidth]{Membrane/Arch_Figures/Execution Flow.pdf}
%        \caption{Membrane Operation Modes}
%        \label{fig:Membrane_Op_Modes}
%        \vspace*{-.25in}
%    \end{figure}

%\sout{In analyzing the time spent on filtering versus data retrieval and aggregation operations, we find that that in queries with high selectivity (fewer records are selected), filtering dominates the execution time. However, in queries with low selectivity, as much as 75\% of the execution time is spent gathering the selected data. This means that the memory system should gather the data selected during filtering and return that as a contiguous block to improve the locality for the aggregation stage, instead of merely providing to the CPU a bitmask of selected records and requiring the CPU to fetch the records.  We therefore evaluate two modes of operation, \textit{Bitmask} and  \textit{Data Push}.}

%    \subsubsection{\textit{Bitmask Mode}} \label{partial wideTable paragraph}
%    \sout{In the Bitmask mode, the PIM device is only responsible for accelerating the filtering operation and communicating the results to the CPU in the form of a bitmap.}
    %\sout{This bitmap has an entry for every record in the database. A value of 1 in the bitmap indicates the selection of a specific record, %while filtering the WideTable
    %while a value of 0 indicate a record that did not match the selection criteria.} 
%    \sout{The CPU finishes the remaining part of the query execution i.e. the aggregate operations, by examining the bitmap and retrieving records that qualified.} %from a second copy of WideTable stored in the main memory.
    %The memory controller finishes the remaining part of the query execution i.e. the aggregate operations, by examining the bitmap and  retrieving records that qualified. %from a second copy of WideTable stored in the main memory.
    
%    If the user has knowledge of the queries to be executed in advance, then a partial WideTable built with only specific database columns that are used for processing queries could be joined together and loaded into the PIM memory. This reduces the size of the WideTable used for filtering operation significantly, thereby occupying less PIM memory. \ks{@Lingxi or @Akhil, describe in more detail what we did in our experiments in terms of a reduced WideTable.} \textit{(Akhil: I have written this and the following paragraph to address what is going on with the reduced WideTable and explained about the data layout of this reduced WideTable. Let me know if any changes are required.)}
    
    
    
%This also provides system designers with a choice to have a mix of PIM memory and main memory of different capacities and ratios. The database software could use this knowledge to tweak the WideTable sizes to fit into the available PIM and main memory space.    The database designers could also take advantage of this mode and cache the most frequently used columns for filtering into the PIM memory on the fly and use it for accelerating portions of the query execution. One of the goals behind this mode is to minimize the expensive data transfers over the memory bus.
    
%    \subsubsection{\textit{Data Push Mode}}
%    \sout{In this mode, the PIM} %\sout{takes on more of the query processing work and also} 
%    \sout{pushes the selected data to the CPU, instead of merely sending the bitmask. Due to the architectural differences between the Membrane-V and Membrane-H, this mode is implemented in a different manner for each. 
    For Membrane-V, because records are laid out vertically (column-wise) along a bitline, the retrieval of the selected data would require many row activations to retrieve each bitslice of the selected records.  Instead  Membrane-V uses a second copy of the WideTable data that is stored elsewhere in memory and in the traditional horizontal format along a subarray row. The memory controller first issues the filtering command and receives the resulting bitmask, and then retrieves the data. For Membrane-H, in which the data is already in a row-wise horizontal layout, the processing unit can gather the data items immediately as they are selected. % as shown in  Figure-\ref{fig:Membrane_arch_overview}. %from and copies it into a dedicated buffer, from which the CPU fetches. This buffer is updated using a latency-insensitive interface between the CPU and the memory controller 
    Section IV presents more details on the orchestration with the memory controller.
    %We evaluated both late materialisation and early materialisation methods on both architectures and found that early materialisation works naturally well for Membrane-H due to its lower batch size (horizontally laid records) compared to larger ones for Membrane-V (due to vertically laid data). Since smaller batches are filtered sequentially by Membrane-H, they can be sent to the CPU for earlier materialisation while larger batches being processed by Membrane-V need to wait longer for an entire batch to be completed before materialising. In the paper we present the following details related Early Materialisation Method with Membrane-H and Late Materialisation Method with Membrane-V.
    %\sout{\ak{AK - Need modify this section to reflect the changes to opreational modes}}
    

%It is much easier for the Membrane-H architecture to retrieve the necessary columns since the database records are layed out horizontally and requires very less number of row activations to perform the same. Hence, 
%The complete version of the WideTable can be stored in the Membrane-H PIM memory and it can act as a drop-in replacement for main memory. 

%\sout{We also considered hybrid layouts, mixing properties of vertical and horizontal, but found that the column-major layout was consistently best for Membrane-V, and row-major was best for Membrane-H.}

%Data layout is another design choice. We explore three options.
% Row-major layout refers to laying out all the attributes of the same database %record along a subarray row while the column-major layout refers to laying down %similar attributes of different database records  along a subarray row, i.e. a %columnar database organization. Hybrid data layout refers to a combination of both, %optimized for which columns tend to be used together, in order to increase locality %in row utilization.
 %We analyze and group the database attributes which are frequently referenced together in the queries, and place these groupings along the same subarray rows in order to increase the row hits. See Figure-\ref{fig:data-layouts},

%\begin{figure}
%\centering
%\begin{subfigure}[t]{0.65\linewidth}
%    \includegraphics[width=\linewidth]{Membrane/Arch_Figures/Row Major layout.pdf}
%    \caption{Row-major data layout.}
%\end{subfigure}%
%    \hfill%
%\begin{subfigure}[t]{0.65\linewidth}
%    \includegraphics[width=\linewidth]{Membrane/Arch_Figures/Hybrid Layout.pdf}
%    \caption{Hybrid data layout.}
%\end{subfigure} 
%\begin{subfigure}[t]{0.65\linewidth}
%    \includegraphics[width=\linewidth]{Membrane/Arch_Figures/Column Major Layout.pdf}
%    \caption{Columnar data layout.}
%\end{subfigure}%
%\caption{Data layout choices to support Membrane-H Bitmask mode and Membrane-V/H Data push mode. %(Each colored block represents a database attribute)}
%\label{fig:data-layouts}
%\vspace*{-.2in}
%\end{figure} % TODO, move to the architecture section

==> Membrane/Sections/Background.tex <==

% Query process on a conventional system 

% SSB, data type 

% DRAM-based PIM landscape?: bit-serial/parallel, element-parallel/serial



% Database Background 
%  - Difference between the Analytics and Transaction Databases
% SSB Benchmark
%  - Query Processing Steps and breakdown of filtering, aggregate and other operations
%  - Von Neumann Bottleneck between moving data between CPU and memory and the necessity for PIM 
%  - Decades of prior research to tackle this (Database Machines?)

% Database Market Opportunity

%  - One of the most used workload in the data centre 
%  - Very much financially lucrative to large cloud scale vendors
%  - Total addressable market area
%  - Sacrificing generalisation for specialisation for this specific application
%  - Database can be a killer app for PIM
%  - Low computation and large data movement associated with database applications 

% 2 figures go here 
% 1. Showing DRAM-bound nature of the workload
% 2. Showing the cycle breakdown of the workload

% 

\section{Background}

\begin{figure}
    \centering
    \begin{subfigure}{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Membrane/Introduction_Figures/olap-schema.pdf}
        \caption{OLAP schema}
        \label{fig:olap-schema}
        \vspace{10pt}
    \end{subfigure}
    \begin{subfigure}{0.53\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Membrane/Introduction_Figures/olap-query.pdf}
        \caption{OLAP query}
        \label{fig:olap-query}
    \end{subfigure}
    \caption{An example OLAP scenario.}
    \vspace*{-10pt}
    \label{fig:olap}
\end{figure}

\begin{figure*}
    \centering
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Membrane/Result_Figures/breakdown-ssee2e.pdf}
        \caption{Components of execution time according to VTune for hand-optimized SSE CPU implementation of SSB queries}
        \label{fig:memory-profile-e2e-prefetch-enabled}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \centering
            \includegraphics[width=\linewidth]{Membrane/Result_Figures/bandwidth-utilization.pdf}
    \caption{SSB queries maximize utilization of available memory bandwidth. Each query was run repeatedly for 10 seconds and the memory bandwidth utilization was measured with VTune.}
    \label{fig:bandwidth-utilization}
%        \includegraphics[width=\linewidth]{Membrane/Result_Figures/breakdown-ssee2e-noprefetch.pdf}
%        \caption{REPLACE WITH BANDWIDTH FIGURE}
%        \label{fig:memory-profile-e2e-prefetch-disabled}
    \end{subfigure}
    \caption{Memory access profile of SSB queries.}
    \label{fig:memory-profile-e2e}
\end{figure*}

\begin{figure*}
    \centering
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Membrane/Result_Figures/breakdown-ssefilter.pdf}
        \caption{\textit{Filter} part}
        \label{fig:memory-profile-parts-filter}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Membrane/Result_Figures/breakdown-aggbitmap.pdf}
        \caption{\textit{Aggregate} part}
        \label{fig:memory-profile-parts-aggregate}
    \end{subfigure}
    \caption{Memory access profile of SSB query constituent parts.}
    \label{fig:memory-profile-parts}
\end{figure*}

\begin{figure}
    \centering
    \vspace*{-9pt}
    \includegraphics[width=0.9\linewidth]{Membrane/Result_Figures/selectivity-all.pdf}
    \caption{Relative time taken by \textit{Aggregate} versus query selectivity. The remaining percentage represents portion of the execution time that can be accelerated by PIM.}
    \label{fig:aggregate-percentage}
\end{figure}

%\begin{figure}
%    \centering
%    \vspace*{-4pt}
%    \includegraphics[width=\linewidth]{Membrane/Result_Figures/bandwidth-utilization.pdf}
%    \caption{SSB queries maximize utilization of available memory bandwidth. Each query was run repeatedly for 10 seconds and the memory bandwidth utilization was measured with VTune.}
%    \label{fig:bandwidth-utilization}
%\end{figure}

Many OLAP workloads are characterized by their emphasis on analyzing historical data, as compared to Online Transaction Processing (OLTP) workloads that generally facilitate business transactions~\cite{OLAPvsOLTP}.
The differences between OLAP and OLTP workloads have driven specialization in database platforms, where analytical and transactional query processing are regularly performed by two separate database solutions.
In many cases, the archived data is stored as a read-mostly, append-only database, commonly referred to as a data warehouse~\cite{Chaudhuri1997}, while the transactional database, typically much smaller, stores the latest copy of the key tables in the database. %For example, in an e-commerce application, information about current orders is part of a transactional database, and the history of all orders is part of the warehouse database used for OLAP queries. The transactional database is usually smaller in size and the data warehouse is much larger, as it keeps track of all the transactions over time.

An OLAP database typically consists of \emph{fact} tables and \emph{dimension} tables. Fact tables often contain historical transaction records, and dimension tables contain detailed information for specific parts/columns in the transaction records. For example, the database shown in Figure \ref{fig:olap-schema} contains an order fact table, which includes a record for each order that is submitted. Each order record stores information about the order, including its price, discount, and quantity 
%(stored in the \textit{o\_price}, \textit{o\_discount} and \textit{o\_quantity} columns resp.).
The database also contains several dimension tables that each describe a different dimension of the order, such as the date the order was placed, the product that was ordered, the customer that submitted the order, and the supplier that fulfilled the order. The \textit{o\_*\_key} columns in the fact table are foreign keys that point to the primary entries in the dimension tables serving as logical pointers connecting records across different tables. Typical OLAP queries involve  selecting %``slicing and dicing''
the data along these dimensions and then aggregating the results to satisfy a specific analytical query. For example, the SQL query shown in Figure~\ref{fig:olap-query} enumerates the product categories that are most popular among customers in their 20s. %Additional queries could be used to ``drill down'' into additional dimensions of the orders, such as the regions from which they were fulfilled or the months in which they were placed.

%\av{It is unclear what you mean by prediction in the following paragraph.  Given the experiment that follows, it seems like you're hypothesizing and then verifying your hypothesis.  Also, the methodology used for experiment needs to be clearly described.} \ks{Hopefully I addressed the first concern with some minor rephrasing.} \jmp{rewriting the next para, so the comment above may not apply. @ks can remove the comments on his pass on this section.}

OLAP queries are data-intensive, because the number of cycles per record of input data is often small -- for example, on the customer records in the SQL example above, the computation is merely to apply the selection predicate. 
%As CPU speed and memory sizes have both increased at faster rates than the memory speed and memory bus bandwidth, OLAP query evaluation in main-memory environments (the focus of this paper) are often memory-bound. 
To verify the hypothesis that OLAP queries are typically memory-bound, we use Intel VTune \cite{vtune} to profile hand-optimized C++ implementations using SSE for the thirteen queries in the Star Schema Benchmark (SSB) \cite{ssbbenchmark} when run on a typical server (Intel Xeon Platinum 8260 with 24 cores and 376 GB of DRAM). More details on the implementation and the server are provided in Section \ref{sec:methodology}. Figure \ref{fig:memory-profile-e2e-prefetch-enabled} shows the time spent by the CPU on accesses to DRAM and the L1, L2, and L3 processor caches. The remainder shows the time spent by the CPU on non-memory operations. The CPU appears to spend the majority of query execution time stalled on DRAM, with L2 stalls comprising a large portion of time as well.

At first glance, the fraction of time spent in L2 stalls appears unexpectedly high for some queries, such as Q1.2. However, we suspect that many of these L2 stalls were linked to the L2 hardware prefetcher, which fetches additional lines of data into the L2 cache when certain access patterns are detected.
%As a result, while VTune categorizes these stalls as L2-bound To confirm this hypothesis, we disabled hardware prefetching on the CPU and re-ran the benchmark. Figure \ref{fig:memory-profile-e2e-prefetch-disabled} shows the memory access profile with prefetching disabled. As expected, the vast majority of execution time is spent on DRAM stalls. The remaining execution time is spent largely on L3 accesses and non-memory operations. In addition,
We therefore measured memory bandwidth utilization while running each query repeatedly for 10 seconds, to allow VTune to collect a sufficient number of samples. Figure \ref{fig:bandwidth-utilization} shows that all queries saturate the memory bus and use all available memory bandwidth, despite the VTune statistics regarding L2.  These results indicate that, while hardware prefetching mitigates DRAM access latency to a limited extent, SSB is nevertheless bound by the maximum memory bandwidth. 
%Therefore, the queries in Figure \ref{fig:memory-profile-e2e} are \emph{effectively} DRAM-bound, despite hardware prefetching. In other words, executing these OLAP queries identifies a streaming access pattern that potentially maps naturally to PIM; huge performance gain can likely be realized with a PIM-approach to OLAP query evaluation by harnessing the large data parallelism across banks, subarrays, and even potentially words within each row operation and avoiding the bottleneck of transferring large quantities of data to the CPU for filtering. 

Although we have shown that OLAP queries are largely memory-bound, a finer-grained analysis is necessary to identify their most memory-intensive operations and thus the most promising candidates for pushing into PIM. Therefore, we break down the queries in Figure \ref{fig:memory-profile-e2e} into two more fundamental constituent parts: \textit{Filter} and \textit{Aggregate}. \textit{Filter} scans the columns needed to answer the \texttt{WHERE} clause of each query and evaluates the conditions. The output of \textit{Filter} is a bitmap that represents the rows satisfying the \texttt{WHERE} clause. \textit{Aggregate} takes as input the bitmap produced by \textit{Filter}. For each set bit in the bitmap, \textit{Aggregate} accesses the corresponding row and performs the remaining work of the query, including any \texttt{GROUP BY} and \texttt{ORDER BY} clauses. Figure \ref{fig:memory-profile-parts} shows the memory access profile for \textit{Filter} and \textit{Aggregate}. \textit{Filter} (Figure \ref{fig:memory-profile-parts-filter}) appears to be largely bound by L2 accesses,
but we performed the same bandwidth characterization for just the Filter stage, and find that it is also saturating the DRAM-access bandwidth.%, meaning that it is also DRAM-bound.
%However, as before, these L2 accesses are effectively DRAM-bound. 
%but with prefetching disabled, we observed that \textit{Filter} spends 70-80\% of execution time on DRAM stalls. 
VTune also shows that \textit{Aggregate} (Figure \ref{fig:memory-profile-parts-aggregate}) is  largely DRAM-bound -- the sparseness of the bitmap results in effectively random access with poor cache locality, meaning the retrieval of the selected data is not easily prefetched, hence the substantial fraction of DRAM stall time. Note that some queries are so selective that, despite this poor locality, \textit{Aggregate} takes a minuscule amount of time, as few rows need to be accessed after the initial \textit{Filter}. However, for less selective queries such as Q3.1, \textit{Aggregate} takes over 75\% of the end-to-end execution time. Overall, the results in Figure~\ref{fig:memory-profile-e2e} confirm that Filtering is responsible for the supposedly L2-bound portion of the bars in Figure~\ref{fig:memory-profile-e2e-prefetch-enabled} and the continuous saturation of the bandwidth in Figure \ref{fig:bandwidth-utilization} shows that even these portions are bottlenecked by DRAM access.

Figure \ref{fig:aggregate-percentage} shows that using PIM to accelerate \textit{Filter} alone may not be enough, as this accounts for less than 25\% of execution time for queries such as Q3.1. Accordingly, we explore an additional processing step in the PIM, beyond simply filtering, that uses the filtering results as the PIM produces them and exploits the massive parallelism and data-gather capability %and internal bandwidth 
of PIM  to efficiently gather disparate rows into a contiguous block, which is then transferred to the CPU under control of the memory controller, as described in Section~\ref{sec:system integration}. The CPU then performs \textit{Aggregate} over these now-contiguous rows. The resulting locality  of this method (\textit{Aggregate-Dense} vs. \textit{Aggregate-Sparse} in Figure \ref{fig:aggregate-percentage}) drastically reduces the execution time of \textit{Aggregate} relative to the end-to-end execution time, hence increasing the maximum achievable speedup. We discuss the details of our methodology in Section~\ref{sec:methodology}.
%\av{Again, the sentence "... spends 70-80\% of execution time on DRAM stalls, but we omit this plot for brevity." seems to hurt more than help, without justification for turning off prefetching.}
%\ks{I think the issue here is twofold. 1. These results were produced using VTune running the actual DB software, so we can't characterize a more ideal prefetching mechanism.  And we don't have time to do a limit study in simulation. In any case, I'm not sure how to do a meaningful limit study that's not overly simplistic (like 100\% hit rate in L2). 2. The fact that prefetching works means these are streaming accesses that are perfect for PIM acceleration, leveraging the massive parallelism of these PIM architectures. So I think the question is how do we tell this story better.}

%\av{For the aggregate dense/sparse experiments, did we try performing "SIMD gather" into a buffer and then aggregate?} \ks{No, but we think the bottleneck is the gather. This would be a good experiment to try to prep for rebuttal, but don't have time now.}

Based on this analysis, it is evident that for the CPU, both filtering and data retrieval are limited by the rate at which data can be fetched from DRAM, and that performing filtering on the CPU entails substantial unnecessary data movement and thus energy expenditure, 
%and that data retrieval involves random accesses that are especi. 
%As the size of the dataset increases, these data movements are bound to become more expensive and be adversely affected by the effects of the memory wall~\cite{memorywall}.  
%Not only are these large data movements expensive in terms of energy, but also increase the latency of the operation. 
Hence, we  leverage processing-in-memory to leverage the parallelism of PIM architectures and overcome these inefficiencies, and  
%to push computation closer to where the data reside and leveraging the parallelism and  i.e. the DRAM and executing simple kernels such as the filtering which happen to be DRAM-bound. Since a major portion of the workload involves these large and expensive data transfers, 
we expect significant reductions in the execution time in addition to reduced energy consumption.
%while leveraging the parallelism and bandwidth gains provided by adopting PIM architecture.

%\ks{Would be nice to have some kind of comparison of peak throughput for CPU vs. PIM here, but we can cut this if necessary.}

As noted previously, to improve efficiency with PIM, we use the denormalized, pre-joined WideTable~\cite{widetable} representation.
This significantly improves the performance of OLAP workloads, due to the removal of expensive join operators during query execution.
This comes at a cost of increasing the size of the database, but we find that careful encoding limits the size increase to 18-22\%. The WideTable representation has been shown to significantly improve the performance of workloads due to removal of expensive JOIN operations as observed in \cite{rockset} \textit{(Akhil - For the above comment, There is a recent work %https://rockset.com/Rockset_Star_Schema_Benchmark_April2022.pdf - commented out because it was breaking the Latex 
from April 2022 that shows large speedups by following this approach.)} \ks{@KG, @MP, @JMP - Should we cite this as evidence of commercial adoption of WideTable?} \kpg{I think it's a good idea. We could reword the prior sentence to say something like: The WideTable representation has been shown to significantly improve the performance of OLAP workloads, due to the removal..., citing that benchmark study.}

%\ks{Can we do some kind of analytical model to estimate the peak filtering throughput of a multicore CPU vs. the peak throughput of our PIM architectures? I would start with just peak computational throughput of multicore AVX vs. Membrane H and V}
%\textit{Akhil - For review : Considering that the filtering operation is bandwidth constrained from Kevin's figure, the theoretical maximum for a CPU in filtering operation of 1-byte words = (2933MHz x 8 byte x 8 memory channel) = 187,712 Million bytes/second. Whereas considering a PIM element placed at every subarray-level for, the theoretical throughput of PIM would be : (2933 MHz x 4 bytes x 16384 subarrays) =  192,217,088 Million bytes per second. PIM architecture would have 1024x higher throughput than what is available at the CPU. For the PIM setup, we assume 16384 subarrays spread across the 8 channels, 2 ranks, 8 banks and 128 subarrays per bank with 16 bit column lines. } \ks{This is for Membrane-H? Is that the right clock speed for DRAM?  We are limited by the row cycle time and the slower logic speed. Also what if we have lower SALP, perhaps even pessimistically just bank-level parallelism? Also, it would be good to see what the peak throughput of all the cores' AVX engines are.} 

% Notes about the PIM throughput calculations, yeah the analysis would be very different depending on each level of SALP.
% Since the area overhead is kept to the minimum, we are assuming it to run at native DDR speeds
% The PIM throughput also drastically changes if the internal DRAM organization changes (for ex. reducing the number of subarrays by making each much larger), hence there are lot of variables to put in just to arrive at the number. This was one of the reasons that we didnt wanted to do analytical calculations earlier. 

% About the theoretical throughput with all core's AVX
% Throughput = 3.9 Ghz x 128bit or 16-byte x 24 cores = 1,497 billion Operations per second 
% This is a large number.

==> Membrane/Sections/Conclusion.tex <==
\section{Conclusions and Future Work} \label{sec:conculsion}

%1. Proposed end to end query processing framework on PIM

%2. Performed a design space space analysis between the Membrane-V and H versions

%3. Explored the issue of data layouts in the PIM architecture 

%4. Proposed 2 modes of operation for PIM execution (Bitmask mode - Data Push Mode)

%5. We got X amounts of speedup with Membrane-V/H versions with following area overheads and energy reductions (To be filled)

%-- Future work is to support the Update operations on PIM and explore the OLTP and HTAP workloads

%-- Proposed datacentre level disaggregation of Compute, Memory, and Storage, explore PIM tehcniques in this surrounding

%\ak{ak - In this work, we aim to center the query execution of OLAP workloads around the inherent advantages and capabilities of PIM architectures and develop a low-overhead end-to-end query execution accelerator called Membrane.}
Our proposed PIM architecture, Membrane-V/H is shown to have a geomean end-to-end speedup of 5.94x/45.39x over a highly optimized reference CPU codebase 
%\cite{kevin_github} 
implementing the SSB Benchmark while achieving an energy reduction of 10.00x/70.77x. Membrane-V/H are also evaluated to have a speedup of 90.26x/359.21x over a state-of-the-art analytical database engine---DuckDB \cite{duckDB}---while having an area overhead of 3.42\%/2.07\%. We have conducted a detailed design space analysis of not only the PIM architecture but also describe the system integration and end-to-end performance. Membrane demonstrates the potential of subarray-level processing-in-memory architectures to accelerate analytics-based OLAP workloads, and shows the value of PIM for accelerating table scans.  This work also shows the value of the H layout with early materialization using Rank-level Units (RLUs) to perform data-retrieval related gather operations. The growing memory wall, combined with rapid growth in data volumes, motivate processing-in memory architectures such as Membrane to accelerate data-intensive workloads such as OLAP queries. %\sout{ to offer better insights   interest in disaggregated datacenter architecture with pools of CXL-attached~\cite{cxl}  memory shared among nodes composed of separate compute, memory, and storage pools.}\sout{In future, we would like to extend this work to support Hybrid transactional/analytical processing (HTAP) database workloads  by introducing support for database update operations on PIM. Furthermore, there is growing interest in disaggregated datacenter architecture with pools of CXL-attached~\cite{cxl}  memory shared among nodes composed of separate compute, memory, and storage pools.}
%, and we also want to investigate the role of Membrane in this setting. %, and explore the potential performance benefits of pushing down database operations close to the memory in a disaggregated memory setting. 
%\textcolor{blue}{TODO AK - Remove CXL reference}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{Membrane/Arch_Figures/Mem_v_arch.pdf}
    \caption{Membrane-V Architecture.}
    \label{fig:membrane_v}
    \vspace*{-.1in}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Membrane/Arch_Figures/ComputeSliceDSE.pdf}
    \caption{Membrane Design Space Exploration: \large{\ding{172}} Compute Slice at the Subarray-level \large{\ding{173}} Compute Slice at the Rank-level \large{\ding{174}} Compute Slice at the Bank-level }
    \label{fig:membrane_dse}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Membrane/Arch_Figures/membrane_full_figure.pdf}
    \caption{Membrane PIM with Compute Slices}\kk{TODO: Add figures explaining LISA hop to this}
    \label{fig:membrane_full}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Membrane/Arch_Figures/membrane_h_v.pdf}
    \caption{Membrane PIM with Compute Slices}
    \label{fig:membrane_handv}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[trim=1cm 9.5cm 1cm 8.5cm, clip=true, width=0.5\textwidth]{Membrane/Arch_Figures/Compute_Slices.pdf}
    \caption{Membrane PIM Compute Slices at every Bank}\kk{TODO: to remove this picture}
    \label{fig:membrane_v}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{Membrane/Arch_Figures/membrane_v.pdf}
    \caption{Membrane V}
    \label{fig:membrane_v}
\end{figure}

%\begin{figure*}
%\begin{subfigure}{\linewidth}
%    \centering
%    \includegraphics[width=0.6\textwidth]{Membrane/Arch_Figures/01_bitline_archs-Folded Bitline.pdf}
%    \caption{Compute Slice in Folded Bitline Architecture}
%    \label{fig:membrane_v}
%\end{subfigure}
%\begin{subfigure}{\linewidth}
%    \centering
%    \includegraphics[width=0.6\textwidth]{Membrane/Arch_Figures/01_bitline_archs-Open Bitline.pdf}
%    \caption{Compute Slice in Open Bitline Architecture}
%    \label{fig:membrane_v}
%\end{subfigure}
%\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.55\textwidth]{Membrane/Arch_Figures/01_bitline_combined.pdf}
    \caption{Membrane PIM Compute Slices at every Bank. (Top) Folded Bitline Configuration (Bottom) Open Bitline Configuration}{Akhil - TODO refine this picture}
    \label{fig:membrane_v}
\end{figure*}

==> Membrane/Sections/Discussion.tex <==

% a table listing all Membrane options, pros and cons, categorized by power, area, latency

% potential deployment model, based on their pros and cons, for example, TRA-based Membrane-V can be a drop-in replacement for DRAM, while SRA-based Membrane-V is a specialized processor

==> Membrane/Sections/Future_Directions.tex <==
% Everything is a database approach - side benefits to other applications
% CXL Dissaggregated Memory Architecture

==> Membrane/Sections/Membrane-H_arch.tex <==
{\subsection{\sout{Membrane-H} Membrane Subarray-Level Architecture \underline{[DRAFT]}} \label{sec:Membrane-H}
The overall goal of the Membrane-H architecture is to process the database records in an element-serial bit-parallel fashion. Towards this end, we propose to use "Compute Slices' ' that are logic elements used for processing data situated at the bottom end of a bank. These Compute Slices are connected to the rest of the bank via the existing bitlines and could be envisioned as compute-capable regions of a single DRAM bank. The bitlines essentially act as interfaces to connect the DRAM subarrays storing the data with these compute-capable regions. Adopting this style of Compute Slices provides us with two major benefits -
It helps us to avoid using the Global Data Lines (GDLs) which are shared resources between different banks i.e. it limits only one bank from using them thereby reducing the available parallelism
It provides a wider interface than the GDL between the DRAM subarrays and the compute regions within the bank since there can be 4K - 16K bit-lines running across the bank which helps in the available bandwidth to the compute regions.}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{Membrane/Arch_Figures/membrane_h.pdf}
    \caption{Membrane H}
    \label{fig:membrane_h}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{Membrane/Arch_Figures/membrane_v.pdf}
    \caption{Membrane V}
    \label{fig:membrane_v}
\end{figure}


The overall goal of the Membrane-H architecture is to process the database records in an element-serial bit-parallel fashion. Towards this end, we propose using "Compute Slices," which are logic elements used for processing data situated within a bank. These Compute Slices are connected to the rest of the bank via the existing bitlines and could be envisioned as compute-capable regions of a single DRAM bank. The bitlines act as interfaces to connect the DRAM subarrays storing the data with these compute-capable regions. Adopting this style of Compute Slices provides us with two major benefits - ( i ) it helps us to avoid using shared datapath between different banks that could limit the degree of parallelism (ii) it provides a wider interface than the narrow internal bus between the DRAM subarrays and compute regions within the bank. The internal bus width is only 4, 8, and 16 bits wide while 4K - 16K bitlines are running across the bank, and thus we adopt a mechanism to leverage these bitlines for large data transfers across the bank.

\textbf{Compute Slices.} The purpose of each Compute Slice is to scan the database records at the subarray level and to produce a bitmap to indicate the result of predicate operations. Hence, to support this, each compute slice consists of -

\textbf{1. 64-bit Comparator Units.}  Since we are only concerned with the comparison operations for processing the database records, the ALUs required to perform these are more apt to be called Comparator Units (CUs) rather than full-fledged ALUs. We propose to have eight bit-sliced 8-bit CUs to perform comparison operations on the subarray data. Bit-slicing is a technique of constructing larger word-length processors from smaller bit-length processors. For example, one could construct a 16-bit processor by merging four 4-bit ALUs. In our case, we propose to use eight 8-bit level CUs to construct a single 64-bit CU. The advantages of such a configuration are twofold - ( i ) The current workloads are already adjusted to the 64-bit computing paradigm ( ii ) the input dataset might contain records whose length varies from 8 - 64 bits. Hence, we adopt this configurable bit-sliced setup to support records of varying bit-lengths with single hardware. The Control Unit (discussed later) would issue control signals to operate the Bit-sliced CUs in the desired configuration. The CU is restricted to supporting equality check ( input\_record == a ) or between check ( x < input\_record < y) for database scan operations. Generally, the comparison operations are executed as a subtraction operation, which in itself is executed as a two's complement addition i.e., A - B = A + (~B + 1). Hence, implementing an adder circuit is enough to support a SCAN operation, and adder circuits generally are easily amenable to bit-sliced configurations. These CUs would not support processing string inputs or regex operations as these would be area-prohibitive to fit inside a single bank. Since we already operate on denormalized WideTable, which is dictionary-encoded, hence, the comparator unit would not encounter any strings as they all would be encoded as an integer, which makes them compatible for PIM CUs.

\textbf{2. Walkers.} Maintaining regular layouts in DRAM architectures is preferred to make them amenable to DRAM manufacturing process. Hence, adopting structures that break this regularity, unless necessary, would impose significant area costs. Hence, we propose using walkers, which primarily consist of regular sense amplifiers combined with a column selection mechanism to shift data from the row buffer into the Comparator Units. Walkers also have an advantage in preserving the mat-level interleaving and read/write data according to the same layout. The advantages of walker-access mechanisms were previously explored in {cite Fulcrum}, and we propose to adapt these access mechanisms to feed data into our processing elements. Specifically, we use two walkers, one for storing and reading the database records and another for storing the generated bitmap results. These bitmaps are flushed periodically when the walker-2 gets full.  
3. Control Unit - The Control Unit is responsible for orchestrating the control signals to control the operations of the PIM unit and ensure its synchronization with the DRAM portion of the bank. Its primary functions include - 
	1. Generating control signals for Bit-Sliced ALU to operate in 8, 16, 32, or 64-bit modes. The ALUs combined take in 64-bit input. Hence, if the ALUs are operating in 16-bit mode, then 4-16-bit words are processed together to produce a 4-bit result indicating the result of predicate operation of each word. 
	2. Storing Partial results in internal register file - After processing the records, the bitmap results are stored in an internal register file, which is periodically written back to a specific DRAM address. In this instance, we allocate a 2048-bit register file for our operations as this offers reasonable performance without imposing significant area overhead. 

\mrtn{We've explored -V and -H individually, but can we now discuss them together here?}

\textbf{Modes of Operation.} As Compute Slices operate on entire row buffers, we recommend setting the minimum virtual page size to be equivalent to the size of a row buffer. More detailed information is provided in the System Integration section, discussed later. Previous works such as BLIMP, AxDIMM, and UPMEM have proposed utilizing all the banks for concurrent PIM operations. Aquabolt moves further by implementing different operation modes, distinguishing between single-bank access for conventional load/stores and all-bank access for PIM execution.

We observe the potential to exploit both bank-level and rank-level parallelism simultaneously. In a conventional scenario, datapaths are shared amongst a set of ranks and banks, allowing only one to be active at any given time. However, with Compute Slices, data is processed in situ and never leaves the bank. This enables us to tap into significantly more parallelism by directing PIM execution across all available banks and ranks. We propose an Aquabolt-style Single Bank-All Rank mode (SBAR) and an All-Rank All-Bank (ABAR mode) to achieve this.

In SBAR mode, a page is striped across all available ranks, with a single bank in each rank contributing to a portion of the page. On the other hand, ABAR mode aims to exploit all available parallelism by striping a page across all available ranks and all banks within a rank. In ABAR mode, a page access disregards the rank, bank-group, and bank bits of the memory address and instead considers the row-column bits to activate a specific set of addresses within this large page. In SBAR mode, only the rank bits are ignored, and bank and bank-group bits are considered to activate a specific bank across all the available ranks. Naturally, ABAR provides a higher degree of parallelism than SBAR since many addresses are activated with a single DRAM command. The PIM execution units are operated under one of these modes, and each mode dictates the degree of parallelism available with a single execution step.

\subsection{Membrane Bank-Level Architecture}


==> Membrane/Sections/Membrane-H_old.tex <==
\vspace*{-0.04in}
\subsection{Membrane-H} \label{sec:Membrane-H}

%Drawing inspiration from Fulcrum {\bf CITATION HERE}, where the data is processed in horizontal element-serial bit-parallel manner by a processing element or ALU placed at the edge of a subarray, we decided to utilize similar principle but in the context of database processing. While Fulcrum and its successors such as Gearbox [ TODO Insert Citations here] and Pulley happened to support a larger selection of kernels such as those used in Graph Processing and Machine Learning, they are also suffered from a large hardware overhead. The walkers used to shift and access the data at the subarray level and also support the indirect access mechanism were one of the biggest culprits contributing to the large area overheads. 

%With Membrane, we realized that these features were not necessary and did not make sense in the context of the database workloads. Although removing these hardware features reduces the area overhead considerably, it also restricts the functionality of the PIM device to a specific application. But considering the ubiquitous nature of the database processing workloads in use and the total addressable market for the services exclusively focused on this workload, it made more sense to analyse this trade-off and sacrifice generalization in favour specialization. This PIM device would make more sense in the context of cloud vendors who offered these services and made optimum use of the hardware over the entire device lifetime. 

%Membrane-V has immense parallelism due to its bit-serial element-parallel processing architecture and this lends itself very favourably while filtering large number of database records simultaneously at any given point of time. Also, in order to support the bit-level operations for this architecture, individual logic blocks need to be placed at every bit of the row-buffer. This naturally has a higher area overhead. In contrast, Membrane-H since it works on an element-serial approach need not invest on bit-level logic blocks but on word-level logic blocks, thereby reducing the area overhead significantly. However, taking this approach also leads reduced throughput of Membrane-H when compared to Membrane-V. 

%The Membrane device specifically is a subarray-level PIM device that places a scalar, ALU-like lightweight processing element closer to the row buffer. The ALU itself supports only operations necessary for filtering,  such as the bit-level mask operations and a single comparison instruction, the \emph{between} operation, to check if x < a < y. Since every other comparison can be derived from this, and in the interest of further reducing the area overhead, we wanted to keep the number of instructions it can support to the minimum while at the same time not sacrificing the functionality. 

%The initial designs of Fulcrum required a "walker" to read the row buffer data and feed into the ALU for processing. In fact, Fulcrum used three walkers, comprising two row-wide operands and one row-wide destination operand, that are traversed a word at a time. Having the walker provides benefits, such as  sequential read and write in both directions [Insert Fulcrum citation here] and also  indirect accesses with column-selection  enabled by the walkers [insert gearbox citation here]. However, we observed that scan operations require performing comparison operation only on the data read and do not require any  writing back of data into the row buffer. Also, indirect accesses are another feature not required in the database scan operations. With these observations in mind, we decided to eliminate the walkers entirely and rely on feeding the data from the row buffer to the ALU directly. When a column is selected by the column decoder, the column word of data flows into the ALU for processing. By placing a switch right after the column decoder, we could arbitrate the data flow between allowing the column word of data to either flow to the global data line or to flow into the ALU for further processing. 

%The Processing Element further has an instruction buffer to store and execute the comparison operations one by one. The length of the instruction buffer is set to 4 for evaluation purposes in this work, but the same could be extended to any suitable length. 



%Introduction paragraph
    % The need for maintaining the lean hardware overhead and the sacrifice between the specialization over generalization
    %Drawing inspiration from Fulcrum \cite{fulcrum}, where the data is processed in horizontal bit-parallel, element-serial (i.e., scalar) manner by a processing element or ALU placed at the edge of a subarray, we optimize the architecture for OLAP workloads.



\begin{figure}
    \centering
    \subfloat[Membrane-H Overall Architecture]{
        \includegraphics[width=0.9\linewidth]{Membrane/Arch_Figures/05_Membrane_H_Arch.pdf}
        %\caption{Membrane-H Overall Architecture}
        \label{fig:Membrane-H}
        % \vspace*{1ex}
    }
    \vspace*{1ex}
    \subfloat[Rank Level Processor]{
        \centering
        \includegraphics[width=0.6\columnwidth]{Membrane/Arch_Figures/02_Rank_Level_Processor_v2.pdf}
        %\caption{Rank Level Processor \underline{AK TODO - Resize this }}
        \label{fig:Rank Level Unit Breakdown}    
    }
    \caption{Membrane-H Architecture.}
    \vspace*{-.22in}
\end{figure}
    
    % Data Layout
    %\subsubsection{\textbf{Data Layout}} - 
    % Describe the WideTable entries
    % Dictionary encoding and its 2 benefits
    % Effect of Data Layout
    % How the element-serial nature comes into the picture. 
    % LISA 
    %Records from different tables are pre-joined and dictionary encoded together to form the WideTable entries. These entries are laid down and distributed either in single or amongst multiple subarray rows. The effect of dictionary encoding has two-fold benefits in the context of Membrane-H architecture. Firstly, it reduces the memory footprint of large datasets by encoding repetitive string values to numerical symbols. Secondly, since the entire dataset is in numerical format, performing comparison operations such as equality, greater than, lesser than becomes easier. Membrane-H does not support regex statements since they are more complex operations that might incur a large area penalty when implemented at the subarray-level.  

    %The way in which these WideTable entries are laid out among the subarray rows again has a significant affect on the Membrane-H performance. This is because the number of row activations required to read the required data for performing query execution can be optimized. Row activations also happen to be one of the most expensive memory operations. This is further discussed and evaluated in detail in the section - (TODO fill the name of Evaluation Section here).

    % TODO Should I remove this paragraph? 
    %Either the entire WideTable entry or sections of each entry can be read and operated upon by the PIM processing element placed close to the Row Buffer. After reading out a row, values are fed in an element-serial manner to the ALU. This processing element is  bit-parallel because it operates on full 16-bit words at a time. 

    % Comparison Unit
    %\subsubsection{\textbf{Comparison Unit}}
%    \sout{Since the Membrane architecture is designed for database workloads, the ALU  supports only the operations required by the workload rather than having a fully-featured ALU, to save both on the hardware overhead costs and power costs. SSB, and many database workloads, do not utilize any floating-point fields, using only signed integers, fixed-point values, and string values.}
    %Generally OLAP database workloads such as SSB, TPC-H operate on string values and signed integers rather than floating point values (which can be further encoded using efficient dictionary compression mechanism), so we  implemented a comparison unit supporting only the necessary comparison operations used in the workloads rather than having a fully-featured ALU. This not only results in significant hardware overhead costs but also power savings.  This also enables us to remove all the ``walkers'' from the original Fulcrum design.
    
    %\sout{Since the Membrane PIM hardware executes only the filtering operation of the query execution pipeline, a lightweight ALU unit that supports just two kernels,  bit-masking  (bitwise AND operation to extract bits of importance from the input data) and the \textit{between} operator. The \textit{between} operation checks if 
    %the value \textit{num} is between \textit{x} and \textit{y} i.e. if 
    %$x < num < y$. Every other comparison operation utilized in the database can be expressed in term of this \textit{between} operator. In our current evaluations, the Comparison Unit operates on 16-bit operands, which was chosen based on the cardinality of fields in SSB. %but the same can again be extensible depending on the application requirement.     The length of the operands upon which the Comparison Unit operates on is directly related to the width of the subarray columns. \sout{The PIM memory architecture being considered has subarray columns that are 16 bitlines in width.}
    %The \textit{between} operator is implemented using subtraction, so the ALU supports general integer/fixed-point arithmetic. The chief area savings in Membrane-H relative to Fulcrum come from removing the three Fulcrum Walkers.}
    %Also, removing the walker shifters from the Membrane design yielded considerable area savings. 

    % Bitmap Register
    %\subsubsection{\textbf{Bitmap Register}}
    %A register is needed to hold the intermediate matching results while the query is being processed. The length of the bitmap register depends on the number of database records held in each subarray row. %For example, if there are 100 database records held in a subarray row, then the length of the bitmap needs to be 100 bits long. 
    %Based on SSB workload, we have portioned a 256-bit length bitmap.
    
    %\begin{figure}
    %    \centering
    %    \includegraphics[width=0.3\linewidth]{Membrane/Arch_Figures/Instruction Buffer-Vertical.pdf}
    %    \caption{Membrane-H Instruction Buffer Format}
    %    \label{fig:Membrane-H-format}
    %\end{figure}
    
    % Instruction Buffer
    %\subsubsection{\textbf{Instruction Buffer}}
    %\sout{The Membrane-H processing element needs to perform a small number of comparison operations at different locations in the row, so it is driven by a small instruction buffer. 
    %\sout{The instructions  convey information as to which specific column in the subarray row needs to be accessed and the type of comparison operation that needs to be performed.} 
    %The fields, as shown in Table~\ref{tab:instruction buffer format} %Figure~\ref{fig:Membrane-H-format} 
    %and their operations are: (i) \textbf{Predicate-1} and \textbf{Predicate-2} determine the values to execute the \textit{between} operator i.e. check if $predicate\_1 < input < predicate\_2$ (ii) \textbf{Mask\_Value} is for the bitmask operation i.e. $(mask\_value \ {\&} \ input)$ (iii) \textbf{Record\_Count} is a decrementing counter to track the number of records to be processed in each subarray.  (iv) \textbf{Column\_Offset} indicates which column of row needs to  read. A single database record occupies several subarray columns, so this indicates which specific column to operate upon. (v) \textbf{Column\_Multiplier\_Value} is used to access the next subarray column  to be processed, e.g. to support striding. }
    %Since  Membrane-H needs to perform different comparison operations across different elements within the same row buffer, we introduce a small instruction buffer to indicate which operations to perform. Each instruction stored within this buffer contains the following fields: (i) \textbf{Predicate-1} and \textbf{Predicate-2} determine the values to execute the comparison operation i.e. check if $predicate\_1 < input < predicate\_2$ (ii) \textbf{Mask\_Value}: If two or more fields are tightly packed within an 8-bit of 16-bit value, this value (a bitmask) is used to extract the field of interest; i.e., $(mask\_value \ {\&} \ input)$. Due to the repetitive and structured layout of database fields in the row-buffer, the PE can execute the commands present in the instruction buffer  one after another while the memory controller issues which specific columns to  read and feed into the PE. 
    %Suppose a database attribute \textit{customer\_id} is present in subarray columns-4, 8, 12 etc. Then, by utilizing the \textit{column\_multiplier\_value, column\_offset and record\_count} values, one could target those specific columns to be read and fed into a comparison operation.  
    %
    %\begin{table}[]
    %\centering
    %    \begin{tabular}{ll}
    %    \hline
    %    Field                  & Length (in bits)                              \\ \hline
    %%    Column Offset            & 16 \\
    %    Column Multiplier Value       & 8                            \\
    %    Record Count               & 16                                 \\
    %    Mask Value             & 16                                 \\
    %    Predicate-1             & 16 \\
    %    Predicate-2             & 16 \\\hline
    %    \end{tabular}
    %    \caption{\centering{Membrane-H Instruction Buffer Format}}
    %    \label{tab:instruction buffer format}
    %    \vspace*{-.25in}
    %\end{table}
    %
    %In the SSB workload, a maximum of four comparison operations are  performed for any given query. Hence, a four-entry instruction buffer is used. %Of course, one could extend this to suit the application requirements or also one could reuse the same four-entry instruction buffer in multiple runs to perform more than 4 \textit{between} operations. 
    
    % Control Unit
    %\subsubsection{\textbf{Control Unit}} \label{membrane-H control unit}
    %The Control Unit is responsible for orchestrating the operations within the Membrane-H processing element. %Due to repetitiveness of the data layout and the simple kernel operations that need to be supported, the control unit is quite simple. It only needs to perform tasks such as extracting column addresses to access, iterating over the instruction buffers, decrementing the \textit{Record\_Count} registers, etc. 
    %It performs tasks such as  
    %s\sout{extracting column addresses to access,} 
    %iterating over the instruction buffer and %\sout{decrementing the \textit{Record\_Count} registers} 
    %and updating bitmap registers. %Due to optimized nature of the workload and limited set of features to be supported,
    %\ak{It controls an additional signal \textit{push\_data\_h} that is used in Data Push mode to indicate to the memory controller to read a specific columnar data element that has evaluated to True after a predicate match. } 
    
    %\subsubsection{\textbf{Subarray Groups}}
    % Explain the nature of subarray group
    % Explain LISA
    % Explain the need for LISA
    % Explain the tradeoffs in the context of PIM
    %Based on the hierarchical organization of a DRAM chip, a bank is sub-divided into subarray groupings that share bitlines and sense amplifiers \cite{TieredDRAM}. %Unlike Membrane-V, the Membrane-H processing element is less intrusive; the circuitry is placed below the sense amplifiers. This %would 
    %will incur area overhead due to addition of new PIM circuitry near every set of sense amplifiers. 
    
    %In order to reduce the area overhead of having a Membrane-H processing element at every subarray, we use subarray groups to place the processing element periodically at every 2, 4, or more subarrays and leverage the \textit{LISA} (Low-cost Interlinked Subarrays)\cite{lisa} mechanism to push data from any given subarray to the PIM-capable subarrays, similar to subarray groups in Membrane-V. 
    
    %While the area overhead is reduced in this method, the execution time is bound to increase due to the additional cycles required to shift the data to the PIM-capable subarrays. A detailed evaluation of the same is available in further section - Evaluation (TODO Add reference). 

    %\ak{The Membrane-H design operates in a horizontal bit-parallel element-serial (scalar) manner along the data present in the row buffer by a processing element or an ALU present at the edge of a subarray. This Membrane-H ALU is optimised to perform the scan operation required by the OLAP workload. }

%\ak{The row buffer contents hold the database attributes against which the predicate operation would be performed to produce a resultant bitmap. 
%The number of database attributes that can be packed horizontally within a single row buffer is vastly smaller ompared to the vertically laid out in the V variant. Due to this, there is an oppurtunity to materialize the result of this smaller batch size earlier and hence, the H variant is considered to pursue the strategy of the early materialisation of results. While the database terminology defines the early materialisation to be at the granularity of each database record, we consider it to be at the granularity of the batch size that can fit into a row buffer. }

%\ak{One of the primary motivations of the H variant was to optimise the area overhead and keep it to the minimum. Often times, having a large area overhead of PIM processing elements can either eat into the memory capacity or affect the bit retention in DRAM cells due to thermal dissipation by the large processing elements. Hence, by having a smaller area overhead, we aim to mitigate both the above mentioned problems. We further couple the subarray-level processing element along with a Rank-level processor to ensure that we do not loose significant in-situ processing capabilities while trying to limit the area footprint. The main benefit of a rank-level processor (RLP) is that it could be mounted as a separate chip or logic block as done shown in the AxDIMM and MCN, with very minimal changes to the memory chips present on the DIMM. }

%\begin{figure*}
%\centering
%    \hfill
%    \begin{subfigure}{1\linewidth}
%        \centering
%        \includegraphics[width=\linewidth]{Membrane/Arch_Figures/Rank Interlea‌ving.png}
%        \caption{\textbf{Memory Channel READs performed concurrently across different ranks} In the above diagram, R-0 \& R-3 complete scan, gather and read of a single row buffer worth of contents. While, R-1 \& R-2 need the gather operation to be spread across two consecutive accesses. The diagram also illustrates the pipelining of operations to hide the scan and gather latency.}
        %\caption{In the above diagram, R-0 & R-3 complete scan, gather and read of a single row buffer worth of contents. While, R-1 and R-2 need the gather operation to be spread across two consecutive accesses}
%        \label{fig:WideTable Approach}
%    \end{subfigure}

    
%    \hfill
%    \begin{subfigure}{\linewidth}
%        \centering
%        \includegraphics[width=\linewidth]{Membrane/Sys Integration Figures/03_Membrane_Execution_Flow.pdf}
%        \caption{\textbf{4-stage Execution Pipeline between CPU and Membrane-H PIM architecture}}
%    \label{fig:Membrane_arch_overview}
%    \end{subfigure}
%    \hfill
%    \caption{\textbf{Membrane-H Execution Flow} -- \underline{TODO AK - Resize the diagrams}}
%   \vspace*{-.2in}  
%\end{figure*}

%\begin{figure*}
%\centering
%    \hfill
%    \begin{subfigure}{0.75\linewidth}
%        \centering
%        \includegraphics[width=\linewidth]{Membrane/Arch_Figures/03_Membrane_V_Execution_Flow.pdf}
%        \caption{\textbf{Membrane-V Execution Flow}}
%    \label{fig:Membrane_arch_overview}
%    \end{subfigure}
%    \hfill
%    \caption{\textbf{Membrane-V Execution Flow} -- \underline{TODO AK - Resize the diagrams}}
%   \vspace*{-.2in}
%\end{figure*}

    
%\ak{The main operation of the Membrane-H unit could be broadly be broken down into three phases namely i) Scan Phase - where the database attributes are scanned to produce a bitmap ii) Gather Phase - where the bitmap is processed and gather the necassary data based on its result iii) TX Phase - where the data is read by the Memory Controller and sent to the CPU for performing aggregate operations.}
%\ak{Our early investigation revealed that a single subarray unit performing both Scan and Gather phase results in not only large logic overhead but also increased delay at the subarray level hurting the performance. But by distributing the scan phase to the subarray unit and gather phase to the Rank-level Processor, we significantly improve the performance by optimising each unit for its operation and also open up oppurtunities for pipelining.}

%\ak{Operation of Membrane-H - 
%Our key observation while designing the H variant was the ability to deeply pipeline the overall operation and hide the latencies related to each stage by overlapping the operations performed. 
%We broadly break down the query processing into 5 major phases - 
%i) Scan Phase - relates to scanning the database attribute to produce a resultant bitmap 
%ii) Gather Phase - is concerned with processing the bitmaps and gathering the data required for aggregate processing based on the results of the bitmap.
%iii) Data Push Phase - is concerned with transmitting the data out of the DIMM into the CPU
%iv) DMA Phase - Where Memory Controller inserts data into the CPU caches via a modified DMA/DCA approach and the kernel provides the data to the application
%v) Aggregate Phase - Where the CPU performs the aggregate operations and finally materialise the result for the end user}

The Membrane-H design operates on one word at a time in the row buffer with a processing element (PE) or an ALU present at the edge of a subarray optimised to perform scan operations. The Membrane-H unit  filters the database attributes held within the row buffer and produces a  bitmap, whose length is equal to the number of attributes that can be packed into a single page or row buffer width.  Since entire attributes are checked in each row access, Membrane-H is able to pursue early materialization. While database terminology defines the early materialization to be at the granularity of each database record, we focus on early materialization at the granularity of a row buffer worth of records to align with the access pattern of the PIM architecture. 

%One of the primary motivations of the H variant was to optimize the area overhead and keep it minimum. Often times, large area overhead associated with having capable PEs can either eat into memory capacity or affect the bit retention in DRAM cells due to thermal dissipation by the logic blocks. [TODO cite DRAM errors paper here]. Hence, by consciously limiting the area overhead, we aim to mitigate both the above-mentioned problems. 
We couple subarray-level processing elements with a rank-level unit (RLU) to perform the gather operation necessary to materialize the result. The RLU is placed on the DIMM module, similar to \cite{AxDIMM} and \cite{mcn-dimm}.
%, with minimal changes to the rest of DRAM chips and their capacities. This ensures that we could also limit the area footprint without losing the in-situ low-latency processing capabilities available at the subarray-level unit.
The operation of Membrane-H breaks down into a scan phase performed in parallel across subarrays that produces a  bitmap; and gather phase, performed by the RLU to gather the desired fields from the selected records, based on the bitmap. Our early investigations revealed that a single subarray unit performing both the phases would result in a large logic overhead and increased delay at the subarray-level. With  the RLU, we not only pipeline scan and gather, but also optimize each unit for its respective task.  An advantage of the RLU is that it provides rank-level parallelism, compared to the traditional method of having the CPU or a CPU-side accelerator such as the IAA perform the gather.

\textbf{Subarray-Level Processing Element.} \label{sec:subarray PE} These elements are distributed at the subarrays next to their respective row buffers and consist of a comparison unit to perform the predicate operation and shift logic to feed data in the row buffer, one word at a time, to the PE. OLAP database workloads such as SSB \cite{ssbbenchmark}, TPC-H \cite{tpch}, etc. generally operate on string values and signed integers, and these can be dictionary compressed, so the comparison unit only needs to operate on integers. A bitmap register is allocated to hold the contents of the resultant bitmap after the predicate operation. Based on the analysis from the SSB workload, we allocate a 32-bit bitmap register per subarray. When a query requires more than 32 bits, it could divided into sub-queries and processed sequentially. A Control Unit associated with each PE is responsible for orchestrating the operations and performing tasks such as iterating over attributes, updating bitmap registers, and interfacing with the RLUs. In case of a limitation related to feeding data sequentially off a row buffer due to mat-level barriers within the subarray, we propose to use a row of latches to store the row buffer contents and process the data. We could avoid the large area overhead by conservatively placing these latches for every 4 or 8 subarrays and bringing data to be processed via the LISA \cite{lisa} mechanism. More details are in Section-\ref{sec:results}.

\textbf{Rank-Level Unit (RLU).} \label{sec: RLU description}The primary job of the RLU is to perform the gather operation and interact with the memory controller. It consists of a small programmable core to orchestrate query execution depending on the data layouts used within the subarrays. It also has a bitmap-gather unit where bitmaps are resolved, and address offsets generated to perform a gather operation. These generated addresses are inserted into an internal READ queue. The RLU also pushes the data gathered from the DIMM into the CPU.
%, interfaces with the Memory Controller to perform this operation.
%More details related to this operation are discussed under the System Integration section %(TODO link the section). }
%\hc{\textbf{Direct Cache Access.} \label{sec: DCA description}
%In the Membrane-V variant, the scanning and retrieval of bitmaps were  driven  by the CPU, because the V layout required a separate copy of the database in a conventional, row-major layout in order to read the desired return values without many bitsliced row accesses. In the H variant, the desired values are in conventional, row-major order
%the same may not hold true for the H variant, where data that is selected based on a scan operation needs to be "pushed" from the PIM memory rather than being read out or "pulled" from CPU. Thus, there are significant changes that need to be introduced into the H variant to account for this. 
This process of transferring data to the CPU can be achieved via a mechanism such as  Data Direct I/O (DDIO)~\cite{ddio} that features in most server-class Intel processors, which allows devices external to the CPU, such as network interface cards, to push data directly into the cache~\cite{farshin2020reexamining,packetchasing}. DDIO is built on top of Direct Cache Access (DCA)~\cite{dca} that allows I/O devices to provide prefetch hints to the CPU. Several works such as \cite{dma-cache, understanding-dca, dont-forget-llc-dca} have studied the benefits and optimization techniques related to DCA to seamlessly integrate it with the OS stack to get better performance. These mechanisms can be leveraged in the PIM context for pushing the data from the Membrane-H DIMM to the CPU. This is discussed further in the following section.
%\vspace{-7pt}

% Akhil First Draft on DCA  AKHIL, WHEN YOU ARE DONE DRAFTING THIS, PLEASE MOVE IT TO SECTION 4
%The DCA approach involves using a descriptor table as means of exchanging addresses that the IO devices can be written to within the CPU cache. Once an IO device performs a write, it is indicates to the CPU by an interrupt mechanism or busy-polling. The CPU in turn updates the descriptor table to recieve the next READ request while processing the currently READ data. 
%We could leverage this mechanism in the context of Membrane, where the memory controller mimics an IO device pushing data from the PIM memory to the CPU. \cite{mcn-dimm} has demonstrated to utilise this approach in the context of Rank-level PIM implementations. Due to the predictable periodic intervals of transmission from PIM, any overhead suffered from the mechanism is hidden by simultaneously receiving the next cache line of data while buffering and transmitting the previous cache lines in a pipelined fashion.
%\ak{Memory Channel Network (MCN) \cite{mcn-dimm} is one such prior work that proposes transparent offloading of computation and retrieval of data from PIM memory by making modifications to the network subsystem to support DCA. Our system integration builds on this mechanism to interface with Membrane-H and "push" data in periodic intervals to the CPU caches. Due to the predictable periodic intervals of transmission from PIM, any overhead suffered from the mechanism is hidden by simultaneously receiving the next cache line of data while buffering and transmitting the previous cache lines in a pipelined fashion.}

%\sout{\ak{\textbf{Pipelining Data Retrievals.} Another observation is that memory is generally organized into channels, DIMMs and ranks. While the channels are independent and can be accessed in parallel, the DIMM and ranks within each channel share the same data and address buses and hence, need to be accessed in a concurrent manner. Our key idea here is that while the memory controller performs an access on a certain DIMM/rank, $\ks{cache line???}$ the addresses for next cacheline of data to be pushed to the CPU can be kept ready by the RLP/subarray units in other DIMMs/ranks executing a scan and gather operation. By pipelining the accesses between several ranks and DIMMs, the memory bus is always kept busy and at the same time hiding the latency of other scan/gather operations. }}
%\ak{Deleting paragraph related to Pipelining Data Retrievals since we speak about this in System Integration section in detail}



==> Membrane/Sections/Membrane_Arch_Combined.tex <==
\section{Architecture}
Our proposed {\em Membrane} family of architectures are optimized solely for accelerating the Filter stage of query processing, since that requires by far the most time on a CPU-only implementation and is entirely memory bound.  The Filter stage produces a bitmap; for PIM, this is stored back into the memory. This bitmap is then read by the CPU to perform other parts of the query execution. We have detailed various aspects of Membrane's architecture in the following subsections below.

\textbf{Compute Slice.} A Compute Slice (CS) is the processing element (PE) of the Membrane family of architectures. These Compute Slices can be adapted for use at different layers of the DRAM hierarchy --- subarray-level, bank-level, or rank-level as shown in Figure~\ref{fig:membrane_dse}. Although the Compute Slice design varies slightly depending on where it is placed, it generally consists of a Comparator Unit (CU) discussed below, some temporary buffer space to store the bitmaps, and a simple control unit to orchestrate the operations. A high-level overview of a Compute Slice at the subarray level is shown in Figure~\ref{fig:membrane_subarray_level}. 
\textbf{Comparator unit (CU).}
The heart of all versions of Membrane is the \textit{Comparator Unit}, a {\em scalar} unit that can support both equality check (input\_record == a) and range check (x < input\_record < y) on integer or fixed-point values. Each comparison produces a result bit that is and-ed into the bitmap, which is stored in a local {\em bitmap buffer}, or in a row-buffer-like structure called a {\em walker} \cite{fulcrum} --- see below.  When performing a sequence of filtering steps, the CU reads the current value of the bitvector for the current position, and ANDs this with the result from the new comparison.  In this way the bitvector accumulates the final Boolean result. 

Range checks are implemented using subtraction.  The CU is a scalar unit, supporting operands up to the width of the DRAM global bit lines, i.e. the DRAM device width (e.g., 16 bits).  The CU does not support processing string inputs or regex operations, as these are infrequent and area-prohibitive for PIM implementation. In any case, since we  operate on the denormalized WideTable, which is dictionary-encoded, the comparator unit would not encounter any strings as they are all encoded as integers, making them compatible for PIM CUs. A high-level breakdown of the Comparator Unit (CU) is represented in Figure~\ref{fig:membrane_subarray_level}.

To support data fields that are wider than the burst width (e.g., x8), the CUs are 64 bits, and inputs are read in a bit-sliced, in the sense that they read their inputs in bursts.  For example, reading a 64-bit input in a x8 chip requires 8 reads to assemble the input.  If the database column being processed is less than 64 bits wide, the CU can process multiple values; e.g., the 64-bit input can be made of four 16-bit values and produce 4 output bits in one step.  The advantage of this approach is that  the input dataset may contain records with varying lengths from 8 to 64 bits, and the CU can support this while maintaining full utilization. The Control Unit (discussed later) issues control signals to operate the  CUs in the desired configuration.
%We now describe how the CU is incorporated into each layer of the memory hierarchy. We start with the bank level, because our results show this to provide the best balance of performance and low area overhead.

\textbf{Bitmap buffer.} At the bank and rank level, the CU contains a bitmap of \ks{SIZE} bits. When it is full, it is written back, one burst at a time. At the subarray level, the Compute Slices use a Walker, which the Control Unit flushes when it fills up.

\textbf{Walkers.} Not all subarrays have Compute Slices, so we need a way to move a row buffer worth of data to be processed from any subarray in the bank to its nearest Compute Slice. Each Compute Slice also needs a bitmap buffer. Each Compute Slice therefore consists of two Walkers, inspired by Fulcrum~\cite{fulcrum}, as shown in Figure~\ref{fig:membrane_subarray_level}. Each is implemented as a row buffer to integrate with LISA data movement (discussed next). The first walker, which holds database columns, is accessed using conventional column addressing.  The second walker, which holds the bitmap buffer, supports circular shift. Walkers preserve the mat-level interleaving and perform read/write operations according to the existing data layout.   

\textbf{Subarray-level LISA copy mechanism.} Accessing data from bank level and rank-level is relatively easy and straightforward, as the data is available using conventional DRAM read/write, regardless of its location within a bank or rank. However, when it comes to subarray-level techniques, the GDL is too narrow to effectively leverage subarray-level parallelism. To address this, we propose using LISA~\cite{lisa} to facilitate a quick, low-latency row copy mechanism between different subarrays. \textcolor{red}{NEED TO DESCRIBE HOW IT WORKS HERE.} \kk{The inter-subarray data movement is enabled by linking adjacent subarrays' bitlines together with isolation transistors shown by green triangles in Figure~\ref{fig:membrane_subarray_level}. This facilitates the charge sharing and sensing the bitline voltages between neighbouring subarrays. The LISA links are activated with RBM (row buffer management) DRAM operation.}

The \textbf{Control Unit} is responsible for coordinating the control signals to manage the operations of the PIM unit and ensure that it is synchronized with the DRAM portion of the bank. Its primary function is to generating control signals for the bit-sliced CUs to operate in 8, 16, 32, or 64-bit modes, orchestrating the comparison operations within the Compute Slice, and writing the result bitmap back when the bitmap buffer is full. 

\textbf{Interleaving} poses a problem for performing PIM on words larger than the native burst size, because neighboring bytes are in different DRAM chips.
%is a major bottleneck to implementing PIM-capable operations because the data layout and placement are important concerns when executing PIM operations. \ak{Probably can cut this future line in case of space shortage} As mentioned earlier a single DRAM rank consists of several DRAM chips connected to form a 64-bit interface. To transfer data in 64-bit chunks, the data is divided into smaller pieces and evenly distributed amongst the DRAM chips. For example, in an x8 DRAM configuration, there are 8 chips with each chip providing 8 bits to service a 64-bit data transfer request. This data layout can be problematic for PIM computations because the entire 64-bit word is not contiguous spatially in a single chip but instead broken down into smaller pieces (8 bits in the previous example) and spread across multiple chips. As a result, any processing element (PE) residing within the DRAM chip would only have access to its local portion of the data and not the portion outside it.
This  can be addressed in several ways. The Compute Slices could produce partial results by processing the local data available, even though these are not full words. Later, these partial results are combined to form a single representative result, but this becomes challenging for range queries. One could simply change the interleaving so that entire words are kept together, but without other changes, this makes traditional load/store inefficient, because cache-line fetch can no longer leverage the full bandwidth of the rank. Our solution is therefore to modify the address interleaving so that full words are kept together; i.e., interleaving is now at 64 bits rather than the burst width. We simply need to add a {\em De-interleaving Unit (DU)} with a cache-line-wide buffer that resides in the memory controller to assemble the cache line being read, or to feed the appropriate bytes for a read. Now a rank wide read or write fetches or writes the appropriate chunk (e.g., a byte for x8) of each word in the cache line. For example, the first read for a cache line would get the 0th byte of each word, the next read would get the 1st byte, then the 2nd byte, and so on.  In this way a cache line access takes the same amount of time.

In the subsections below, we discuss the architecture implementation features of implementing Compute Slices at different levels of DRAM hierarchy to perform a design space exploration within these levels as illustrated in Figure~\ref{fig:membrane_dse}.

\textbf{Subarray-level.} Subarray-level PIM  presents several design space parameters . We evaluated the following parameters under the subarray-level: ( i ) Scalar vs. Vector PE - Due to the massive internal bandwidth available at the Row Buffer level, one could either consider a scalar processing element being fed with the a single word at a time or a series of processing elements connected directly to the row-buffer that can execute the comparison operations in single execution cycle. 
(ii) - Data Placement - We could assume just one Compute Slice placed per bank or a Compute Slice placed at each of the subarrays. In the former case, since we are using LISA  rather than going through the narrow bus interface to bring the data to reach the Compute Slice (CS), it introduces a non-uniform access phenomenon between the subarrays and the CS. The subarray farthest from the Compute Slice needs more LISA hops (and thus more time) to get its data to the Compute Slice's walker. There is possibility that the input data might either follow the most pessimistic data placement policy or the optimistic data placement policy which directly affects the performance since more time would be spent on LISA hops in the former scenario. 
(iii) Subarray-level Parallelism - As mentioned earlier, we could have multiple Compute Slices per bank that could be activated in parallel to accelerate the SCAN performance. 


\textbf{Bank-Level Configuration} Bank-level is the second hierarchical level within the DRAM we aimed to explore by infusing with Compute Slices to assess the query execution performance. 

Previous works such as BLIMP \cite{blimp}, and UPMEM \cite{upmem} proposed using all the banks in parallel for concurrent PIM operations. Aquabolt-XL \cite{aquabolt-xl} makes further advancements by supporting different operation modes of operation which distinguish between single-bank access for conventional load/stores and all-bank accesses for PIM execution.  \ks{Briefly mention how these architectures handle interleaving.} \ak{(AK: Done)} \ak{Both Aquabolt-XL \cite{aquabolt-xl} and UPMEM require the data to be placed in a way such that a single word resides completely within a bank without being striped across differnt chips or other parts of a bank. They propose to have software libraries which take care of this interleaving mechanism to achieve the necessary data placement amenable for PIM computations.}  

We adapt the prior idea of accessing all banks for PIM execution from Aquabolt and explore both single-bank (SB) and all-bank (AB) modes of operation for PIM. In both cases, Membrane operates on a {\em PIM page} --- a multiple of virtual-memory superpages (see Section~\ref{sec:system integration}) which is spread across all channels, ranks, and banks, according to the conventional address interleaving. In SB mode, a single PIM operation can only operate on one bank per DRAM chip, although there is still parallelism across all the chips within each rank and across all ranks and channels. To process the full PIM page requires performing the PIM operation in bank 0, then bank 1, and so on. In AB mode, every bank is activated simultaneously. (Unlike in Aquabolt, there is no need to process even and odd banks separately.) This ignores the bank group and bank bits of the memory address and instead reads the same row position in every bank. \ak{We evaluate SB and AB modes for both bank-level and subarray-level PIM configuration since these DRAM heirarchies can support both these modes of operation. In SB mode, the CU sits at the I/O interface feeding off the data arriving on the global bitlines. Also, irrespective of the mode of operation, effectively the PIM commands are executed at every tCCD\_S interval. }
%To exploit both bank-level and rank-level parallelism simultaneously, Compute Slices process data in situ within the banks or subarrays, and avoids using the common datapath which is a common source of contention that limits the number of subarray, banks, ranks that can be used simultanesouly . This enables us to tap into significantly more parallelism by directing PIM execution across all the available banks. We propose two operation modes similar to Aquabolt viz. Single Bank (SB) mode and All-Bank (AB) mode.

\textbf{Rank-level.} Introducing compute elements at the rank-level is much easier from a manufacturing perspective since it can be mounted as a separate logic chip which can interface with the DRAM chips through a small buffer chip. The interfacing with the CPU and with the DRAM can follow that of Samsung's  AxDIMM \cite{AxDIMM} design. 
%A Compute Slice at the rank level would have access to relatively large amount of data to address within its local space and could support more complex operations other than comparison operations. 
However, the amount of parallelism available at the rank level is lower than the AB modes.  Rank-level actually provides the same performance as SB bank-level; both operate on one logical, rank-wide bank at a time.

%reads a value a page is striped across all the available ranks, with a single bank in each rank contributing to a portion of the page. On the other hand, AB mode aims to exploit all available parallelism by striping a page across all available ranks and all banks within a rank. In AB mode, a page access disregards the bank-group, and bank bits of the memory address and instead considers the row-column bits to activate a specific set of addresses within this large page. 

%AB mode provides a higher degree of parallelism than SB mode since many addresses are activated with a single DRAM command. The PIM execution units operate under one of these modes, and each mode dictates the degree of parallelism available with a single execution step.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{Membrane/Arch_Figures/membrane_subarray.pdf}
    \caption{Membrane Compute Slice integration at subarray-level}
    \label{fig:membrane_subarray_level}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.35\textwidth]{Membrane/Arch_Figures/membrane_bank.pdf}
    \caption{Membrane Compute Slice integration at bank-level in AB Mode}
    \label{fig:membrane_bank_level}
\end{figure}

%\ks{Need to fix this up and integrate with the text above.}
%\textbf{1. Comparator Units (CUs).} We propose using eight bit-sliced 8-bit Comparator Units (CUs) to perform comparison operations on subarray data for database record processing. Bit-slicing is a technique that constructs larger word-length processors from smaller bit-length processors. Our configuration combines eight 8-bit level CUs to build a single 64-bit CU. There are two advantages to this setup: 1) current workloads are already adjusted to the 64-bit computing paradigm, and 2) the input dataset may contain records with varying lengths from 8 to 64 bits. This configurable bit-sliced setup can support records of varying bit-lengths with a single hardware, and the Control Unit (discussed later) would issue control signals to operate the Bit-sliced CUs in the desired configuration. 
%The CU can support equality check (input\_record == a) or between check (x < input\_record < y) for database scan operations. Generally, comparison operations are executed as a subtraction operation, which in itself is executed as a two's complement addition, i.e., A - B = A + (~B + 1). Implementing an adder circuit is capable of supporting a SCAN operation, and we observe that adder circuits are easily amenable to bit-sliced configurations. However, these CUs do not support processing string inputs or regex operations as they would be area-prohibitive to fit inside a single bank. 


%\textbf{4. Modes of operation.} are an important aspect of Compute Slices. As these operate on entire row buffers, it is recommended to set the minimum virtual page size equivalent to the size of a row buffer. More detailed information on this can be found in the System Integration section (TODO link it), which is discussed later.

% \ks{LISA belongs in the Arch section}


==> Membrane/Sections/Motivation.tex <==
% motivation and key ideas %
% (1-1.5 pages)

% analytical query processing creates data movement due to table joins on the fly
% naively implementing query processing with PIM is suboptimal
    % sw/hw codesign --> modify the OLAP algorithm --> pre-join/join offline
    % Why doing JOINs on PIM is suboptimal and very bad at subarray level 
    % Akhil has several experiments
        % PIM has parallelism that JOINs cant take advantage of
        % Justify
    % PIM only focuses on filtering --> aggregation is difficult to support in PIM. supporting arithmetic is costly in PIM -> we might expand this depending on overhead
    % bring the arch intro here
    % 2-3% is spent on aggregation ... breakdown of the query
    % leverage the wide table approach
        % advantages -> side-stepping table joins -> 
        % it's acceptable for analytical query processing --> operate on historical data
        % data explosion concern -> dictionary encoding -> comparable to 
        % how does dictionary encoding work

        % Design Goals - Given that our main goal was to accelerate the query processing particularly, we wanted to aim for a PIM architecture that is very optimized to handle this specific application only. This not only allows us to ensure the least possible hardware overhead but also ensures a more coherent software-hardware architecture that is codesigned to make complete utilization of the available resources. Oftentimes having large hardware overheads in PIM designs leads to reduced clock speeds to make sure one does not breach the thermal constraints associated with the design. Adversely reduced clock speeds of the PIM architecture also lead to decreased performance of the architecture, which can be quite significant considering that the baseline comparison, i.e., CPU has clock speeds in the range of a few GHz while the memory is usually in the range of a few MHz. Hence, maintaining a very lean architecture super optimized for database application allows us to deliver the best possible performance and also ensure the design is quite manufacturable due to significantly reduced logic being added to the DRAM designs. 

% why co-processing with CPU
    % not replace the CPU
    % able to keep PIM low-cost and lean

\section{Motivation and Key Ideas - OLD}
    
In this section, we introduce the database workload and the gap between the workload requirements and the architectural capabilities offered by PIM or Near Data technologies.

{\bf NEED A FIGURE TO ILLUSTRATE THESE CONCEPTS}

An OLAP database typically consists of \emph{fact} tables and \emph{dimension} tables. Fact tables contain records that are of some importance to business intelligence, and dimension tables contain additional attributes that describe these records. For example, the database shown in Figure \ref{fig:olap-schema} contains an order fact table, which includes a record for each order submitted to a company. Each order record stores information about the order, including its price, discount, and quantity. The database also contains several dimension tables that each describe a different dimension of the order, such as the date the order was placed, the product that was ordered, the customer that submitted the order, and the supplier that fulfilled the order. Typical OLAP queries involve "slicing and dicing" the data along these dimensions and then aggregating the results. For example, using the SQL shown in Figure \ref{fig:olap-query}, one could ask what product categories are most popular among customers in their 20s. Further queries could be used to "drill down" into additional dimensions of the orders, such as the regions from which they were fulfilled or the months on which they were placed.. 

Database workloads in general tend to have a low computational intensity per byte of memory accessed, since many of the operations being conducted on the data are either simple comparison operations or simple arithmetic operations, such as summing, group by, order by, being performed on the filtered data in the aggregation step of the query processing. Table JOINs in particular involve comparing a set of foreign keys and primary keys from two different tables and combining the row contents associated with those keys when a match occurs. While implementing this JOIN operation one could either perform naïve table scan of foreign keys for a every primary key or alternatively scan every foreign key for a given primary key; both the approaches would involve a lot of sequential accesses to the memory. The scans could be replaced by hash lookups to make the task easier, which will end up generating a lot of random accesses to the memory. Theses are the conventional steps steps employed by the algorithms in the CPU paradigm. Of course various optimizations and several alternative mechanisms are being researched but the overall nature of table JOINs remain the same. 

When trying to implement the same JOIN operation on a PIM architecture, things are much more difficult. First, while the CPU can address the entire memory, the processing elements within the PIM can only address a few megabytes if they are implemented at the sub-array level and a few hundreds of megabytes if they are at a bank-level. Hence, if the dataset tends to be large, then the processing element needs to always reach outside its addressable memory space when probing a particular memory address. This is expensive, since data needs to be fetched from elsewhere, often via narrow data paths, and obviates some of the potential efficiency compared to 
CPUs. 
% Cutting this text becasue I think it's obvious /K
%The situation is much more aggravated at the subarray-level while it is relatively less so at the rank or channel level PIM designs since they tend to have larger addressable space. 
%Thus, for every foreign key or primary key probe a subarray-level PIM element is performing expensive memory reads outside its addressable space and if there happens to be millions of such lookups that need to be performed, this might either lead performance degradation or marginal performance improvements over the CPU. 

{\bf FIXME - this paragraph is clunky, maybe unnecessary - I would cut it drastically and merge it with the preceding paragraph. /K}
Second, considering the DRAM hierarchy, the data movement within the same region such as rank, bank, or subarray, will be relatively cheaper than the movement among different ranks, banks, or subarrays respectively.
%Again, at the subarray-level too, the problem is magnified as often for every foreign key or unique lookup, data needs to travel from other subarrays. 
Other works such as LISA (TODO citation needed) have been proposed that provide inexpensive inter-subarray movements. But these still take up more cycles depending on how far the data must travel from the source subarray to the destination subarray. The problem might be less so, when the PIM architecture is implemented at the bank or rank-level. However, one looses the degree of parallelism when implemented at the bank or rank level. 

Consider the SSB dataset with scale factor-100, which has a memory footprint of 60 GB and has around 600 million records approximately in its fact table. During all the queries, the fact table needs to be joined with the four other smaller dimension tables. These dimension tables range in size from a few hundred kilobytes for a few thousand records, to hundreds of megabytes for millions of records. Thus, realistically, for every table join even between the fact table and a dimension T=table, we are looking at 600+ million expensive lookups. The cost of course increases with the number of dimension tables

Thus, while implementing the above workload on PIM has two potential bottlenecks.  
First, in the absence of an efficient lookup mechanism utilizing low area overhead, the performance is bound to degrade seriously compared to the CPU. {\bf THIS IS TOO VAGUE. BE SPECIFIC ABOUT WHY}

{\bf THIS IS ALSO VAGUE. WHY IS THIS A POTENTIAL BOTTLENECK }Secondly, even when efficient lookup mechanisms are implemented, the memory regions holding the dimension tables are bombarded with 600+ million memory access request from the Fact Table. This can end up becoming a potential bottleneck while servicing all the requests crimping the performance again when compared to the CPU. Ofcourse, alternatively one could probe the Fact Table for given values in the Dimension Table to reduce the number of lookups drastically but that also involves looking across several memory regions simultaneously for each lookup since the Fact Table is of size 60 GB in itself. 

Hence, the JOIN operations implemented on PIM architecture necessarily do not take complete advantage of the massive parallelism and immense bandwidth afforded by the hardware. {\bf THIS DOES NOT FOLLOW FROM THE PRECEDING.} This realization lead us to investigate WideTable (TODO citation) which avoided the JOIN operations entirely by pre-joining it offline. By eliminating the JOINs entirely, every query is reduced to filtering operation over the entire WideTable. And filtering is able to effectively utilize the parallelism and bandwidth offered by the PIM hardware effectively. Hence, this inspired our work to rethink the way in which database operations are mapped to the PIM architecture and co-design the PIM hardware and the query execution software together for maximum speedup. {\bf EXPLAIN HOW}. We analyzed the query execution pipeline and implemented parts such as the filtering operations on the PIM hardware while other aggregate operations are 

Thirdly, even after eliminating JOINs, aggregation operations such as group by, sorting, etc on the filtered data are one of the  final steps, which again necessarily do not completely benefit from the PIM capabilities. One could add these capabilities to the PIM but doing so might not be the best course of action for two reasons namely, that these filtered data anyway needs to travel to the CPU for materializing the result to the user and the CPU with its large cache is already very good at performing these group by and sorting operations. Hence, rather than PIM trying to replace the CPU over the entire query execution pipeline, our design allows us to offload parts of the pipeline that best take advantage of the architectural benefits offered both by the CPU and PIM and cooperatively process the query together. 

One of the major benefits from this approach is the very low area overhead in PIM memory since it only happens to support the filtering kernel while rest other operations are executed on the CPU. By having low area overhead brings three-fold advantages, namely, maintaining near native DDR clock speeds, not sacrificing memory capacity and acting as a drop-in replacement for conventional memory. Due to thermal constraints, large area overheads in PIM sometimes translate to reduced clock speeds as seen in prior works (cite Fulcrum and Gearbox) and reduced clock speeds also greatly diminish the PIM performance. We have also observed in other designs (such as HBM-PIM) where large area overheads also eats into the memory capacity which might be very expensive in terms of datacentre economics. Also by having low-area overhead, we could propose the PIM memory as a drop-in replacement for conventional memory which happens to be slightly more intelligent and capable of performing filtering operations rather than replacing the CPU for end-to-end tasks. 

==> Membrane/Sections/Motivation_2.tex <==
% motivation and key ideas %
% (1-1.5 pages)

% analytical query processing creates data movement due to table joins on the fly
% naively implementing query processing with PIM is suboptimal
    % sw/hw codesign --> modify the OLAP algorithm --> pre-join/join offline
    % Why doing JOINs on PIM is suboptimal and very bad at subarray level 
    % Akhil has several experiments
        % PIM has parallelism that JOINs cant take advantage of
        % Justify
    % PIM only focuses on filtering --> aggregation is difficult to support in PIM. supporting arithmetic is costly in PIM -> we might expand this depending on overhead
    % bring the arch intro here
    % 2-3% is spent on aggregation ... breakdown of the query
    % leverage the wide table approach
        % advantages -> side-stepping table joins -> 
        % it's acceptable for analytical query processing --> operate on historical data
        % data explosion concern -> dictionary encoding -> comparable to 
        % how does dictionary encoding work

        % Design Goals - Given that our main goal was to accelerate the query processing particularly, we wanted to aim for a PIM architecture that is very optimized to handle this specific application only. This not only allows us to ensure the least possible hardware overhead but also ensures a more coherent software-hardware architecture that is codesigned to make complete utilization of the available resources. Oftentimes having large hardware overheads in PIM designs leads to reduced clock speeds to make sure one does not breach the thermal constraints associated with the design. Adversely reduced clock speeds of the PIM architecture also lead to decreased performance of the architecture, which can be quite significant considering that the baseline comparison, i.e., CPU has clock speeds in the range of a few GHz while the memory is usually in the range of a few MHz. Hence, maintaining a very lean architecture super optimized for database application allows us to deliver the best possible performance and also ensure the design is quite manufacturable due to significantly reduced logic being added to the DRAM designs. 

% why co-processing with CPU
    % not replace the CPU
    % able to keep PIM low-cost and lean
    
    
% Focus Points
% DRAM Overhead Concerns
% Tradeoffs of Different Sieve Designs
% Novel Data Layout and pattern matching
% The Motivation for early termination

% Focus Points Here
% 1. OLAP workloads do not change - Usage of WideTables
% 2. CPU is already good at Database Processing - Don't replace it
% 3. PIM is proven to be very good at filtering operations
% 4. Hence make best use of both in key parts of the database execution pipeline
% 5. Two Modes - Expected Benefits
\section{Key Ideas}
%\textcolor{blue}{proposed rewrite}
%\begin{itemize}
%\color{blue}
%  \item Motivation: Data Analytics (replaces current section)
%  \begin{itemize}
%      \item Massive data volume.
%      \item Data warehousing as a solution.
%      \item Read-mostly environment.
%      \item Existing optimizations for warehoused data (WideTable, etc.).
%      \item Hardware acceleration in data warehouses.
%  \end{itemize}
%  \item Cooperative Processing (new)
%  \begin{itemize}
%      \item Denormalized data has two main steps: Filter and Aggregate
%      \item Filters and Aggregations are handled differently by PIM and CPU.
%      \item Filtering:
%      \begin{itemize}
%          \item Massive parallelism exposed by PIM allows for high speed filtering.
%          \item CPU must transfer all data from memory to cache to perform a filtering operation. Inherently disadvantaged.
%      \end{itemize}
%      \item Aggregations:
%      \begin{itemize}
%          \item CPU is easily able to maintain a hashmap for each group by key. These maps usually fit into cache, which is shared by all cores.
%          \item PIM does not have a global working space, which complicates the creation of large hash maps.
%      \end{itemize}
%      \item Both components are necessary for modern analytical queries. Cooperation of PIM and CPU allows for the ``best of both worlds.''
%  \end{itemize}
%\end{itemize}
\textbf{OLAP Workloads}
\jmp{Should we axe this entire next para? Since we clearly scope the paper to OLAP, we may not need this para?}
Many OLAP workloads are characterized by their emphasis on analyzing historical data, as compared to Online Transaction Processing (OLTP) workloads that generally facilitate business transactions~\cite{OLAPvsOLTP}.
The differences between OLAP and OLTP workloads have driven specialization in database platforms, where analytical and transactional query processing are regularly performed by two separate database solutions.
In many cases, the archived data is stored as a read-mostly, append-only database, commonly referred to as a data warehouse~\cite{Chaudhuri1997} and the transactional database stores the latest copy of the key tables in the database. For example, in an e-commerce application, information about current orders is part of a transactional database, and the history of all orders is part of the warehouse database used for OLAP queries. The transactional database is usually smaller in size and the data warehouse is much larger, as it keeps track of all the transactions over time.

\ks{I'm suggesting we cut this entire section. I do like the above paragraph though, for the edification of architects, and will move it into Sec II}

In the data warehouse environment, updates to the data are usually performed in large batches by creating a snapshot of the transaction-focused database.
Loading data into a warehouse allows for a number of optimizations that may not be suitable in a live transactional environment.
Of these optimizations, we emphasize the WideTable~\cite{widetable} technique. \ks{Why is this not suitable for transactional? Also, can we say anything about whether these systems are dedicated for analytical? Overall this phrasing is awkward - implying a bunch of optimizations that we ignore.} 
% [Redundant] Broadly, this technique significantly reduces the complexity of OLAP queries by storing pre-joined tables using a process known as denormalization.
This significantly improves the performance of OLAP workloads, due to the removal of expensive join operators during query execution.
This comes at a cost of increasing the size of the database, but we find that careful encoding limits the size increase to 18-22\%. \ks{All this is redundant}
%This places further strain on the underlying memory subsystem, exacerbating the existing challenges that drive the adoption of PIM in a database setting, as shown in the preceding section.
%\textcolor{teal}{mp: reference memory bound figure}.

%Compared to Online Transaction Processing (OLTP), which tends to be more update-centric,  Online Analytical Processing (OLAP)  tends to be more query-centric i.e. the updates are more infrequent. The main goal behind the optimization of  OLAP  is fast browsing, aggregation, and analysis of massive datasets \cite{OLAPvsOLTP}. Since the design goals for optimization of OLAP and OLTP  are in conflict with one another, it is difficult to arrive at an architecture design that can optimize both without degrading the other \cite{onesizefitsall}. Hence, the scope of this work is to focus on and accelerate the OLAP database workloads.
%\av{Could be cut for space.} \ks{I actually think this paragraph is quite helpful, but this paragraph would benefit from an extra sentence about how large the market is and why this one application is worth specialized hardware.}

% Akhil Notes
% On the CPU, the JOIN oeprations massively favour the cache locality and accesses
% Hence, the algorithms are tweaked accordingly to favour these large caches on the CPU. 
% These algorithms massively contribute to the overall speedup and execution. 
% However, these algorithms are not directly translatable to the PIM hardware, since the PIM memory has either limted or no cache at all. 
% In the absence of optimized algorithms, one needs to perform the naive JOIN plans in the hope that PIM's increased parallelism and bandwidth come to the rescue. 

%\textbf{Nature of the JOIN operations}
%A JOIN operation involves combining two or more tables based on the foreign and primary key attributes that establish the relationship  between these tables. Na\"ively, in order to perform a JOIN operation, one could either look for a primary key, given set of foreign keys (many-to-one relationship) or perform a lookup for a set of foreign keys given a primary key (one-to-many relationship). When a match occurs, the set of record contents from both tables are combined together to form a new table. There are various optimizations such as scans, hash lookups (Akhil-cite), and optimized query execution (Akhil-cite) plans that dictate how a JOIN operation is performed on the CPU. Many  of these optimizations, especially the hash lookups, bloom filters, etc., try to take maximum advantage of the locality benefits offered by the CPU caches. These techniques, combined with aggressive prefetching and column-store techniques (which boost spatial locality) result in significant speedups in performing the JOIN operations with the CPUs. 

%However, the PIM architectures either have limited amounts of or no cache memory available to their processing elements to take advantage of similar techniques. 
%Hence, na\"ive implementation of these algorithms to PIM architecture either results in marginal speedup or even performance degradation due to the architectural differences.
%Furthermore, the CPU can address the entire memory to perform a table lookup or scan operation while the processing elements implemented for PIM can address only few megabytes at the subarray-level and few hundreds of megabytes at the bank- or rank-level. For massive datasets that exceed these sizes, data needs to travel through narrow bus interfaces to reach PIM elements present in other regions of the memory. These narrow buses can act as bottlenecks to performance in the absence of clever partitioning schemes that minimize such cross-region accesses between different PIM elements.  \ks{Why can't we just do clever partitioning and avoid the need for PIM?}

%Consider the SSB dataset with scale factor-100, which has approximately 600 million records in its main \textit{Fact Table} and occupies a memory footprint of 40-60 GB (depending on the encoding scheme used). The dimension tables range in size from a few hundred kilobytes to hundreds of megabytes storing between hundreds to thousands of records themselves. During table join operation, foreign keys present in the \textit{Fact Table} are matched against the Unique keys in the \textit{Dimension Table}. Thus, realistically, for every table join between the fact table and a dimension table, we are looking at 600+ million expensive lookups and large data movements across narrow interfaces between different PIM regions. In the absence of temporal and spatial locality benefits offered by caches, and without a capable communication interface between the PIM processing elements, the JOIN operations tend to either offer smaller improvements or deterioration in performance against the CPU.

%\ks{I think we could cut the above a lot. I don't think most of the above information is needed to justify WideTable, which is what all this leads up to.}



\textbf{Filtering Operations On PIM Architecture}
As joins have been preprocessed out of the OLAP workload through the usage of denormalized tables, OLAP queries on data stored in WideTables are primarily focused on filtering and aggregating data.
Several past works (Akhil-cite) have indicated that filtering and scanning operation on PIM favorably leverage the massive parallelism and bandwidth afforded by the nature of this architecture. 
% Cut - not relevant:
%Generally, the effect of indirect accesses or random access patterns can be alleviated with presence of caches and prefetching. But due to the absence of these expensive capabilities at the PIM level, these type of accesses tend to significantly degrade the PIM performance. However, filtering and scanning operations 
%because they follow a streaming access pattern that can leverage the massive parallelism in PIM architectures, including bank-level, subarray-level, and row-level parallelism.
%is PIM-friendly by nature and thus, these kernels get accelerated massively by the PIM architecture.

%\textbf{WideTable}
%With the above three key insights that OLAP database workloads are infrequently updated, the JOIN operations tend to be expensive on PIM and filtering operations can be accelerated massively by the same architecture, we decided to leverage the concept of WideTables \cite{widetable}. WideTable is a denormalized table that is generated by pre-joining all the tables of the dataset together and dictionary-encoding its values. The denormalization process is a one-time preprocessing ste[ that needs to be done only when an update occurs. Our analysis in the figure-(todo Akhil) indicates that this WideTable has an extra 18-22\% memory footprint when compared to the vanilla dataset. With the WideTable approach, every query is solved by a series of filtering operations with no JOINs to be performed. Although the technique offers significant benefits even on the CPU paradigm, massive amounts of data still need to travel over the memory bus between the memory and the processor, thereby suffering from the Von Neumann bottleneck. However, with the PIM architecture, not only are the expensive data movement costs removed, but the increased parallelism of the architecture improves the speedup dramatically.
%\ks{This last sentence oversimplifies. A lot of data still traverses the bus (it's not removed entirely), but we certainly reduce it to only the data that satisfies the query. Some of the PIM benefit simply comes from greater parallelism.  I don't actually know that we've characterized how much performance we save by simply reducing the amount of data transferred.}

\textbf{CPU's Role in Database Application}
To analyse the role of a CPU in an OLAP database application, one needs to acknowledge that various innovations in both the software and hardware domain have significantly increased the throughput of these workloads significantly. The CPU performance has improved on an average by around 22\%/year (Akhil - cite Comp Arch book) in the past two decades, and the memory capacity by around 128x over the same period (Akhil - Mutlu PIM primer). Various optimizations and other software techniques such as hash-table data structures, compressed column stores, optimized query execution plans, etc., have further sustained the continuous improvements to the database performance. 

Although several alternative architectures such as the FPGAs and GPUs (Akhil -citations) have been proposed, the CPU still remains the prevailing architecture to process database workloads. \ks{Why? What prevents those from being good solutions and why aren't those problems issues for us as well?} \{\textit{Akhil : I had spoken about this in the Related Works section where earlier works had explored this. But I will add a comment here stating that the flexibility of the CPU happens to be one of the reasons. Others being the potential GPU VRAM to Main memory copy costs which could exhaust the gains we got. }Hence, rather than replace the CPU, we decided to compliment its capabilities with the PIM architecture. Since the entire query execution pipeline consists of various stages, there are certain operations such as grouping and sorting, that the CPU with its large cache and high clock speeds is inherently good at performing. PIM with its massive parallelism and immense bandwidth is shown to be very good at performing filtering and scanning operation (Akhil - provide ambit, fulcrum citations here) as discussed earlier. Hence, rather than PIM trying to replace the CPU over the entire query execution pipeline, our design allows us to offload parts of the pipeline that best take advantage of the architectural benefits offered both by the CPU and PIM and cooperatively process the query together. 

\textbf{Lean PIM Architecture}
One of the major benefits from this approach is the very low area overhead in PIM memory since it only happens to support the filtering and scanning kernel while the rest of the operations are executed on the CPU. Having low area overhead brings three-fold advantages, namely, maintaining near native DDR clock speeds, not sacrificing memory capacity to accommodate PIM capability and finally, acting as a drop-in replacement for conventional memory over adopting an accelerator-first approach. 

Due to thermal constraints, large area overheads in PIM sometimes translate to reduced clock speeds as seen in prior works (cite Fulcrum and Gearbox) and reduced clock speeds also greatly diminish the PIM performance. We have also observed in other designs (such as HBM-PIM) where large area overheads also eats into the memory capacity which might be very expensive in terms of datacentre economics. Also by having low-area overhead, as discussed earlier, PIM with a lean hardware overhead can act as a drop-in replacement for conventional memory which happens to augment certain kernels rather than replacing the CPU for end-to-end tasks. 

\ks{This needs to be tightened up. Kevin S can work on this.}



==> Membrane/Sections/Old-Introduction.tex <==

%% TODO Relevance and Problem Scope (Kevin G. or Akhil) %%
    % [x] briefly define analytic query processing (AKA OLAP).
    % [x] maybe an example of transaction tables with other dimension tables, SQL queries, etc.
    % [ ] a couple of sentences highlight OLAP importance, use cases, market value, etc.
    % [ ] recently, more and more OLAP is migrating into the main memory, due to the cost of DRAM comes down
    % (this work target in-memory DBMS where the entire data set is fit in memory)

%% OLAP is inefficient in traditional architecture %% 
%Databases are an important application category, and improvements in the underlying computer architecture across the processor, memory, and storage layers have been critical in allowing database systems to meet the never-ending need for high performance that end database applications demand.


Database sizes continue to grow unabated, and the query complexity also continues to grow. Increasingly, database systems are looking towards hardware innovations to allow them to obtain higher performance. This drive is especially critical in database applications called Online Analytical Processing (OLAP), characterized by complex queries on the underlying database that often (conceptually) need to scan the entire database. OLAP workloads include SQL queries that have many selection/filter, join, and aggregation operations. These workloads drive traditional enterprise report-writing use cases (the classic use of database systems for analytic query processing). 
OLAP queries are also critical in newer machine learning (ML)-based settings, where similar analytic SQL queries are used to prepare the data in the underlying database into a form that is amenable for downstream processing in an ML pipeline. Thus, the importance of rich SQL queries, characterized by the OLAP style of query processing, is growing rapidly~\cite{olapmarket}.

% TODO. Fig. (Kevin G) shows the performance breakdown of Duck DB, a state-of-the-art OLAP system executing XXX queries. Clearly, most of the stall cycles are caused by memory accesses. 

%% PIM is a promising alternative %%
%% Question from JMP: Should we narrow down the scope of our work to PUM instead or is PIM better as it is more general? 

Furthermore, the importance of {\em in-memory} database organizations is growing rapidly for OLAP systems, including in data science and business analytics settings where complex analytic queries are often performed with a human-in-the-loop (a key driver behind the rise of DuckDB)~\cite{alliedmarketresearch}. Furthermore, even when the database does not fit in memory, smart caching methods are used by the database management system (DBMS) to keep hot data in memory. 
Thus the CPU-DRAM level is critical for overall query performance~\cite{seattlereport}. %(The advent of CXL and DRAM pools may make this portion of the memory hierarchy even more important in the future.) We therefore focus on in-memory database settings in this paper.
\textcolor{purple}{
Similarly, Intel has released additional architectural support for OLAP-related tasks in the form of the Intel In-Memory Analytics Accelerator (IAA), which directly supports OLAP-related operations such as filtering and bitmap manipulation~\cite{intel-iaa}.
}

%This paper examines how DRAM-based processing-in-memory (PIM) methods can be used to accelerate OLAP workloads. A PIM-based approach is especially appealing for these workloads, because they are often bound by the memory system's performance in conventional von Neumann-style processing systems (which dominates the server landscape on which database systems are deployed). For example, consider Figure~\ref{fig:memory-profile-e2e}a, \jmp{This figure is now gone. Do we plan to bring it back?} which shows the different contributors to the aggregate time  to run each of the 13 queries in the widely-used  OLAP benchmark, SSB~\cite{ssbbenchmark}, on a hand-optimized SSE implementation of the benchmark (our baseline, which as we note later is significantly faster than the state-of-the-art database engine DuckDB~\cite{duckDB}). The database here is at a scale factor of 100 ($\sim$ 60GB of data in the SSB schema) with the database in a pre-joined format called WideTable that has been shown to be especially efficient for OLAP workloads~\cite{widetable}. As can be seen in  Figure~\ref{fig:memory-profile-e2e}a and b, even a highly optimized implementation of the SSB queries using SSE vector instructions is memory-bound. In other words, today OLAP applications hit the memory wall~\cite{memorywall}, and this problem is likely to grow over time as memory densities are likely to grow faster than memory bus speeds (both latency and throughput are important for OLAP workloads)~\cite{olapmarket}. 

%\jmp{Alternative text if we don't want to  bring back the figure that is referred to in the para above. Uncomment the para above in LaTeX. \newline}

This paper examines how DRAM-based processing-in-memory (PIM) methods can be used to accelerate OLAP workloads. A PIM-based approach is especially appealing for these workloads because they are often bound by the memory system's performance in conventional von Neumann-style processing systems (which dominates the server landscape on which database systems are deployed). As noted in~\cite{SirinA20}, OLAP applications hit the memory wall~\cite{memorywall}, and this problem is likely to grow over time as memory densities are likely to grow faster than memory bus speeds (both latency and throughput impact OLAP workload performance)~\cite{olapmarket}.

%For example, consider Figure~\ref{fig:memory-profile-e2e}a, \jmp{This figure is now gone. Do we plan to bring it back?} which shows the different contributors to the aggregate time  to run each of the 13 queries in the widely-used  OLAP benchmark, SSB~\cite{ssbbenchmark}, on a hand-optimized SSE implementation of the benchmark (our baseline, which as we note later is significantly faster than the state-of-the-art database engine DuckDB~\cite{duckDB}). The database here is at a scale factor of 100 ($\sim$ 60GB of data in the SSB schema) with the database in a pre-joined format called WideTable that has been shown to be especially efficient for OLAP workloads~\cite{widetable}. As can be seen in  Figure~\ref{fig:memory-profile-e2e}a and b, even a highly optimized implementation of the SSB queries using SSE vector instructions is memory-bound. In other words, today OLAP applications hit the memory wall~\cite{memorywall}, and this problem is likely to grow over time, as memory densities are likely to grow faster than memory bus speeds (both latency and throughput are important for OLAP workloads)~\cite{olapmarket}. 

%PIM methods have emerged as a promising alternative to address the performance bottleneck caused by large off-chip data movements. By bringing the computation closer to the memory instead of fetching data into the processor cores, significant gains can be realized on both the latency and energy metrics. For example, it has been shown that  fetching a 32-bit word from off-chip DRAM has a 6400x higher energy consumption than performing an ADD operation on the same data word by the CPU on a 45 nm technology \cite{eie}.
% Cut this for now, because I think the final sentence in this paragraph is sufficient. /K
%so PIM can achieve substantial improvements in energy efficiency by minimizing data movement~\cite{edge, online_profiling}. 
%Prior works also suggest big improvements in bandwidth and energy reduction by enabling computation at the DRAM row buffer level compared to the same computation on the CPU
%Furthermore, PIM offers massive parallelism, because multiple large operands stored in memory arrays can be operated upon concurrently. In this paper, we hypothesize that PIM architectures can be leveraged to accelerate OLAP/analytic workloads by enabling massively data-parallel execution, while simultaneously eliminating a large portion of data movement and achieving substantial energy savings. \ks{@Lingxi - Need to include an energy result in the results section or else fix this last sentence.}

%% Mapping OLAP to PIM is not straightforward %%
Unfortunately, there is no straightforward solution to map the end-to-end execution plan of an OLAP query to a PIM architecture. For instance, while PIM is ideal for data filtering (i.e., applying  single table predicates in the \textit{WHERE} clause of a SQL query) due to its high data-level parallelism, it cannot efficiently support table joins, which suffer from extensive internal data movement across different memory layers.
%, such as  channels, banks, and subarrays. (The database in an OLAP environment is generally not indexed, because indices slow down appends and queries tend to scan large portions of the database.) 
Furthermore, arithmetic expressions, sorting, and grouping operations that are processing steps in many OLAP queries are actually slower on a PIM architecture than on a typical multicore CPU. Thus, naively mapping the entire OLAP processing flow onto a PIM is likely to either result in marginal speedups or even performance degradation in certain cases. % TODO More analysis in Section TODO.
%\av{The use of multi-core here might be confusing.  I'm assuming those processing steps we're talking about benefit from the compute capabilities of a conventional OOO superscalar rather than thread-level parallelism exploited in multi-core processing.} \ks{The issue is simply that some parts of the processing flow map well to PIM (filtering and packing the data) but not others (joins).  I edited the text to clarify.}
%\av{There is a key missing piece here -- why aren't current PIM approaches proposed in the literature applicable?  We talk about challenges above, but we want to be more specific as to why OLAP workloads don't easily map to conventional PIM techniques and discuss potential tradeoffs, which would then nicely segue into the next paragraph.} \ks{Ashish, great point. Our current text makes it sound like we're inventing these techniques in a vacuum. @Lingxi or @Akhil, can you write a copule sentences here about why prior bit-serial techniques such as Ambit but also Sieve/DRAM-CAM, and prior word-level techniques such as BLIMP, Fulcrum, and Aquabolt (Samsung's FIMDRAM) aren't sufficient, and why we need to refine them for this specific application space?  Then we need to refine the next paragraph accordingly.  It should motivate the two architectures we study in this paper, H and V, in light of this prior work.} \textit{(Akhil: I have framed the next two lines to address the above concern, )}
Prior bit-serial techniques such as Ambit\cite{ambit}, SIMDRAM\cite{simdram} and word-level techniques such as Fulcrum\cite{fulcrum} and BLIMP\cite{blimp} have mapped kernels such as comparison operations used in database queries, but have not performed an evaluation of the end-to-end query pipeline and the critical role of data retrieval after filtering, nor have they optimized the PIM architecture specifically for database queries.
In this paper, we consider the impact of query processing techniques that utilize either \textit{early} or \textit{late materialization}, and the interaction of these mechanisms with the design of subarray-level PIM, in the context of an end-to-end data OLAP framework evaluated on the SSB benchmark suite~\cite{ssbbenchmark}.

%, meaning they carry performance, area, and power overheads that can be eliminated with specialization for OLAP. 

\begin{figure*}
\centering
    \hfill
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Membrane/Arch_Figures/WideTable.png}
        \caption{WideTable Approach}
        \label{fig:WideTable Approach}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.62\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Membrane/Arch_Figures/V and H diagram.png}
        \caption{Types of Membrane Architecture}
    \label{fig:Membrane_arch_overview}
    \end{subfigure}    
    \caption{Membrane Architecture for Query Processing with the WideTable Approach.}
   \vspace*{-1em}
\end{figure*}


%% We propose Membrane, and its key mechanisms %%
% This work aims to 
We then propose Membrane, a PIM-enhanced database engine for OLAP. We take a holistic approach to query execution by offloading suitable portions of the OLAP workload to PIM while mapping the remaining work that is less PIM-friendly to the host CPU. Specifically, we consider two distinct Membrane flavors. The first flavor, Membrane-H, is a bit-parallel but element-serial approach, inspired by Fulcrum~\cite{fulcrum} that processes one word at a time in each subarray; here data is laid out in a traditional ``horizontal,'' row-major manner. The second flavor, Membrane-V, is bit-serial but element-parallel, inspired by Sieve~\cite{sieve} and DRAM-CAM~\cite{DRAMCAM} and uses the entire width of each subarray's row buffer; in Membrane-V, words are laid out vertically up the subarray columns, as shown in Figure~\ref{fig:Membrane_arch_overview}. {We make novel contributions over prior work by efficiently implementing ranged-queries support instead of only exact matches in the Membrane-V subarrays. In addition, Membrane-H integrates a set of area-efficient scalar processing elements at the edge of each group of subarrays working in tandem with Rank-level Units to handle data materialization by pipelining operations for query processing and data selection.}


We develop the Membrane approach with two key ideas.
First, we observe that join operations are difficult to map to subarray-level PIM (these join operations combine data/records from two or more datasets/relations in the underlying database). Therefore, we adopt the \textit{WideTable} \cite{widetable} approach in which the database is pre-processed into a more efficient, denormalized or ``pre-joined'' form, which has the natural effect of converting join operations into selection operations on the underlying ``wide'' tables. {The WideTable format is also beneficial on traditional CPU-based architectures and has been used extensively in prior academic works~\cite{widetable, quickstep, ambit, bitweaving, byteslice} and also in commercial database settings~\cite{rockset}.}
{
WideTables use a dictionary encoding technique commonly found in existing database techniques~\cite{farber2012sap, krueger2011, raman2008constant, patel2013design}.
%To minimize the size of the WideTable, we apply dictionary encoding, which is often used  with denormalization~\cite{farber2012sap, krueger2011, raman2008constant, patel2013design}.
%The encoding mechanism is similar to the sorted dictionary encoding employed in \cite{widetable} and can support range predicates.
These dictionary encoding techniques support range predicates, making WideTables compatible with PIM scans on the encoded data.
} 

%% Second, we counter the data explosion challenge of a WideTable by employing dictionary encoding on each database column based on its cardinality, which keeps the size of a fully-joined WideTable comparable to that of a set of disaggregated tables. %% %Moreover, there are domain-specific heuristics that can be utilized to only pre-join a subset of columns, which produces a partial WideTable, alleviating the data size challenge even further.
%% By employing the dictionary encoding, we reduce the size of a WideTable by at least 3.7x in the SSB benchmark database. Compared to the original disaggregated dataset, the encoded WideTable is only 18-22\% larger than the original dataset size, even after joining all the SSB tables together. The WideTable approach slightly increases the cost of appending data, which must now be pre-joined, but this is an one-time offline pre-processing step, so the modest size increase is the key additional cost.

%\av{It is probably worth mentioning this challenge upfront rather than bringing it up in the contributions section.} \ks{I think it flows ok this way, and given that we claim the WideTable approach for PIM as one key idea, I don't know how to move this second point up. Anyway, I thinkn we have more urgent issues to worry about!}

Second, we find that the most appropriate OLAP task for the PIM device is predicate filtering (i.e., table scan/selection), which often dominates the query execution time on databases that are denormalized. Thus, we design  minimalist custom logic  embedded at the DRAM subarray levels to enable high-throughput in-situ table scans for both Membrane-V and Membrane-H. The integrated logic incurs a small area and power overhead compared to a commodity DRAM chip.

{Furthermore, to our knowledge, this paper is the first to conduct a comprehensive end-to-end comparison of V and H-based column layout methods for OLAP. Previous studies in software, such as BitWeaving, have favored V-methods when making such comparisons. Hardware research in this domain has concentrated on V-based methods. However, our end-to-end evaluation reveals that H-based methods are more favorable in our architecture. Both V and H-based approaches benefit from hardware acceleration in the filtering step, but the data gathering step between query operators presents a new bottleneck. In this regard, the H-based design offers more efficient solutions, with the RLU playing a critical role in accelerating this process.}

\ks{Need to update all this text:

Third, we identify the gathering of the selected data as the next largest bottleneck and explore how best to transfer data from the memory to the CPU. 
In the \underline{late materialization mode}, Membrane returns 
%the host CPU instructs Membrane to perform a predicate-based table scan operation, and Membrane merely returns 
a bitmask indicating which WideTable records satisfy the conditions in the filter predicate. The host then ``pulls'' data from the DRAM based on the bitmask. This form of query processing naturally aligns with existing bit-parallel PIM techniques such as Ambit~\cite{ambit} and Sieve~\cite{sieve} and is reflected in our evaluation of Membrane-V.
%to complete the remainder of the query processing operations, which is typically an aggregation operation that involves applying reduction functions such as MIN, MAX, and AVERAGE on input records that may be optionally be grouped based on an orthogonal grouping criteria.  However, our evaluation reveals that 
However, the task of processing the bitmask and fetching/gathering the data from the host CPU can often dominate the overall query processing time, especially after the filtering step has been accelerated. Therefore, we propose \underline{early materialization mode}, which directly returns the selected records. We find that early materialization mode maps well to Membrane-H.\footnote{Optimizing queries using early or late materialization remains a rich area of database research~\cite{Chernishev2022, Shrinivas2013, Abadi2007}.}
%In our end-to-end evaluation of SSB, 

%a packed set of contiguous  data vectors that are required by the final aggregation operation (which is still run in the host CPU). This Data-Push mode approach fits naturally into the PIM filtering task; as records are identified that match the predicate, those disparate records are gathered and sent back to the CPU, without the need for a large number of fetch transactions from the CPU. The CPU could reduce the number of transactions by sending a vector of addresses from which to gather results, but this is wasteful, because the PIM already has that information as it performs filtering. Data-Push mode effectively doubles the speedup over Bitmask mode in many cases, but with some restrictions. The tradeoffs associated with this design space are discussed in Section~\ref{sec:results}. 

%av{Might be a lot of detail for a paragraph in the introduction section.  The wording in the above paragraph (particularly, "however, our evaluation ...") seems to indicate that mode one is rather na\"ive and isn't practical?  I understand that there are trade-offs and this is a design space exploration, but our "final products" (i.e., mode one and mode two) need to be pitched as options that are beneficial in their own way (e.g., one is less invasive than the other).} 
%\ks{This is a good point. I personally like the detail we have here, but I think this paragraph needs to set it up better and open by explaining that filtering seems like a natural fit for the PIM, but it's not clear whether the data should then be "pulled" by the CPU based on a bitmask produced in the filtering stage, or "pushed" by the PIM as a tightly coupled part of the filtering, and pros and cons of each approach.}  \ks{Hopefully I addressed this now.} 

Finally, we describe a full-stack system integration solution for Membrane, including a set of ISA instructions 
%and API library calls 
that expose the PIM functionalities to the expert database system designer and a set of modified DRAM controller commands that allow the host to communicate with Membrane.

We compare the performance of the Membrane-assisted OLAP system using a popular SSB benchmark suite \cite{ssbbenchmark} (a set of 13 queries) with realistic data size (a compressed size of 60 GB at scale factor 100) to a highly-optimized handcrafted C++ CPU baseline using AVX 512 that outperforms DuckDB, a state-of-the-art OLAP system, by 18X (geometric mean). The evaluation suggests that Membrane-V/Membrane-H offers a geomean of 5.24x/10.63x end-to-end speedup over the highly optimized CPU baseline, incurring $\sim$2-3\% area and power overhead.



%The remainder of this paper is organized as follows ... 
%\av{easy to cut.}


==> Membrane/Sections/PIM_Operation.tex <==
\section{Query Execution with Membrane [DRAFT]}
\ks{If we need space, I think we can cut this, or condense it drastically. It's mostly repetitive.}
\hc{I agree with ks: I would merge the two sections into one that includes - 1) what is a PIM page, what systems calls we need to support (pim\_malloc, etc.), and 2) life of a query.}
The section below illustrates the flow of query execution from start to finish. It presents an overall view of the various components of system interactions described earlier in the execution flow.  

\textbf{1. Database setup within Membrane.} During the initial setup phase, denormalized databases are written in a columnar format into Membrane's PIM memory. Specifically, we propose that pim\_malloc( ) invokes a call to allocate a new page/pages, mark it as PIM-capable in the TLB, and start writing the database \hc{WideTable} columns into these pages. During this database write phase, the \hc{first mention?} de-interleaving unit re-arranges bits of a cacheline such that contiguous bits related to a record are placed within a single DRAM chip rather than being striped across different DRAM chips. 

\textbf{2. Query Input.} When a user enters the query, the database engine converts it into an execution plan containing two parts - ( i ) a series of SCAN operations to be executed on the PIM memory and ( ii ) a set of aggregate operations to be executed on the Host CPU. 

\textbf{3. PIM - Filter Phase.} \hc{This paragraph is talking about the same as PIM Configuration in the previous section but they do not fully say the same thing.} In order to launch the SCAN kernel, the CPU offloads the operation to the (PIM Command Generator) PCG with a descriptor indicating the start and end virtual address of the database column and details of the operation to be performed (value to compare against, type of comparison operation, length of each record). This descriptor offloading is similar to that of Intel's Data Streaming Accelerator, where all descriptors are communicated between the Host and the Accelerator through a series of MMIO registers and work submission portals as detailed in \cite{intel-dsa}.

\textbf{4. PCG Operation.} The PCG decodes the descriptor and configures the PIM processing elements to execute the SCAN operation by writing to specific addresses in the PIM Configuration (PIM CONF) space. It then consults the Translation Lookaside Buffer (TLB) for physical addresses of the associated page. It schedules a SCAN operation on the entire page after translation (as PIM operations are at a page-level granularity). 

\textbf{5. Membrane SCAN.} The control unit associated with each processing element decodes the instructions from the PIM CONF (PIM Configuration) addresses and prepares to execute the SCAN kernel. The memory controller passes a series of LISA hop commands in case of a subarray-level architecture being used to insert the data into Compute Slices. Furthermore, as mentioned earlier, a DRAM READ command in PIM Mode to particular address triggers a PIM computation on that address. For the Membrane's  bank and rank-level architectures, the memory controller issues a series of such READ commands to dictate and orchestrate the PIM operations. 

\textbf{6. PCG - Membrane Synchronization.} The PCG invokes a series of memory read commands addressing the page to be scanned. Note that this page is striped across all the ranks and banks depending on the mode of operation (SB or AB) described in Section-(TODO). This process is repeated for all the pages containing the specific database column. 

\textbf{7. Bitmap Read Phase.} The SCAN kernel is deterministic, as there are no conditional statements to execute. Hence, the PCG can time itself to know when the operation is completed. The results of the SCAN kernel are stored at a predetermined location (as indicated by the offloading descriptor), and the CPU is notified of job completion by updating a register similar to that described in (TODO cite Intel DSA spec). 

\textbf{8. Bitmap Retrieval and Aggregation.} The bitmap is read from the specified address location, with each index of the bitmap indicating if a record was filtered during the SCAN process or not. The CPU begins the aggregate phase after reading the bitmap, which involves executing sorting, grouping, min, max, and so on upon the filtered data as indicated by the input query. Filtered records are retrieved from the DRAM memory upon processing the bitmap. Note that these records reside within PIM-capable pages and are marked non-cacheable. The CPU reads them into a temporary structure (such as a hash-table or other convenient data structure) upon which it can perform the required aggregate operation later and materialize the result to the user.

==> Membrane/Sections/PiM_Design_Goals.tex <==
\section{PiM Design Goals and Workload Suitability (NEW)}

%\hl{We aim to accelerate in-memory databases with DRAM-based PiM architectures. Thus, we aim to optimize the architectures around the needs of the overall workload rather than targeting specific kernels in isolation since the query processing consists of various steps/operators, the results of each one being fed into the other parts. Hence, there is a need to take a comprehensive look the overall application from an end-to-end perspective. Based on this assumption, we try to answer the question as to what is the most optimum PiM architecture that we can design based on the requirements of an in-memory database. 

%Main Memory model vs Acceleration model. The in-memory databases typically store a major portion of the datasets within the main memory, and service the queries primarily around it. These datasets can be quite large and typically run into several hundreds of gigabytes. If we adopt an acceleration model for PiM similar to the one followed in GPUs, we might need to allocate large amount of DRAM capacity just to store, process and return the results back to the host CPU. This may make sense from a performance perspective, but DRAM is still considered expensive per gigabyte and would be difficult to argue for an economic use case especially if the final PiM architecture can only accelerate one application. Also, in a compute-centric accelerator such as FPGAs, or GPUs which bring the data in, process and write back the results, the compute elements can process large datsets with the compute capacity. However, in a memory-centric accelerators such as DRAM-based PiM architectures, a major or complete portion of the dataset needs to reside in the memory for the PiM processing elements to accelerate. Hence, in the latter case, with increasing dataset size, the size of PiM-capable memory too needs to increase without suffering major performance degradation. 
%Hence, with these constraints in mind, it makes more sense for the PiM architecture to follow a main memory model rather than an acceleration-based model since the same memory can be used for non-PiM workloads too which makes for an economic argument. Also, a majority of the in-memory database stacks are already designed with the main memory in mind and not around the accelerators, thus, it makes for economic argument since existing software can be ported over with minimal changes rather than redesigning the entire stack.

%PiM-based Main Memory. With the previous observation, we conclude that the workload should be accelerated with the main memory-capable of PiM computations. However, since memory is such a crucial aspect of the system performance, we need to careful as to not introduce too many disruptive changes such that it might hamper the performance or make it incompatible for non-PiM workloads. With this in mind, we aim to design our main-memory based PiM architecture around the following two criteria - 
%1. Low logic overhead - Typically DRAM is optimized for capacity and latency, hence any PiM architecture we aim to design should have low area overhead that does significantly affect the DRAM capacity or introduce dramatic changes that might affect its latency
%2. System compatibility - Since main memory is one of the key components for the overall system functioning, introducing any PiM elements should be compatible with existing host systems and again not introduce disruptive changes to this DRAM interface. 

%With these criteria in mind, we narrowed our PiM design space to mimic commercially available PiM architectures that not only are viable but are also compatible with host systems. For this work, we chose to center our design around Samsung's Aquabolt PiM which tries to serve as an add-in replacement for conventional memory without many changes required on the host side. Ofcourse there exist other alternative designs such as SK Hynix AiM and UPMEM. However, for the purpose of this work, we wanted to focus on Samsung's Aquabolt design as there was significant documentation available which assisted in understanding the architecture better from an end-to-end perspective and other works that performed an exhaustive evaluation (citation needed) upon this design.

%A significant differentiator between Samsung's Aquabolt and this work is that while Samsung's Aquabolt was primarily based on HBM memory, our PiM architecture is based around conventional DDR memory since query processing generally tends to use conventional DDR memory which scales in size easily  and is the preferred solution in systems that execute in-memory databases. 

%Workload-centric Design Space Exploration. We first begin our PiM Design Space exploration with most important question about which parts of the query execution are most suitable for PiM. To answer this question, \cite(inclusive PiM) introduces a set of 4 PiM-Amenability-tests that determine if a specific workload is suitable for acceleration by PiM or not. Ofcourse, these tests were determined with Samsung's Aquabolt in mind, and it might be reasonable to assume that a dramatically different PiM architecture might follow a different set of assumptions. Since our PiM system architecture will be based around Aquabolt, these assumptions hold true for our work too. 
%Currently, the PiM design landscape is too large and it would be difficult to evaluate every PiM architecture end-to-end with the Host system faithfully with a reasonable degree of accuracy. As more commercial PiM systems are adopted and the hardware and software stacks mature over time, our expectation is that we might eventually settle down on a common system framework and programming model for PiM. However, as PiM is yet to gain widespread adoption, we are compelled to choose amongst the existing commerically available designs and base our experiments around them.

%The PiM-Amenability-Tests help the programmer to assess if a specific portion of the workload is amenable to PiM acceleration based on workload's characteristics. The kernel should pass all the four tests and not just a subset of the tests to be amenable for PiM acceleration. The tests are as follows - 
%1. Is the workload memory-bound? 
%2. Does the workload have low on-chip cache reuse? 
%3. Does the workload exhibit localized operand interaction i.e. intra-bank interaction? (Inter-region transfers are expensive)
%4. Does the workload exhibit address-interleaving aware allocations i.e. can it exhibit aligned data parallelism? 

%When we look at the query processing workload, we observe that it can be broken down into three kernels broadly - 
%1. Scans - To read a row/column of data and perform filtering operation, the results of which are consumed by the downstream operators. 
%2. Joins - combine elements of two tables based on the foreign key-primary relationships existing between the said tables
%3. Aggregate operations - These are operations such as average, sum, group by, sorting that are performed on the output data before it is materialized to the user. 

%Typically during a query execution, the scans are performed on the database rows/columns and the results of the scan operator is consumed by the Join operator involved in joining two or more tables together. Finally once the query executes a series of scan and join operations, we obtain the output data that goes through the aggregate operator before materializing the final results to the end user. 

%When examining the above three kernels broadly, the scan kernel passes 4/4 tests while Joins and Aggregate operations pass only 1/4 tests. A brief explanation of the kernels and their behaviour with regards to these tests are elaborated below. 

%The scan kernel tends to be memory-bound as we access a large dataset from the memory and execute a series of comparison operations upon these tabular structures. They also do not reuse the cache extensively as data is streamed in to the processor to perform a comparison operation without a major portion of it typically not being reused at a later stage. It also does not significantly interact with other operands as comparison operations on database queries tend to be against a fixed value (for ex. 2000 > d\_year > 2008). The scan kernel also exhibits aligned data parallelism where the same kernel can be executed across multiple DRAM regions (subarrays/banks/ranks) with aligned memory addresses feeding data from DRAM locations into the PiM compute elements with the same command. 

%The Joins meanwhile although being memory-bound (cite Deming Chen paper CIDER '20), do benefit from having caches while performing hash-join which is a relatively popular technique utilized to perform joins on database tables. In fact, the join algorithms are tweaked in many instances (citations needed) to make the join algorithm cache-aware. We also observe that while joining two different tables, these tables most often are large enough that they do not fit within the same subarray/bank/rank and thus cross-region interactions become a  necessity. Furthermore, random memory accesses dominate the join kernel making them unviable to obtain a large degree of aligned data parallelism. Hence, the join kernels tend to fail in 3/4 of tests. While the workload can be significantly pre-processed and partitioned which could possibly improve the operand locality, we still believe that it might not be able to pass the tests completely making them not the best possible candidates for PiM acceleration. 

%The aggregates is a broad term that encompasses a large number of kernels that are executed on the filtered data. Kernels such as sums, averages, count are relatively simple and are amenable to PiM, however other aggregate operations such as sorting and grouping are not PiM-amenable. This is because, kernels such as sorting and grouping have a high on-chip cache reuse and do not exhibit aligned data parallelism as the accesses are random in nature. Also, the data to be operated on for aggregate operation post-filtering can reside anywhere in the memory across various subarrays, banks, ranks and channels. Thus it makes more sense for the aggregate operations to be performed on the Host CPU rather than on PiM exclusively. 

%#### Cooperative Processing between Host and PiM
%As elaborated earlier, we observe that only the scan kernel is amenable for PiM acceleration while JOINs and aggregate operations are not. The JOINs and aggregates are well-studied and there are several existing works (citations) that optimize these kernels for the CPUs. Thus, we propose to build up on these existing works and offload parts of the query execution pipeline (such as SCANs) unto PiM and cooperatively process the rest of the query execution pipeline on the host CPU. }


\hl{In-memory databases store datasets in the main memory, and our goal in designing a PiM architecture is to integrate compute capability into this memory to process queries. However, there are certain constraints to consider when designing the PiM architecture. The architecture should have low area overhead, so as not to significantly affect DRAM capacity or latency. It should also be compatible with existing host systems without disrupting the CPU-DRAM interface.

To meet these constraints, we chose to explore architectures similar to commercially available PiM designs that maintain compatibility. Specifically, we centered our exploration around Samsung's Aquabolt PiM, which can serve as an add-in replacement for conventional memory without requiring many changes on the host side. While there are other alternative designs such as SK Hynix AiM and UPMEM, we chose Samsung's Aquabolt since it had significant documentation that allowed us to understand the overall approach better.

One significant difference between Samsung's Aquabolt and our PiM architecture is that Samsung's Aquabolt is primarily based on HBM memory, while our architecture is based around conventional DDR memory. Query processing generally tends to use DDR memory, which is also the preferred solution in systems executing these types of workloads. Additionally, DDR memory scales in size easily, making it a better option for our PiM architecture.Since the in-memory databases typically store the datasets within the main memory, our aim with regards to designing a PiM architecture is to infuse this main memory  with compute capability to process the queries. With this in mind, there are certain constraints to keep in mind while designing the PiM architecture - 
1. Low logic overhead - Typically DRAM is optimized for capacity and latency, hence any PiM architecture we aim to design should have low area overhead that does not significantly affect the DRAM capacity or introduce dramatic changes that might affect its latency
2. System compatibility - Since main memory is one of the key components for the overall system functioning, introducing any PiM elements should be compatible with existing host systems and again not introduce disruptive changes to this CPU-DRAM interface. 

Hence, we narrowed our PiM design space to mimic commercially available PiM architecture designs that maintain this compatibility. For this work, we chose to center our architecture exploration around Samsung's Aquabolt PiM which tries to serve as an add-in replacement for conventional memory without many changes required on the host side. Ofcourse there exist other alternative designs such as SK Hynix AiM and UPMEM. However, for the purpose of this work, we wanted to focus on Samsung's Aquabolt design as there were significant documentation which assisted in understanding the overall approach better. 

A significant differentiator between Samsung's Aquabolt and this work is that while Samsung's Aquabolt was primarily based on HBM memory, our PiM architecture is based around conventional DDR memory since query processing generally tends to use the latter. Also, DDR memory scales in size easily and tends to be the preferred solution in systems execution these types of workloads. 

\textbf{We are conducting a thorough exploration of the PiM Design Space to determine which parts of query execution are most appropriate for PiM acceleration. To accomplish this, we are relying on prior work from AMD, which evaluated Samsung's Aquabolt-XL and identified a set of 4 PiM-Amenability-tests that determine whether a workload is suitable for PiM acceleration. Although these tests were determined with Samsung's HBM-PiM in mind, we recognize that a different PiM architecture may follow a different set of assumptions.

We acknowledge that the PiM design landscape is vast, making it impractical to evaluate every PiM architecture end-to-end with the host system in a reasonably accurate manner. However, as more commercial PiM systems are adopted and the hardware and software stacks mature, we expect to eventually settle on a mature design. In the meantime, we must choose from the existing commercially available designs and base our experiments on them.

The PiM-Amenability-Tests provide programmers with a means to assess whether a specific portion of the workload is amenable to PiM acceleration, based on workload characteristics and heuristics. To be amenable to PiM acceleration, the workload or kernel should pass all four tests, not just a subset, as suggested by the authors.

When examining the query processing workload, we observe that it can be broken down into three kernels: Scans, Joins, and Aggregate operations. Scans tend to pass all four tests, while Joins and Aggregate operations pass only one of the four tests. Scans are memory-bound, accessing a large dataset from memory and executing a series of comparison operations. They do not reuse the cache extensively, as data is streamed into the processor to perform a comparison operation without a major portion of it being reused later. They also do not significantly interact with other operands, as comparison operations on database queries tend to be against a fixed value. The scan kernel exhibits aligned data parallelism, allowing the same kernel to be executed across multiple DRAM regions with aligned memory addresses, feeding data from DRAM locations into the PiM compute elements with the same command.

Joins, on the other hand, although being memory-bound, benefit from having caches while performing hash-join, a popular technique used to perform joins on database tables. In many instances, join algorithms are tweaked to make the join algorithm cache-aware. Joining two different tables often requires cross-region interactions, making random memory accesses dominate the join kernel, which makes them unsuitable for achieving a large degree of aligned data parallelism. The join kernels tend to fail in three of the four tests. Although the workload can be significantly pre-processed and partitioned, which could possibly improve operand locality, we still believe that it might not be able to pass the complete set of tests, making them not the best possible candidates for PiM acceleration. 

Overall, based on our analysis, we assert that the scan kernel is the most appropriate part of query execution for PiM acceleration, whereas Joins and Aggregate operations may not be the best candidates for PiM acceleration.
}

==> Membrane/Sections/PiM_Design_Goals_-_Short.tex <==
\subsection{PiM Design Goals and Workload Suitability}

\ak{The message to give here is that we give a brief overview of the workload and how we select portions of the workload to offload to PiM based on a certain criteria}

\hl{Our exploration of the PiM Design Space is a crucial step in determining which parts of query execution are most suitable for PiM acceleration. This endeavor is built upon prior work (TODO citation), which introduced a set of 4 PiM-Amenability-tests that serve as a litmus test for determining if a workload is amenable to acceleration by PiM.  

The PiM-Amenability-Tests help programmers assess if a specific portion of the workload is amenable to PiM acceleration based on workload characteristics and heuristics. The tests are:

1. Is the workload memory-bound?

2. Does the workload have low on-chip cache reuse?

3. Does the workload exhibit localized operand interaction, i.e., intra-bank interaction? (Inter-region transfers are expensive)

4. Does the workload exhibit address-interleaving aware allocations, i.e., can it exhibit aligned data parallelism?

The authors suggest that the workload or the kernel should pass all four tests, not just a subset, to be amenable to PiM acceleration. 

When we examine the query processing workload, we observe that it can be broken down into three kernels broadly: Scans, Joins, and Aggregate operations. Scans read a row/column of data and perform filtering operations, and downstream operators consume the results. Joins combine elements of two tables based on the foreign key-primary relationships between them. Aggregate operations such as average, sum, group by, and sorting are performed on the output data before it is materialized to the user. 

Typically, scans are performed on the database rows/columns, and the results of the scan operator are consumed by the join operator involved in joining two or more tables together. Finally, once the query executes a series of scan and join operations, we obtain the output data that goes through the aggregate operations before materializing the final results to the end user. 

When examining these three kernels, we find that the scan kernel passes 4/4 tests, while Joins and Aggregate operations pass only 1/4 tests. The scan kernel tends to be memory-bound as we access a large dataset from memory and execute a series of comparison operations. They use the cache sparingly, as data is streamed into the processor to perform a comparison operation without a major portion of it typically being reused later. It also doesn't significantly interact with other operands, as comparison operations on database queries tend to be against a fixed value. The scan kernel exhibits aligned data parallelism, where the same kernel can be executed across multiple DRAM regions with aligned memory addresses, feeding data from DRAM locations into the PiM compute elements with the same command. 

On the other hand, although memory-bound, Joins benefit from having caches while performing hash-join, a popular technique utilized to perform joins on database tables. Join algorithms are tweaked in many instances to make the join algorithm cache-aware. Joining two different tables requires cross-region interactions, making random memory accesses dominate the join kernel, which makes them unsuitable for achieving a large degree of aligned data parallelism. The join kernels tend to fail in 3/4 of the tests. Although the workload can be significantly pre-processed and partitioned, which could improve operand locality, it may not be able to pass the complete set of tests, making them not the best possible candidates for PiM acceleration. }

==> Membrane/Sections/Results.tex <==
\label{sec:results}
%\vspace{-0.1in}
\subsection{Power, Latency, and Area Evaluation} \label{sec:overhead}

\textbf{Energy Evaluation.} \mrtn{Careful: Section contains RLU-related results.} Table \ref{tab:hardware} reports area, delay, and power of each Membrane-H (M-H) ALU  and the Membrane-V (M-V) filter logic (i.e., 1-bit comparator). The dynamic energy of entire Membrane-V filter array is calculated as the energy of the 1-bit comparator multiplied by the subarray width, and total dynamic energy consumption on the table scan for each query can be estimated as the number of times the filter array is accessed multiplied by energy cost of accessing the filter array once. The total dynamic energy consumption for Membrane-H is calculated as the ALU energy cost multiplied by the times the ALU is used for predicate filtering plus the energy consumed by RLUs. Our RTL simulation indicates that each bitmap processing and gathering Unit consumes 417.38 $\mu$W and with presence of a programmable core, we have approximated the overall power consumption of the RLU to 0.5 W.  Membrane's peak power usage depends on its subarray-level parallelism as more active subarrays lead to a significant rise in static power.
% The peak 
%We observe for both Membrane-V and Membrane-H, enabling a modest amount of subarray-level parallelism (SALP=2 or 4) achieves the best performance per watt, shown in Figure \ref{fig:salp_overall_analysis}(a).  %Cut here because it's repeated below.

\textbf{Area Evaluation.} To estimate the area overhead of a Membrane chip, we first obtain the area breakdown of the DDR4 chip (Micron\_8Gb\_x8) that is used to build  the Membrane using Cacti-3DD \cite{cacti}. Each subarray contains 512 rows, and there are 128 subarrays per bank.  For Membrane-V, the logic can only fit along the sense amplifier's long side as indicated in \cite{sieve}. We adopt a DRAM sense amplifier layout described by Song et al.~\cite{samsungDramChip} and a patent from Micron~\cite{micronPatent} for a conventional 4F\textsuperscript{2} DRAM layout.  The short side and long side of the sense amplifier are 6F and 90F, respectively. We estimate 990F needs to be added on the long side of the local sense amplifiers to fit the 1-bit comparator logic. To support the LISA mechanism, an extra 60F on the long side is added to each sense amplifier for considering the area overhead of the links between the subarrays. For Membrane-H, since the ALU does not need to be pitch-matched to the bitline, the area overhead is much smaller. We estimate fitting 64 additional ALUs (shared by 128 subarrays) per bank, along with the overhead of enabling SALP and LISA, incurs only 5.26\% area overhead. The Rank-level Unit incurs negligible area overhead (Table \ref{tab:hardware}) compared to the overall chip area. \mrtn{Careful: More RLU.} Additionally, RLU would not affect the storage density of the Membrane since it is integrated into the DIMM module. Overall, the area overhead for Membrane-V with 1, 2, 4, 8, 16, 32, 64, and 128 filter arrays (i.e., SALP-1 -- SALP-128) is 2.35\%, 2.71\%, 3.42\%, 4.84\%, 7.75\%, 12.50\%, 25.00\%, and 46.0\% respectively, and the area overhead for Membrane-H with 1, 2, 4, 8, 16, 32, and 64 ALUs (i.e., SALP-1 -- SALP-64) is 2.02\%, 2.04\%, 2.07\%, 2.14\%, 2.28\%, 2.55\%, 3.10\%, and 5.26\% respectively.  For both Membrane-V and Membrane-H, we observe that enabling a modest amount of subarray-level parallelism (SALP=2 or 4) achieves the best performance per watt, shown in Figure-\ref{fig:salp_overall_analysis}. These results and a sensitivity study regarding the area efficiency w.r.t. subarray-level parallelism are also shown in Figure \ref{fig:salp_overall_analysis}(a) and Section \ref{sec:salp}. 
Additionally, introducing a row of latches to overcome the mat-level organization within the subarray structure to store and feed data sequentially into the Membrane-H ALU would introduce only a 1.9\% area overhead to the DRAM cell-array area.

% Moved to sensitivity study Membrane-H shows much better scaling with the degree of subarray-level parallelism (SALP) but our results in Figure REF HERE show that performance flattens out at very low levels of SALP because \ks{REASON HERE}.

\textbf{Latency Evaluation.} The main latency of the filter array logic in Membrane-V is on the  write broadcast in the Membrane-V path of the row activation. However, it adds negligible overhead ($\sim$0.47 ns) compared to the DRAM row cycle (35$\sim$50 ns). For Membrane-H, the ALU latency is also on the critical path. While filtering on one attribute takes an insignificant amount of time ($\sim$1 ns), the total ALU latency to check all relevant attributes in a row can add up to a similar latency as a DRAM row cycle, depending on the data layout. Still, it is sufficiently hidden by the data materialization cost. We show more insights on the latency breakdown of Membrane-V/H in Section \ref{sec:breakdown}.  



\begin{table}
\scriptsize
    \centering
    \caption{Membrane Hardware Characteristics. \vspace*{-6pt}}
        \begin{tabular}{|l|r|r|r|}
        \hline
        & \textbf{M-H ALU (16-bit)} & \textbf{M-V Filter (1-bit)}  \\
        \hline 
        \hline
        \textbf{Area} $(\mu m\textsuperscript{2})$ & $301.08$ & $11.36$\\ \hline
        \textbf{Delay} $(ns)$ & $0.36$ & $0.47$ \\ \hline
        \textbf{Power} $(\mu W)$ & $25.75$ & $1.14$ \\ \hline
        \end{tabular}
\label{tab:hardware}
\vspace*{-.15in}
\end{table} 

%\vspace{-0.15in}
\subsection{Overall Membrane Performance}
\mrtn{This subsection will need to be cleaned up and split into subsubsections. Consider the following as individual subsections:}
\begin{itemize}
    \item \textcolor{teal}{Discuss the other systems to compare. How do they cover a variety of other options in PIM and PIM-adjacent spaces. This may be worth a dedicated subsection in the methodology.}
    \item \textcolor{teal}{Discuss SSB and TPC-H as evaluation benchmarks. Discuss the usage of WideTables for each. This can be placed in the relevant methodology subsection, but it may be beneficial to move it closer to the experiments. Depends on if we're using WideTables for everything.}
    \item \textcolor{teal}{Discuss SSB results.}
    \item \textcolor{teal}{Discuss TPC-H results. Explain why we don't perform all queries (strings, etc.), but also note how this is common in other academic works (bulk citation beneficial).}
\end{itemize}
\textcolor{teal}{Also, make sure to freshen all results in the text, as appropriate.}

Figure \ref{fig:overall_perf} shows the overall \textit{end-to-end} performance improvement of  Membrane over the CPU and two other possible PIM-based OLAP solutions (SIMDRAM \cite{simdram}, and RVU \cite{rvu}) in log scale. We select SIMDRAM as an alternative DRAM-based bit-serial processing technology to the Membrane-V. SIMDRAM differs from Membrane-V with its charge-sharing (analog) triple-row-activation-based computing. The RVU is a 3D-stacked near-memory-processing solution comparable to the Membrane-H because it employs an element-parallel but bit-serial columnar data layout. We assume all PIM architectures only accelerate the table scan portion of the workloads. The host cooperates with the PIM using the bitmask, which can fully leverage the CPU and PIM processing potential (Sec. \ref{sec:background}). The CPU configurations are reported in Table \ref{tab:workstation}.  %Each columnar database scan is executed as a vector utilizing GPU's parallelism to evaluate the predicate operation of its elements and report the result either in the form of a \underline{bitmap or data-push method}.  
We compare the Membrane integrated system with the handcrafted optimized AVX512 C++ query implementation described in Section \ref{sec: baseline_perf_modelling}. Membrane-V/H and SIMDRAM are configured to be eight channels with two ranks per channel using Micron's DDR4\_8Gb\_x8 DRAM chip as the building block. For the RVU, we assume 16 HMCs (configuration in Table. \ref{tab:hardware}) connected with zero communication overhead to make up the same capacity as other architectures.  We choose a moderate degree of subarray-level parallelism, namely, four subarray groups (SALP=4) in Membrane-V and SIMDRAM\cite{simdram} and four concurrently working ALUs in Membrane-H. For Membrane-V, we also enable the write broadcast feature by assuming each write command updates the query regions of two subarrays. For both Membrane-V and Membrane-H, we report the performance of the row-major data layout. 

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{Membrane/Result_Figures/results_ete.pdf}
    \vspace*{-1em}
    \caption{
    \mrtn{Careful: Not yet updated for RLU-removal.} End-to-end SSB performance of various PIM techniques, compared against a hand-optimized AVX-512 CPU baseline. Results are depicted as a speedup against the CPU baseline. Aside from Membrane-H, which uses the RLU, all techniques are evaluated using a late materialization strategy.}
    \label{fig:overall_perf}
    \vspace*{-.1em}
\end{figure}

First, the Membrane architecture consistently outperforms the CPU baseline in all queries. Membrane-V and Membrane-H offer 1.26$\times$/25.97$\times$/5.94$\times$ and 7.20$\times$/185.75$\times$/45.39$\times$ \break min/max/geomean speedup respectively. Second,  Membrane achieves the best performance gain when the query selectivity is high (i.e., few database records passed matched to the predicate), such as in %\sout{Q3, Q9, Q10, and Q13} 
Q1.3, Q3.3, Q4.3. This characteristic is because Membrane can save data movement overhead by performing an in-place table scan, significantly eliminating the overhead of fetching data into the CPU. However, for queries with low selectivity, data retrieval for aggregation becomes the larger bottleneck. For example, %\sout{Q7}  
Q3.1 selects the most data to aggregate; hence, the portion of the workload that benefits from Membrane-V's late materialization is limited. Third, Membrane-H almost doubles the performance of  Membrane-V because H works well with the RLU and thus provides densely packed data for the host to consume, saving the cost of processing the bitmask and return trips from the CPU to memory for data retrieval. %The Membrane-V/H outperforms the GPU by 4.75x/8.88x, respectively. Since the processing elements within PIM combined are exposed to a higher bandwidth than the available bandwidth between the GPU and its VRAM by at least an order of a magnitude, the Membrane outperforms the GPU significantly. 
%Finally, the lower the number of columns being scanned in a given query and the higher the selectivity, the lower the speedup of the Membrane. 


Compared to SIMDRAM, Membrane-V is, on average (geomean) 34\% faster. We notice that while SIMDRAM is 15\% faster than Membrane-V to set up the predicate due to its ability to leverage the DRAM burst write feature better; it suffers performance loss in the actual predicate scan. Each triple-row activation is 6.8X slower than a single-row activation, and additionally, SIMDRAM spends 3X more operations at each bit location than Membrane-V. Compared to RVU, Membrane-H is, on average (geomean) 72\% faster. While both RVU and Membrane-H scans horizontally laid out data, RVU has a much smaller throughput because of the narrow row buffer in HMC compared to 2D planar DRAM banks. Each row activation allows the Membrane to process more database records than RVU. Additionally, the computing logic of RVU is integrated at the logic layer; therefore, it is limited to DRAM bank-level parallelism, contrary to Membrane, which further exploits subarray-level parallelism. 

The energy reduction (not shown in a figure) is highly correlated to the execution time of the query. Both Membrane-V and H versions achieve the best energy reduction for Q1.3 and the least for Q3.1. Specifically, Membrane-V offers a min/max/geomean of 2.01$\times$/48.09$\times$/10.05$\times$ energy reduction, while H offers a 8.46$\times$/456.73$\times$/71.40$\times$ energy reduction.

\subsection{Membrane Performance Breakdown} \label{sec:breakdown}

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{Membrane/Result_Figures/membrane_v_bitmask_breakdown.pdf}
    %\vspace*{-1em}
    \caption{\mrtn{Careful: Not yet updated for RLU-removal.} Membrane-V SSB query breakdown.}
    \label{fig:M-V-breakdown}
    \vspace*{-.20in}
\end{figure}

Figures \ref{fig:M-V-breakdown} and \ref{fig:M-H-breakdown} show the execution time breakdown for both Membrane architectures (using the same configuration that is used in Figure \ref{fig:overall_perf}). In the case of Membrane-V, write broadcast is enabled. Figure \ref{fig:M-H-breakdown} also shows the effect of three different data layouts, namely, row-major, hybrid, and columnar, on Membrane-H. We make several key observations. First, the actual time spent activating rows for table scans (Filter) is relatively low for both Membrane-V and H. Membrane-V's execution cycles are mostly spent on populating the subarray query regions. Each query, i.e., predicate value, must be written vertically along the bitlines. The predicate values are several hundreds of bitlines apart, which is a highly inefficient way to access the DRAM.
Furthermore, the write latency associated with setting up the queries in Membrane-V cannot be sufficiently reduced by the subarray-level parallelism because column commands within a bank must be served serially unless the write-broadcast hardware design is enabled (Figure. \ref{fig:salp_overall_analysis}(b)). Membrane-V favors queries that filter on fewer attributes or attributes with low cardinality (e.g., \ak{Q2.1}). Membrane-H spends roughly the same amount of cycles on row activation and processing the latched bits in the local row buffer using the ALU, regardless of the data layout. A key aspect of Membrane-H is the benefit of the RLU in performing data retrieval at a rank-level. The increased parallelism and bandwidth available with RLU helps in reducing the data retrieval time by 2.66x across the benchmark. More in-depth analysis of the effect of data layout on Membrane-H's performance is in Section \ref{sec:data_layout}. 

\subsection{Sensitivity Study}
\subsubsection{\textbf{Effect of Data Layout}} \label{sec:data_layout}

Figure \ref{fig:M-H-breakdown} illustrates how different data layouts affect the performance of the Membrane-H architectures. The row-major layout activates the same number of rows across different queries because each row activation brings a whole row of complete database records to filter, and all database records must be checked. The hybrid layout is a combination of row-major and column-major layouts. Only rows containing attributes used in the table scans are activated in the hybrid and columnar  layout. The performance of the columnar and hybrid data layouts improves as fewer attributes are scanned. The hybrid data layout improves the row activation time (Row-Act bars in Figure. \ref{fig:M-H-breakdown}) of eight queries by 1.4$\times$ and five queries by 2.6$\times$. The columnar data layout improves the row activation time of three queries by 1.4$\times$, seven queries by 1.9$\times$, and three queries by 2.7$\times$. 

\begin{figure}
    \centering
    \includegraphics[width=1.05\linewidth]{Membrane/Result_Figures/data_retrieval_time_comparison_new.pdf}
    \vspace*{-1.5em}
    \caption{\mrtn{Careful: Not yet updated for RLU-removal.} Membrane-H time to materialize each SSB query, by layout. For each query, the data layout with the shortest time to materialize each query is labeled above.}
    \label{fig:M-H-breakdown}
    \vspace*{-.12in}
\end{figure}

The hybrid data layout favors queries that scan attributes concentrated in a few subarray rows. We spent considerable time trying to find the optimal hybrid layout using the Louvain method for community detection \cite{louvain_clustering}. 
%The number of rows to activate between the row-major layout and the hybrid layout would be similar if the attributes of the database records participating in the table scan operation were more scattered in different subarray rows. 
The data layout choice also affects the latency spent on the ALU. The amount of time the ALU spends on each activated row depends on how many attributes in that row are participating in the table scan. %\sout{Since the row-major layout stores complete database records in each row, the attributes required by the filtering operation tend to be sparsely located. Thus the ALU spends the least amount of time on each row. The hybrid layout tends to perform the worst because each row stores the most attributes for the ALU to check, even more so than the columnar layout. Overall,  the columnar data layout offers the best performance for the Membrane-H because it checks fewer rows, row-major is slightly worse, and hybrid is much worse.}}

%\sout{However, the row-major layout is the most efficient data layout when data retrieval is considered,  because, all of the attributes needed for the data retrieval are located in the same row for the database records that pass the predicate filters.  But for the hybrid and columnar layout,  Membrane visits multiple rows to gather the required attributes for each record that passed the scan/predicate filters.  When combining filtering and data retrieval, the best data layout choice depends on the query's selectivity. Queries that return few records, such as Q3.4, are dominated by the filtering task and thus perform better with a columnar organization. Still, those that return more records perform better with a row-major layout. Overall, %the benefits of a columnar layout do not overcome the importance of data retrieval, and row-major is a safer choice.}
%\ak{ak comemnt - Its quite possible due to very low selectivity (<0.01\%) in majority of the SSB queries, that row-major is winning. I think the difference between row-major and column-major in data retrieval is very narrow when looked at the overall query execution (TODO run numbers to see what is the percentage point difference) Traditionally column-majors are considered over row-major for high performance if I am not wrong. Hence, claiming that row-major to be safe choice in every scenario might not be good. Atleast for SSB dataset as we observed, we empirically found that row-major is safe. The best data layout in each case depends on combination of factors such as number of attributes being used by selection operator, number of attributes being used by aggregate operators and the overall query selectivity.}

%\ak{An interesting observation is that hybrid layout was designed to achieve least filtering time based on the attributes being utilised by selection operators of all queries, and we observe that this layout was indeed able to achieve it as demonstrated by the results. Hence, in situations where advanced knowledge of queries to run is available, hybrid layout could be utilized to configure the data layout to achieve the best performance. }
We observed marginal differences in performance between different data layouts across the query suite. The hybrid approach demonstrates that in the presence of prior knowledge related to the queries to be executed, the data layout could be optimized for better performance. However, this is highly dependent on data schema and the queries being run themselves. \ref{fig:M-H-breakdown} demonstrates the empirical results observed from our experiments with the data layout modifications on  SSB. 

\begin{figure*}
\centering
\begin{subfigure}[t]{0.338\linewidth} 
    \includegraphics[width=0.75\linewidth]{Membrane/Result_Figures/salp_power_area_scatter_new.pdf}
    \caption{\mrtn{Careful: Not yet updated for RLU-removal.} The Membrane chip power and area overhead at varying levels of subarray-level parallelism. }
    \label{fig:salp_area_overhead}
\end{subfigure}%
    \hfill%
\begin{subfigure}[t]{0.62\linewidth} 
    \includegraphics[width=0.85\linewidth]{Membrane/Result_Figures/salp_time_new.pdf}
    \caption{\mrtn{Careful: Not yet updated for RLU-removal.} Query execution time breakdown in multiple Membrane modes, by query component. \mrtn{Which query? Need to specify if it's SSB or TPC-H.} H/V-: Membrane-H/V, RowAct.: Membrane latency on row activation, Materialize (Mtz.): Membrane-H latency to materialize data, and +B: write broadcast.}
    \label{fig:salp_geo_mean_time_breakdown}
\end{subfigure} 
\caption{Effect of subarray-level parallelism on area, geometric mean query power consumption, and performance.}
\label{fig:salp_overall_analysis}
\vspace*{-.1in}
\end{figure*}

\vspace{-0.05in}
\subsubsection{\textbf{Subarray-level Parallelism}} \label{sec:salp}

\textbf{Effect on Power and Area.} Figure.\ref{fig:salp_overall_analysis}(a) illustrates the area (X-axis) and power (Y-axis) overhead that is associated with subarray-level parallelism (SALP). Note the area and power overhead of the Membrane-H RLU (integrated on the DIMM) are not included in the analysis since it is not affected by subarray-level parallelism. Membrane-H chip stays low in area overhead even if we aggressively increase the potential subarray-level parallelism. The ALU logic does not need to be pitch-matched to the sense amplifiers (Section.\ref{sec:overhead}), unlike Membrane-V. For low SALP values, such as SALP=2 and 4, Membrane-V and H have a similar area overhead ($\sim$2\%). The geometric mean power consumption difference of Membrane-V and Membrane-H is small regardless of the SALP values, but both grow rapidly with higher SALP values. The peak power consumption associated with  SALP=128 incurs over 60\%  overhead compared to SALP=1.

\textbf{Effect on Performance.} Figure \ref{fig:salp_overall_analysis}(b) shows the geometric mean performance breakdown of query processing with varying degrees of SALP. Increasing the SALP 1) reduces the overhead of inter-subarray data movement (LISA) incurred by copying rows from non-PIM subarrays to the PIM-enabled subarrays, and 2) overlaps multiple row activations that go to the same bank but different subarray groups/ALUs. {Doubling subarray-level parallelism adds 10\% to 15\%  additional performance for Membrane-H and Membrane-V w/o write-broadcast optimization.} The subarray-level parallelism is most beneficial when the write broadcast mechanism in Membrane-V is enabled, significantly reducing the predicate value setup time in Membrane-V. However, the benefit of subarray-level parallelism plateaus after SALP=4 (without Membrane-V broadcasting) or SALP=8 (with Membrane-V broadcasting) for both Membrane-V and Membrane-H for several reasons. First, bank-level access conflicts can be eliminated with a moderate number of concurrently working subarrays. Second, subarray-level parallelism can only parallelize the row activation of retrieving data from different subarrays. However, for Membrane-H, the column commands are still performed serially.  %Furthermore, in retrieving the data, served in serial because only one local row buffer can connect to the global data line to send the data out. ???
Finally, the data set is not large enough to saturate the capacity of the Membrane device. From the above analysis, we conclude that SALP=4 balances the performance and overhead the best for both Membrane-V/H.



==> Membrane/Sections/Results_2.tex <==
\section{Results-2 - New }
\label{sec:results_2}

\begin{figure}
\centering 
    \includegraphics[width=\linewidth]{Membrane/Result_2_Figures/End-To-End Query Execution Time.pdf}
    \caption{End To end Query Execution Time vs PIM Design parameters (O) - Optimistic Data Placement (P) - Pessimistic Data Placement and SALP - Subarray Level Parallelism}
    \includegraphics[width=\linewidth]{Membrane/Result_2_Figures/Geomean Perf of all SSB Queries.pdf}
    \caption{Geomean Perf of All SSB Queries (Either one of the above two figures goes in but not both) }
\end{figure}

\begin{figure*}
\centering 
    \includegraphics[width=0.55\textwidth]{Membrane/Result_3_Figures/figure_01-ete_perf.pdf}
    \includegraphics[width=0.55\textwidth]{Membrane/Result_3_Figures/figure_02-scan_perf_pim_design.pdf}
    \caption{Fig-1 : Final}
\end{figure*}

\begin{figure}
    \includegraphics[width=0.75\linewidth]{Membrane/Result_2_Figures/Query Execution Breakdown-1.pdf}
    \caption{Query Selectivity vs Breakdown (Aggregates dominate overall and reduce when selectivity is very low)}
\end{figure}

\begin{figure}
    \includegraphics[width=\linewidth]{Membrane/Result_2_Figures/Query Execution Breakdown.pdf}
    \includegraphics[width=\linewidth]{Membrane/Result_2_Figures/End to End Query Latency Comparisons.pdf}
    \caption{End to End Query Evaluation (Membrane vs PIM Baseline) }
    \label{fig:E2E-ssb-query-latency-cpu-pim-comparisons}
\end{figure}

\begin{figure}
    \includegraphics[width=\linewidth]{Membrane/Result_2_Figures/Single Bank vs All Bank.pdf}
    \caption{Performance across different PIM Configurations to SCAN one SSB Scale Factor-100 Database Column}
    \label{fig:salp_area_overhead}
\end{figure}

\begin{figure}
    \includegraphics[width=\linewidth]{Membrane/Result_2_Figures/End to End Perf. Per Area Across DRAM Heirarchy.pdf}
    \caption{End to End Perf Per Area Estimation at different DRAM hierarchies}
    \label{fig:salp_area_overhead}
\end{figure}

\begin{figure}
    \includegraphics[width=\linewidth]{Membrane/Result_2_Figures/Query Excecution Breakdown - Simple.pdf}
    \caption{Query Execution Breakdown across the different DRAM heirarchies}
    \label{fig:salp_area_overhead}
\end{figure}




\subsection{Observation - 1 : SCAN Performance improves as we travel down the DRAM heirarchy (Rank -> Bank -> Subarray)}
The DRAM is organized into a hierarchical structure consisting of ranks, banks, subarrays, and rows/columns. This structure is designed to balance tradeoffs and achieve high density while offering reasonable latency in terms of load/store performance. Generally, the number of units at each level increases as you go down the hierarchy, while the capacity per unit at each level decreases. For example, at the rank level, the amount of parallelism is typically equal to 4 ranks, which represents the number of ranks available at a single channel. At the row/column level, the number of rows and columns can vary from 1024 to 64k. In a single rank, the capacity can be as high as 16 GByte, while at a row level, you can only accommodate roughly 8192 bits per subarray.

Introducing PIM-capable compute elements at each of these levels presents a series of opportunities and limitations. We also need to consider the manufacturing constraints associated with each level. Introducing compute elements at the rank level is relatively easier from the manufacturing perspective since it can be mounted as a separate logic chip that interfaces with the DRAM chips through a buffer, similar to the AxDIMM design. A Processing Element at Rank-level would have access to a relatively large amount of data to address within its local space and could support more complex operations with sophisticated hardware structures such as caches, registers, and vector units. However, the amount of parallelism available at rank-level is relatively lower and can vary from 4-32 (with 4 ranks considered per channel).

There have been a number of bank-level memory products accommodating PIM capabilities in recent years, such as the Aquabolt, UPMEM, and SK Hynix AI memory. Prior works exploring this design space include (cite BLIMP). Conventionally, banks are considered to be independent of one another, with only the datapath being shared commonly among all the banks within a chip. Hence, banks could provide a reasonable degree of parallelism when leveraged accurately, provided that the data is not traveling across the datapath, which is a common resource contended among all the banks. There can be between 4-16 banks per rank, and generally, these offer an order of magnitude higher parallelism than what is available at the rank level. However, area and manufacturing constraints could limit the banks from having large extraneous hardware to support complex operations.

Further down the hierarchy, we are presented with the subarray level, where there can be more than 4 or 16 subarrays per bank, depending on the DRAM configuration used and the number of memory channels available. This level presents another order of magnitude higher parallelism compared to the bank level, but it again suffers from area and manufacturing constraints that can limit the implementation of complex hardware structures. However, the subarray level could be considered as a potential massively parallel architecture with tens of thousands of execution units.

In our experimental evaluation, we quantified the SCAN performance of each level within the DRAM hierarchy. We considered the time taken to perform a single columnar scan by PIM elements at each level to quantify the performance. For this experiment, we used a single SSB (Scale Factor-100) denormalized column containing 600,038,146 elements of 16-bits each, which is representative of most of the columns present within the given input dataset.The DRAM organized into a heirarchy of ranks, banks, subarrays and rows/columns. The DRAM designers and vendors have arrived at this heirarchical structure to balance the tradeoffs and achieve a high density while also offerring reasonable latency in terms of load/store performance. The general trend is that the number units at each level increases as one goes down while the capacity per unit at each level reduces. For ex. at rank-level, the amount of parallelism is generally equal to 4 ranks which represents the number of ranks available at a single channel while at row-column level, we observe that the number of rows and columns can vary from 1024 to 64k. In a single rank the capacity can be as high as 16 GByte while at a row-level one can only accomodate roughly 8192 bits per subarray. 

Introducing PIM-capable compute elements at each of these levels presents a series of oppurtunities and limitations. We also need to take into account the manufacturing constraints associated with each level. Introducing compute elements at the rank-level is relatively easier from the manufacturing perspective since it can be mounted as a separate logic chip which can interface with the DRAM chips through a buffer similar to the AxDIMM (TODO cite) design. A Processing Element (PE) at Rank-level would have access to relatively large amount of data to address within its local space and could support more complex operations with sophisticated hardware structures such as caches, registers and vector units. However, the amount of parallelism available at rank-level is relatively lower and and can vary from 4 - 32 (with 4 ranks considered per channel). 

There have been a number of bank-level memory products accomodating PIM capabilities in the recent years such as the Aquabolt, UPMEM, SK Hynix AI memory. There have been prior works exploring this design space such as (cite BLIMP). Conventionally banks are considered to be independent of one another with only the datapath being shared commonly amongst all the banks within a chip. Hence, banks too could provide a reasonable degree of parallelism when leveraged accurately and provided that the data is not travelling across the datapath, since that being a common resource contended amongst all the banks. There can be between 4-16 banks per rank and generally these offer an order of magnitude higher parallelism than what is available at the rank-level. However, area and manufacturing constraints could limit the banks from having large extraneous hardware to support complex operations. 

Further down the hierarchy, we are presented with the subarray-level, where there can be more than 4 or 16 subarrays per bank. This is entirely dependent on the DRAM configuration and there can be even more number of subarrays per bank. Hence, one is presented with anywhere between 8k to 64k subarrays depending on the DRAM configuration used and the number of memory channels available. Although the subarray-level again presents another level of magnitude higher parallelism when compared to bank-level, it again suffers from area and manufacturing constraints that can limit complex hardware structures from being implements. However, subarray-level could be considered as a potential massively parallel architecture with tens of thousands of execution units.

In our experimental evaluation, we wanted to quantify the SCAN performance of each level within the DRAM hierarchy and we consider the time taken to perform a single columnar scan by PIM elements at each level to quantify the performance at each level. For this experiment, we considered a single SSB (Scale Factor-100) denormalized column containing 600,038,146 elements of 16-bits each. This is representative of most of the columns present within the given input dataset. 

During our analysis, we discovered that subarray-level PIM architectures offer several design space parameters to consider, due to their fine-grained nature. We evaluated the following parameters at the subarray-level: 

(i) Scalar vs. Vector PE - Given the vast internal bandwidth available at the Row Buffer level, we could choose between a scalar processing element fed with a single word at a time or a series of processing elements directly connected to the row-buffer that execute comparison operations in a single execution cycle.

(ii) Data Placement - We could assume either one Compute Slice placed per bank or a Compute Slice placed at each of the subarrays. However, when using the LISA mechanism instead of the narrow bus interface to bring data to the Compute Slice, it introduces a non-uniform access (NUMA) phenomenon between the subarrays and the CS. Input data might either follow the most pessimistic data placement policy or the optimistic data placement policy, which directly affects performance. More time would be spent on LISA hops in the former scenario.

(iii) Subarray-level Parallelism - We could have multiple Compute Slices per bank activated in parallel to accelerate the SCAN performance.

At the bank and rank-level, DRAM accesses are at a coarser granularity and thus, there is very little room for the design space exploration of different parameters since the data is always fed off the narrow global bitlines emanating out. We could operate in the All-Bank (AB) mode or in a Single Bank (SB) mode at the bank-level, but the same option is not present at the rank-level since all the banks share the same datapath and only one can be used to feed the rank-level processing element (PE).

Note that the subarray scalar vs vector comparisons were done with SALP-1 to assess the performance of these configurations. We observe that the vector-variant has 128x the area overhead compared to the scalar-variant, yet offers approximately 20.5% to 22.3% improvement in performance. We concluded that there were minimal returns in adopting a vector-variant of subarray-level PE and moved ahead with further evaluations. Therefore, all the Subarray-level Parallelism (SALP) used in the figure-TODO are of scalar variant. The data placement of representing optimistic and pessimistic scenarios is marked as (O) and (P) respectively in each configuration to represent the upper and lower bounds of performance related to these parameters. In the SALP analysis, we observe that SALP-2, 3, and 4 offer 10.8% to 16%, 17.14% to 24.3%, 22.3% to 29.85% improvements over SALP-1. Furthermore, in the performance per area (PPA) measurements as shown in Fig - TODO, we observe that all the SALP levels have equivalent PPA numbers. Therefore, we decided to pick SALP-4 as an average value to best represent the subarray-level architectures in future comparisons against the bank and rank-level architectures as shown in Fig - TODO.

There is a 21.4% performance degradation while going from the subarray-level (SALP-4) to bank-level. However, we observe that Bank-level architectures offer significantly higher PPA when compared to the subarray-level, specifically 3.76x in SB mode and 7.1x in All-Bank mode. Note that for equivalent comparisons, we compare the single-bank bank-level against the single-bank variant at subarray-level (where a single bank in DRAM is enhanced with subarray-level PIM PEs).

Rank-level has a significant degradation in performance (of around 2.2x) when compared against the all-bank mode in SCAN performance.

End to End Results Comparison - TBD - Akhil (repeat the same story for End to End results)

\subsection{Observation - 2 : An All-Bank PIM mode offers reasonable performance in end-to-end query latency while the SB Bank-level offers reasonable }

We observe a strong trend wherein the All-Bank mode is generally highly performant than the Single-Bank mode across the board. Even the least-perform PIM configuration can surpass the best-performing PIM configuration in Single Bank (SB) mode. 

However, the performance improvement can also come with large increases in the area overhead of these PIM units. The figure-(TODO) details that the AB mode and SB mode having identical performance-per-area numbers. Of particular importance to note is that the massive parallelism provided by activating multiple banks at bank-level far outpaces even subarray-level parallelism available across the single bank mode. Hence, adopting a bank-level all-bank mode approach could be a feasible alternative to having large subarray-level parallelism restricted to certain banks provided the workload can support it. The All-Bank mode is also shown to work in modern PIM architectures such as the (cite HBM-PIM work) where it was implemented by discarding the "Ba" (Bank) and "Bg" (Bank-group) parts of a memory address.

\subsection{Observation - 3 : Bank-level is a sweet spot in terms of SCAN performance}

We observe that the DRAM heirarchies are subjected different constraints at each level and thus, any placement of PIM processing elements (PEs) too is oriented around these constraints. Subarray-level in particular provides various design space points to consider when evaluating its performance. At higher DRAM heirarchies such as the bank-level, rank-level or the channel-level, the degree of abstraction is relatively high such that it has predictable behaviours and lesser design space parameters to wrestle with. Amongst the many possible issues, we aimed to perform an exhaustive design space analysis at the subarray-level and considered the following parameters while evaluating - 

- The following parameters are explored in subarray-level

 - Compute Element configuration - Scalar (single 8-bit word) vs Vector (8192-bit wide)
	
 - Data Placement - Pessimistic (farthest from Compute Slice) vs. Optimistic (nearest)
	
 - Subarray-level Parallelism - We vary the number of simultaneous subarrays executing compute instructions from 1, 2, 4, 8 

- Overall beyond SALP-4 we see diminishing returns

- Bank-level offers reasonable degree of performance improvement

\subsection{Observation - 4 : SCAN performance is close to ideal value in terms of End-To-End Evaluation}

- We see that the aggregate operation dominates the operations

\subsection{Observation - 5 : The Performance Per Area benefits the Single Bank architectures over the All-Bank Architectures.}

- Show the PPA of this SB mode and AB mode

- Talk about the runtime query breakdown

\subsection{Observation - 6 : Rank-level offers free performance that is least intrusive to the DRAM}

- Micron comments for this particular aspect

\subsection{Area and Energy Analysis}
\kk{}
\subsection{Energy Analysis}

\subsection{Comparison with Alternative Architectures}

==> Membrane/Sections/Results_3.tex <==
\section{Results - 3}


\begin{figure*}
\centering 
    \includegraphics[width=\linewidth]{Membrane/Result_3_Figures/figure_01-ete_perf.pdf}
    \caption{End-to-End Latency Comparison of Membrane PIM architecture against various CPU baselines }
    \label{fig:End-to-End Latency Comparison of Membrane PIM architecture against various CPU baselines }
\end{figure*}

\begin{figure}
\centering 
    \includegraphics[width=\linewidth]{Membrane/Result_3_Figures/figure_09-membrane_area.pdf}
    \caption{Area estimate for different Membrane PIM configurations}
    \label{fig:Area estimate for different Membrane PIM configurations}
\end{figure}

\begin{figure}
\centering 
    \includegraphics[width=\linewidth]{Membrane/Result_3_Figures/figure_05-area_perf.pdf}
    \caption{Performance per area (PPA) for different Membrane configurations}
    \label{fig:Performance per area (PPA) for different Membrane configurations}
\end{figure}

\begin{figure}
\centering 
    \includegraphics[width=\linewidth]{Membrane/Result_3_Figures/figure_08-salp_area.pdf}
    \caption{Area estimate for differenet Subarray-level Parallelism levels}
    \label{fig:area-salp}
\end{figure}

\begin{figure}
\centering 
    \includegraphics[width=\linewidth]{Membrane/Result_3_Figures/figure_10-membrane_power.pdf}
    \caption{Power estimate for Membrane PIM configurations}
    \label{fig:Power estimate for Membrane PIM configurations}
\end{figure}



In Figure-TODO, we provide the speedup values in comparison to each of the baselines. However, we must note that comparing the DuckDB database engines is unfair due to the various other management tasks it performs besides executing the actual query. Nonetheless, we included it in the figure for reference to real-world implementations. The ideal time only takes into consideration the memory access-related timings when executed by DuckDB, while the AVX-512 time refers to the hyper-optimized SIMD-accelerated C++ implementation whose details were provided in the previous section-TODO. DuckDB can run either with a WideTable denormalized input dataset (eliminating JOINs) or a plain version that performs JOINs during query execution.

We compared the SALP-8 (subarray-level parallelism with 8 Compute Slices per bank), bank-level and rank-level PIM configurations. The subarray-level and bank-level configurations can support both Single Bank (SB) mode and All-Bank (AB) mode, while the rank-level can only function in single-bank mode or its native functioning mode. Our observation shows that the lower levels of the DRAM hierarchy provide better end-to-end speedups against the hyper-optimized baseline. These speedups decrease as one goes higher up the DRAM hierarchy until the rank-level. We observe very marginal improvements in end-to-end results especially related to the optimistic and pessimistic data placements in subarray-level PIM configurations. To recap, data is brought into the compute slices from other subarrays through LISA mechanism and there exists a possibility that certain subarrays might have to do more LISA hops (pessimistic placement) and some lesser hops(optimistic placement) to access the compute slices. 

The Fig-\ref{fig:Area estimate for different Membrane PIM configurations} and Fig-\ref{fig:area-salp} provides the Area results. To gain a better understanding of the area breakdown, we analyzed the SALP-1 in AB mode, which is comparable to the Bank-level (in AB mode too) and contains similar number of Compute Slices. We compared it to the rank-level configuration. The area overheads are reported as a percentage increase over the existing DRAM die area obtained in the CACTI, as explained in Section-\ref{sec:methodology}. The rank-level has the least area overhead, while the area increases as we move towards the subarray-level. Although the bank-level and SALP-1 have the same number of Compute Slices, the subarray-level has a larger area overhead due to the addition of an extra walker to buffer the input data from source subarrays and then sequentially feed it into the comparators. This additional walker is not required in the case of Bank-level units as they operate on the data coming out of the global bitlines directly. Moreover, within the subarray-level configurations, one can vary the amount of available parallelism from 1 to 8, and the introduction of multiple Compute Slices to tap into this subarray-level parallelism would incur higher area costs with the increasing parallelism levels. However, it is important to note that this increase is not linear in nature since a significant portion of the area cost is borne by the introduction of isolation transistors to support the LISA mechanism, and this cost remains almost constant even with the increasing number of Compute Slices introduced into the subarrays.

Regarding the rank-level architecture, one can consider the area overhead to be almost free since, unlike bank-level and subarray-level architectures, it does not require in-situ placement of PIM elements within the DRAM dies. Instead, it can be mounted outside the DRAM die, similar to that followed by the AxDIMM \cite{AxDIMM}. This does not affect the memory capacity and is also relatively easier from the device integration perspective.

The figure provided in Fig-\ref{fig:Power estimate for Membrane PIM configurations} shows the increased dynamic power consumption when the device is performing PIM computations. We observed that the subarray-level configuration consumed more power than the bank-level configuration because of the presence of an extra walker at the subarray-level required to buffer and sequentially feed the subarray row data into the comparators. The bank-level configuration does not require this walker as it receives data incoming from the global bitlines. However, we found that the power associated with these global bitlines can be significantly higher than that associated with an entire walker. The rank-level configuration has an order of magnitude higher dynamic power consumption since the data buses from the chips to rank-level processing elements (PEs) consume a lot of power. The longer length of the traces from the chips to the PEs and the associated delays contribute to higher dynamic power consumption at the rank-levels.

\subsection{Insights}

After a thorough analysis of the design space which considered various DRAM parameters and PIM configurations within each of these memory hierarchies, several interesting insights have been provided, which are detailed below.

\begin{enumerate}

\item \textbf{Rank-level Architecture Tradeoffs.} Based on the performance per area values reported in Fig-\ref{fig:Performance per area (PPA) for different Membrane configurations}, it can be concluded that the rank-level offers an extremely valuable proposition considering the various very high performance obtained relative to its minor area overheads. As discussed earlier, one could consider the area overheads associated with the rank-level to be practically zero since the processing elements at this level are mounted externally to the DRAM chips without sacrificing the memory capacity. However, it is also to be noted that the end-to-end speedup in SSB Benchmarks \cite{ssbbenchmark} offered by this architecture, as reported in Fig-TODO, is relatively smaller at 1.3x against the baseline. Hence, when query latency is an important criterion to be considered, one could resort to more fine-grained PIM architectures such as those present at the subarray-level and bank-level. This also presents another interesting conclusion that one could leverage the nearly-free rank-level parallelism to accelerate analytical workloads albeit by a modest 1.3x.

\item \textbf{Query performance.} in a Membrane PIM-based query processing scenario can be broken down into two major parts: filtering operations and materialization and aggregation. The filtering operation is executed on PIM-capable memory hardware, while the materialization and aggregation phase is executed on the CPU. Materialization involves reading the bitmaps and gathering filtered records to perform aggregate operations such as sorting, group by, average, sum, etc. 

In the All-Bank configurations, filter operations are almost negligible or executed with very minimal latency, usually taking only a few microseconds or milliseconds, as shown in Fig-\ref{fig:End-to-End Latency Comparison of Membrane PIM architecture against various CPU baselines}. The fastest possible PIM configuration in Fig-\ref{fig:E2E-ssb-query-latency-cpu-pim-comparisons} is close to the "Ideal (Aggregate-Only)" value, which indicates that the materialization and aggregation parts of the query are starting to dominate the query execution. Therefore, the time consumed by these operations represents the lower bound in terms of the best possible latency that can be achieved. 

However, a deeper analysis shows that the query selectivity, defined as the number of records selected after the filtering operation, directly dictates the amount of time spent in the above mentioned two operations. Query 3.4 in the SSB benchmark \ref{ssb} has the lowest selectivity, meaning that very few records are selected after the filtering operation, resulting in very little time being spent on the materialization and aggregation operations. 

Of course, the complexity of the aggregation operation, which can include grouping and sorting, could be a major factor as well. However, we have observed that there is a direct correlation between the query selectivity and the percentage of time spent on the above two operations.

\item \textbf{Subarray-level vs. Bank-Level PIM.} When comparing subarray-level PIM with bank-level PIM, subarray-level offers the best possible SCAN performance. However, the difference in terms of end-to-end speedup is relatively low between the two. In fact, the difference between the best performing PIM configurations at the subarray and bank-level results in a 5.2x and 4.1x speedup respectively over the baseline. When considering Performance per Area values as shown in Fig-\ref{fig:Performance per area (PPA) for different Membrane configurations}, it can be concluded that bank-level PIM might offer an optimal point  by providing the best possible latency while suffering from relatively minimal area overhead when compared to other PIM configurations. However, when low latency is the primary concern, subarray-level techniques can be utilized to achieve the lowest possible execution times for a given query.

\item \textbf{Single Bank vs. All Bank Mode.} The Aquabolt-XL introduced the All-Bank (AB) mode, which provides a significant boost in execution parallelism with a single DRAM command. However, this mode is only supported at the subarray-level and bank-level PIM configurations, not at the rank-level. After evaluating the AB and Single-Bank (SB) modes for SSB workloads, it was found that the AB mode on average reduces end-to-end latency by 1.9 times compared to the SB mode. However, this improvement in latency comes with a cost of approximately 7 times reduction in perf. per area (PPA) value as compared to the SB mode. Therefore, when latency is of primary concern, the AB mode can provide better performance, but with a higher area overhead concern. On the other hand, the SB mode offers reasonable performance with a relatively lower area overhead.

\end{enumerate}

==> Membrane/Sections/Sys_Integ_v2.tex <==
\section{System-Level Integration \underline{[DRAFT]}}
\ak{
Our goal while integrating Membrane with CPU was to extend the Host CPU’s capabilities to support and operate PIM-capable memories while proposing as many minimal changes as possible. To this end, we detail the following modifications on both sides of the memory bus i.e. DRAM-side (or DIMM-side) and Host side (CPU-side).}

\ak{\subsection{\textbf{DRAM-side Changes}}
On the DRAM-side of the memory bus, we identified that interleaving happens to be one of the major bottlenecks to implementing PIM-capable operations since the data layout is an important concern while executing these PIM operations. Specifically, we observe two types of interleaving, and we have detailed their effects on PIM operations and proposed changes to overcome the same. }

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{Membrane/Sys_Int_2_Figs/01_DRAM_Heirarchy.png}
    \caption{Chip-level Interleaving where 16-bits of each word are interleaved amongst 4 DRAM chips of a single rank 
(Picture taken from Half-DRAM paper for understanding and illustration purpose)}
    \label{fig:membrane_v}
    \vspace*{-.1in}
\end{figure}

\textbf{Chip-level Interleaving.} 
\mrtn{How can we integrate the de-interleaving unit (DU) without changing the DRAM command table? We need to mention that here. If we have to change that table (by introducing new command bit-lines, etc.), we're effectively proposing a change to the entire DDRx specification, which I don't think the reviewers will like.}
\ak{Refers to the portions of the 64-bit words accessed are interleaved amongst different DRAM chips. For ex. in x16 Chip configuration, 4 chips contribute 16 bits each to service a single 64-bit DRAM command. In a x8 configuration, 8 chips contribute 8 bits each to service a DRAM command. This might be problematic for the PIM operations since a single word (either 16 bit or 32-bit) might be dispersed amongst different chips and the PIM processing element resident within each chip might be only able to access the local portion of the word and not the complete word.
One could address this potential issue of chip-level interleaving either by using special algebraic methods such that the PIM processing element (PE) produces partial results which are combined together to form the final result. Or another solution is re-architect the DRAM configuration to prevent the interleaving and instead store the entire 64-bit word within a single DRAM chip. The former solution is either feasible for a smaller subset of operations or requires extensive post-processing of partial results to stitch together the final output while the latter solution severely affects the READ and WRITE bandwidths since the operations need multiple cycles into a single chip rather than spreading the data out across all the chips.
Hence, we propose to utilise a De-interleaving Unit (DU) on the DRAM side that collects the entire cacheline worth of READ / WRITE data and de-interleaves it before storing or reading from the DRAM chips. This unit is said to reside closer to the DIMM's register buffers and intercept the data being read or written to de-interleave it. This approach introduces an overhead with each READ / WRITE command as it now takes an additional 8 beats or four cycles since the interleaving unit first needs to buffer the entire cacheline's READ / WRITE data, perform the de-interleaving and then read it to either the memory controller or write it to the DRAM chips. However, we observe that the performance trade-off of utilising such an approach is highly beneficial and the overhead minimal considering that the primary motivation of adopting PIM is to reduce the number of such READ / WRITE commands and decrease the data movement across the memory bus. Since the de-interleaving unit resides close to the DIMM's register buffers rather than on the memory chips, it does not affect the memory capacity of the said chips.}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{Membrane/Sys_Int_2_Figs/02_MAT_Breakdown.png}
    \caption{Mat-level Interleaving where each subarray is broken down into multiple mats internally and all the mats combined contribute to a single cacheline worth of data (Half DRAM paper)}
    \label{fig:membrane_v}
    \vspace*{-.1in}
\end{figure}

\textbf{Mat-level Interleaving.} 
\mrtn{If mat-level interleaving is not impactful, do we even need to talk about it?}
\ak{Each subarray is further broken down into multiple matrices or mats where each mat is said to consist of its own local row decoder and local sense amplifier. This is done to improve the DRAM performance. Typically a mat is said to be of 512 x 512 row and bitline dimensions and a subarray would consist of 32 such mats in an x16 configuration. Hence, a single subarray in this configuration would contribute 128 bits to a cacheline and each mat would effectively contribute 4 bits. However, since the compute slice would access the data at row buffer granularity, the mat-level interleaving would not significantly affect its operation since the manner in which the data was stored is also the manner in which the data is read back into the local subarray processing element.}

\ak{\subsection{\textbf{Host-Side Changes}}
Typically before the system boots up, each channel is either configured to be in PIM-mode or main-memory mode. Some of the memory channels can be configured to be in PIM mode while others in the main memory mode depending on the user’s requirements and workloads. In the main-memory mode, the memory channel and the DIMM is said to behave in conventional load-store fashion without any modifications. However in the PIM-mode, the memory controller behaves in such a manner as to support the DIMM’s compute capabilities. During the bootup phase, one could configure the channel to be in either of the two modes. In case a main-memory option is chosen, the compute capable portions of the DIMM are turned off and the DIMM behaves in a conventional manner.}

\ak{However, the main changes to be introduced on the host-side to support the PIM-mode of operation are as follows -}

\ak{\textbf{Timing Changes} - As mentioned earlier, we introduce a De-interleaving Unit (DU) to change the layout of the cacheline's data that is being stored into each of the individual chips. Since the unit buffers and operates on the entire cacheline, it introduces a delay of extra 8 beats or 4 cycles on top of any READ / WRITE commands. Hence, the memory controller needs to take into account this delay while performing the DRAM operations.}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{Membrane/Sys_Int_2_Figs/03_Virt_Addr_Space.pdf}
    \caption{Virtual Memory with Membrane PIM}
    \label{fig:membrane_v}
    \vspace*{-.1in}
\end{figure}

\ak{\textbf{Virtual Memory.} Since portions of a system's DRAM memory are either configured to be in PIM mode or Main Memory Mode, the virtual memory needs to be made aware of this configuration and map the physical addresses appropriately. Specifically, when an application needs to store the database which requires the PIM operation, it needs to explicitly specify for it to be stored in channels that are under the PIM-mode. Towards this end, we introduce a single bit in the TLB called “PIM -bit” to indicate whether the specific page would need to be stored in the PIM memory region or main memory region.}

\ak{\textbf{Page Mapping.} For integrating Membrane's PIM memory, we recommend that the page size be either the size of a single subarray row or multiple of it. This is because the Membrane's Compute Slices (Membrane-H) generally work on an entire row-buffer's (or subarray row's) worth of contents and having multiple pages co-located in the same row-buffer would introduce erroneous results. We observed that all DDR4's configurations listed in the DramSim3 repository exhibited a subarray row size of 8 KB. Hence, we recommend that any page size be either 8 KB or a multiple of 8 KB. In case of larger page sizes i.e. multiple of subarray row size, a PIM Command Generator Unit (PCG - discussed at later sub-section) would introduce additional commands to activate other subarray rows and get it computed with the respective PIM processing elements. For example, If the Page Size is fixed at 2 MB (256 times the row buffer size of 8 KB), then the given page occupies multiple contiguous subarray rows and the PIM command generator would introduce new commands to get the entire page computed at the respective subarray-level PE. Furthermore, we observed that x86 manual dictates 3 different page sizes are currently supported i.e. 4 KB, 2 MB, 1 GB. We recommend the usage of the latter 2 of the available options. \mrtn{We may want to discuss how forcing the usage of big pages is acceptable for database workloads.} Moreover, usage of multiple page sizes within the same system too has been explored in prior works, hence a smaller page size for conventional main memory region while larger page size for PIM memory region could also be adopted.}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{Membrane/Sys_Int_2_Figs/04_PIM_System_Integr..pdf}
    \caption{PIM System Integration}
    \label{fig:membrane_v}
    \vspace*{-.1in}
\end{figure}\textbf{}

\textbf{PIM Command Generator (PCG) Unit.} \ak{We observe the introduction of special data mover and transformation accelerators such as Intel's DSA (Data Streaming Accelerator). These units relieve the CPU of performing basic data mover operations and also offload certain database specific operations such as SCANs as observed by Intel Analytics Accelerator (IAA) which works along with DSA for database workloads. This also demonstrates the existing need for such an unit to accelerate certain database specific operations which can primarily be bounded by I/O related operations in most cases.}
\ak{We propose PCG to be along the lines of DSA where the primary purpose of this on-chip unit sitting on the Host side is to offload the operation of issuing memory-related commands. The PCG dispatches PIM-specific commands to the memory controller once the TLB parses the physical page address. The primary job of PCG is to control and direct the memory controller to perform PIM operations. One of the primary motivations for introducing the PCG is the fact that CPUs traditionally lack fine-tuned access to the memory controller and also operate on the virtual addresses rather than physical addresses. Hence, it is difficult for the CPU to guide the PIM operations to respective channel, rank, and bank as required in the PIM scenario. Hence, the PCG is an intermediate unit that helps in orchestrating the PIM operations under the guidance of the CPU. The PCG can be programmed and controlled in a manner similar to that of the DSA by writing to specific registers.}


==> Membrane/Sections/Sys_Integ_ver3.tex <==
\section{System-Level Integration \underline{[DRAFT] Fig. \ref{fig:system_integration}}}

\begin{figure*}
    \centering
    \includegraphics[width=0.7\linewidth]{Membrane/Sys_Int_2_Figs/04_PIM_System_Integr.pdf}
    \caption{PIM System Integration}
    \label{fig:system_integration}
\end{figure*}

Our objective while proposing the system integration mechanism was to suggest as many minimal changes as possible while extending the existing system's functionality to support subarray-level PIM techniques. Processing-in-memory architectures have a significant degree of divergence from one another and propose different system integration mechanisms (cite MCN, Mutlu's PEI ISCA 2015 work, SIMDRAM). We find real-world implementations such as those of (cite Samsung AxDIMM, Aquabolt, UPMEM) that successfully integrate PIM capabilities with existing system architecture, albeit with their changes. Moreover, these are targetted at a coarser granularity, such as bank-level (UPMEM, HBM-PIM) or rank-level (AX-DIMM), and we see very few proposals in the realm of subarray-level techniques that have gained widespread adoption. Hence, we propose to build on the concepts of existing implementations, such as Samsung's Aquabolt and Intel's Data Streaming Accelerator (DSA), and propose extensions to them within the context of subarray-level PIM architecture design. The paper's primary objective is to explore subarray-level PIM techniques in the context of OLAP workloads and not necessarily expand the scope in search of the most optimum system architecture for such a scenario. Hence, with these conservative goals, we have proposed the following changes to integrate Membrane with the rest of the system framework. 


\textbf{1. Chip-level Interleaving.} We identified that interleaving is one of the major bottlenecks to implementing process-in-memory operations since data layout and placement are important concerns that dictate their execution.
	A single DRAM rank is constructed by grouping together multiple DRAM chips, forming a 64-bit memory interface. Any data transfer across such a setup involves breaking the data into smaller chunks and spreading it evenly amongst the multiple DRAM chips. For example, in an x8 DRAM configuration, there are eight chips, each with an 8-bit bus width interface and providing 8-bits each to service a 64-bit data transfer request. 
	This layout is potentially problematic for the PIM computations since the 64-bit word is not contiguous spatially within a single chip and is instead broken into smaller chunks and striped across multiple chips. Hence, any processing element (PE) residing within the DRAM chip would have access to its local portion of the data, not the entire word. 
	We could address this potential issue of chip-level interleaving in two ways. The first solution involves allowing the PIM elements to produce partial results by processing the available local data and, later, combining these partial results to form a single representative result. The second solution is to de-interleave and re-arrange the bits of an entire cacheline so that the necessary parts are placed together within a single DRAM chip. Amongst the two approaches, the former solution is feasible only for a small subset of operations and requires extensive post-processing of partial results to stitch together the final output. The latter approach is simpler and straightforward: a component named "De-Interleaving Unit (DU)" resides on-chip near the CPU, buffers the cacheline, and performs the de-interleaving process before writing it into the DRAM device or while reading from it.

\textbf{2. Virtual Page Size.} As detailed in the earlier section, the Membrane Compute Slice operates on the contents of an entire row buffer at once, and thus, we propose that the minimum size of a virtual page be equivalent to the size of a DRAM row buffer. This allows us to place the input data into a page and schedule PIM operations at a page-level granularity. In Membrane, we observe that the only PIM operation to be executed is the SCAN kernel, and the PIM units always read the data from these pages but never write into them. Hence, managing and operating these pages is simpler and straightforward in the context of Membrane's database workloads. 
	Membrane works in two modes, i.e. Single-Bank All-Rank (SBAR) Mode and All-Bank All-Rank (ABAR) Mode. To summarize, SBAR mode involves activating a page spread across all the available ranks, and a single bank within each rank holds a portion of the page. For an 8-channel configuration with four ranks per channel and an 8 KiB row buffer, a single page size would be 8 ch x 4 ra x 8 KiB = 256 KiB. In ABAR mode, a page is again spread across all the ranks, but this time with all the available banks within each rank holding a portion of the page. Considering the previous system configuration with four bank groups and four banks per bank group, the page size would be 4 MiB. 
	We recommend setting page sizes according to the Membrane modes (ABAR or SBAR) of operation that would be used. Interleaving pages in this manner may have possible effects on different workloads. However, exploring these implications falls outside the paper's scope, and we anticipate that systems leveraging Membrane PIM accelerators will be custom-configured to be optimized for maximum database performance.
 \mrtn{We may want to discuss how forcing the usage of big pages is acceptable for database workloads.}
	
\textbf{3. Virtualization.} The Membrane PIM architecture operates within the main memory's confines; hence, we need a mechanism to differentiate between the conventional and PIM-capable pages. PIM-capable pages are the ones that hold the data required for the PIM computations. We suggest introducing a bit in the TLB to indicate the PIM capability of a page.
Additionally, we propose that pages with PIM capability be designated as non-cacheable. This is because any PIM data if cached within one of the available cache levels, must be flushed before starting a PIM operation. However, since we operate on an OLAP database that is not frequently updated, the CPU requires only the filtered data to arrive at its caches to perform the final aggregation and result materialization step. Also, making the PIM-capable pages non-cacheable relieves us of further complexity associated with flushing PIM-capable cachelines before scheduling a PIM operation. 

\textbf{4. PIM Command Generator (PCG) Unit.} We perform LISA hops to push the data from its source subarray row location into the compute slice within the respective bank. The LISA hops are a series of memory controller commands to shift the data at a row-buffer granularity, and the number of LISA hops to the Compute Slice depends on the source row's location w.r.t the Compute Slice. A subarray row far from the compute slice might require more LISA hops compared to the one residing closer. Therefore, we introduce the PIM Command Generator (PCG) unit, which is designed to determine the subarray row's location using the physical memory address obtained from the Translation Lookaside Buffer (TLB). The PCG then initiates a sequence of LISA hop commands within the memory controller to facilitate the transfer of data into the Compute Slice. The PCG abstracts the Host CPU from physical address calculations related to LISA hops as the CPU does not have access to any physical addresses and only has virtual addresses available. Hence, we propose invoking the PCG after the TLB decodes a virtual address of a page to be operated in PIM mode. The PCG would orchestrate the LISA hops once the physical addresses are decoded from the TLB. 
	(not sure if this paragraph needs to be included)
	We proposed the PCG along the lines of Intel's DSA (Data Streaming Accelerator), whose primary objective is to issue a series of memory commands to relieve the CPU of trivial data copying and minor processing (CRC, fill, memcpy) operations. Indeed, IAA (Intel Analytics Accelerator) was developed leveraging DSA to carry out on-chip database filtering operations in close proximity to the CPU. In contrast, Membrane seeks to achieve the same goal without relying on access across the memory bus. A key difference between Intel's DSA (or IAA) and PCG is that the former operates on virtual addresses while the latter operates on physical addresses. 

\textbf{PIM Configuration.} Aquabolt proposes a series of reserved addresses that could be written into to configure the modes of operation and the instructions to be executed by the PIM subsystem. These are accessible and configurable using a simple DRAM write command by the Host CPU and can direct the PIM execution units more easily. We could write into a special register to toggle the PIM execution mode ON/OFF and describe the instructions and operands to execute. This space is demarcated as PIMCONF in the address space. Any userspace programs could access it without incurring the overhead of switching to kernel space every time to invoke a PIM execution.

\textbf{5. CPU - PIM Synchronization.} In our system integration scheme, we propose that while the PIM operations are occurring, any accesses to the DRAM memory system are said to be blocked. This is required because whether the Membrane operates in SBAR or ABAR mode, all the ranks are being leveraged to accelerate the scan kernel parallelly. Hence, any accesses from the CPU must be blocked until PIM commands are completed. As mentioned earlier, this could be a potential issue that might affect other applications, and hence, we envision a system adopting Membrane to be geared towards ensuring database-specific workloads. In our evaluations, the PIM operations for executing a query ran for less than <10 ms under an 8-channel configuration operating on scale factor-100 datasets. 

==> Membrane/Sections/Sys_Integrat_v1_old_.tex <==
\section{System-Level Integration}
\label{sec:system}

%\ak{\subsection{AK - This section requires a changes to correct some grammer and modify sentnces.}}

%\subsection{Host Integration}%(Change to Execution Orchestration?)}}
%Membrane's system integration consists of two levels of abstraction. First, we create a small set of Membrane-specific ISA instructions to expose the PIM functionalities that can be expressed by a DBMS developer. Second, we add logic in the DRAM controller to further decompose these new ISA instructions into DRAM commands specific to each Membrane (V/H) architecture. 

Membrane's system integration consists of two levels of abstraction. First, a small set of Membrane-specific ISA instructions expose the PIM functionalities that can be used by a programmer. Second, logic in the {DRAM controller}  is used to further decompose these new ISA instructions to DRAM-specific commands for each Membrane (V/H) architecture. 

\textbf{Membrane ISA.}
There are three main types of Membrane ISA instructions: \emph{predicate}, \emph{data movement}, and \emph{configuration} instructions. Predicate instructions include equality and inequality flavors and take the predicate value, the type of predicate (e.g., equal, not equal, less than or equal, greater than or equal, between, etc.), and the target column to which to apply the predicate. Data movement instructions are typically used offline by the DBMS to orchestrate loading the WideTable into the PIM. (Since generating the WideTable is considered a fixed cost that is paid once, we decided not to add dedicated hardware to accelerate it.)

In order to maintain a reasonably user-friendly interface of the Membrane ISA instructions and to keep the instructions' encoding lightweight, we add eight internal column-operand names $c_0-c_7$ that can be used by the PIM instructions.\footnote{When a query operates on more than 8 columns, the query is divided into sub-queries.}
%, each with at most 8 columns, and executed separately.} 
Similar to existing vector-length agnostic ISAs which maintain the state of their vector register names using Control Status Registers~\cite{waterman14}, we augment the memory controllers with bookkeeping logic to keep track of the start address, size, layout, and bitwidth of each column operand. Then, data movement and predicate instructions addressing a specific column operand will read these data structures to generate addresses for the required DRAM commands. 

A DBMS would utilize the Membrane instructions as follows, assuming that space has been allocated in row-aligned blocks where each row spans all channels/banks/ranks---see below for more detail on this issue---and virtual-to-physical mappings have been established. 1) Use data movement instructions to load the WideTable into Membrane. This is a one-time cost for an analytics session. 2) Use configuration instructions or a system call to map specific columns from the WideTable that are used in the query to column operands $c_0-c_7$ by specifying the starting virtual address, size, layout, and bitwidth of the data elements. This column setup step performs translation so that the memory controller knows the starting physical address of the column---see below for more detail on support for virtual memory.  These column setup operations are broadcast to all memory controllers. 3) Call Membrane predicate instructions as part of the query execution to execute the selection operators in Membrane. For example, suppose we want to filter on d\_year and return lo\_date. We would set d\_year’s starting address, length, bitwidth, and data layout with a configuration instruction and map it to c\_0, and do the same with lo\_date and map it to c\_1.  Finally, we would execute a predicate instruction on c\_0 and project the masks on c\_1. If the RLU is present, the projection command is sent to the RLU.  If not, the projection requires the memory controller to fetch the bitmap produced by the predicate operation on c\_0 and use it to fetch the selected items. Again, these predicate instructions are broadcast to all memory controllers.

\textbf{Virtual Memory.}
%While older DBMSs manage physical memory directly, 
Modern DBMSs run on top of conventional operating systems and use the OS virtual memory management techniques. Traditional virtual memory has considerable flexibility in mapping virtual pages to physical frames in DRAM. But for subarray-level PIM, to maximize subarray parallelism during a scan, data used by the DBMS should be mapped in a ``breadth-first'' fashion across all the subarrays being used for PIM acceleration. Furthermore, to allow the memory controller to simply broadcast PIM commands to all channels/ranks/banks and subarrays, rather than sending a separate command to each subarray, we need to ensure that for any PIM operation, all subarrays participating in that PIM operation are working on the same row. The typical address interleaving helps with both these considerations: it spreads successive cache-lines across channels, ranks, and banks before returning to the next column positions in a given row of a given subarray. However, when a given row ``position'' is filled up across all the channels/ranks/banks, interleaving typically moves on to the next row in the same subarray ``position'' across the channels/ranks/banks.  This suggests that a system performing PIM acceleration would benefit from a slight change in the interleaving so that when one row is filled up across the channels/ranks/banks, the next row is in a different subarray. If the PIM architecture uses subarray groups, the interleaving should prioritize subarrays with the filter array, to avoid the overhead of the LISA data movement. Changing the interleaving in this way should not affect performance of regular applications.  It is also desirable that allocations for PIM should be in aligned units that fill an entire row across all the channels/ranks/banks.  This may require padding the end of the WideTable with some canary values.

%To deal with cases where the dataset used for PIM cannot fill a row and is not present in some subarrays, the PIM setup for a process requires sending a mask to the memory that sets up configuration bits that will mask off PIM commands to the non-participating subarrays. This requires each subarray to support these mask bits.

In Membrane, the PIM operation is driven by the memory controller in with PIM commands that operate on one row of DRAM at a time, where a row spans all channels/ranks/banks. This means that rows not used for PIM can be used for regular (non-PIM) data in the same or other processes. %However, to support efficient address translation for PIM, it is beneficial for the physical address range allocated for the WideTable to be contiguous.  

The PIM support in the virtual memory system consists of an allocation system call for the WideTable, with a descriptor for each column's size.  The allocator returns a descriptor with the starting virtual address for each column, and ensures that each column is placed in a contiguous, row-aligned region of physical memory.  If a satisfactory allocation cannot be made, the allocator can return an error or move other processes' data to free up sufficient space (this configuration choice is up to the system administrator.) The allocator records each column's virtual and physical starting address in a PIM mapping structure, so that when a column is specified as part of a PIM computation (see ``Membrane ISA'' above), the specified starting virtual address can be quickly mapped to a physical start address and the size can be checked.  If no valid mapping is found, a segmentation fault occurs.  This mapping can be a system call or---preferably---supported at user level with a new form of TLB for PIM, the PIM-TLB, that contains the column mappings. If the WideTable has too many columns to fit in the PIM-TLB, a TLB-miss will raise a PIM-TLB-fault that checks the table in the OS. 

%However, to ensure that each participating subarray has the same number of rows participating, data structures used for PIM must be padded accordingly, and the {\em data movement} instructions mentioned above must use the OS virtual memory system to convey physical address ranges to the memory controller. 

%This means that when a data structure such as the WideTable is allocated for use with PIM, a new flavor of PIM-mode memory allocation is needed that obeys these principles. The simplest approach is to support partitioning, in which an application can request a PIM partition of the desired size, that is distributed across the subarrays as outlined above. Data in the DBMS, or in other processes not using PIM, can use unallocated rows.  If multiple applications are using PIM, each partition will use a subset of the rows, with the partition spread across the subarrays. Note also that for V mode, enough rows must be allocated to support the V, column-major layout.

%It should return the degree of subarray parallelism that can be achieved so that the user-level program can determine whether to proceed. (In typical system configurations used for large-scale OLAP, the entire system will be dedicated to this purpose.)  

%A further concern is that the rows in a subarray may be wider than an OS page---e.g., a subarray row may be 8 KB for an OS that uses 4 KB pages. The memory allocator can either guarantee that successive pages in a row all hold DBMS pages that will be operated on together in PIM operations, or the PIM must discard results from unused portions of a row (with V) or stop walking the row at the page boundary (with H), and only save the bitmap from the portion(s) that are part of the PIM operation.\footnote{In V mode, operating on the entire row is harmless because the state in the subarray is not changed.} To avoid needing different state bits per row, a given subarray should be used so that all participating rows have the same occupancy of PIM pages.

%The above considerations suggest that in systems with PIM capability, the virtual memory system should allocate pages not used for PIM in a way that leaves space for PIM memory allocation to obey these principles and achieve sufficient subarray level parallelism. 


%\ak{\textbf{Virtualization} Membrane interfaced with the host is said to support virtualization. Membrane-H operates on one complete row buffer to perform predicate operation on a set of database records while Membrane-V requires multiple row buffers (due to vertical layout) to perform the same operation. Thus, it is advised that the page sizes be allocated accordingly and it is observed that modern processors are known to support large page sizes of upto 1 GB [TODO cite Intel Arch Software Dev Manual Vol 3.] which would be beneficial for sequential scan operations.  Since the CPU is not performing the scans itself but offloading it onto the PIM architecture at a page size granularity without the knowledge of their physical address, the virtualization is left unchanged. However, we propose changes to the memory controller to support interfacing with the PIM components to execute scan and gather operations in the following sections.  }

%\begin{figure}
%    \centering
%    \subfloat[Filtering with Membrane-H Architecture]{
%        \includegraphics[width=0.9\columnwidth]{Membrane/Sys Integration Figures/04_flow_diagram_v3.pdf}
%        %\caption{Membrane-H Overall Architecture}
%        \label{fig:Filtering with Membrane-H Architecture}
%        %\vspace*{-.21in}
%    }
%    \vspace*{1ex}

%    \subfloat[Filtering with Membrane-V Architecture]{
%        \centering
%        \includegraphics[width=0.8\columnwidth]{Membrane/Sys Integration Figures/03_Membrane_V_Execution_Flow_v3.pdf}
%        %\caption{Rank Level Processor \underline{AK TODO - Resize this }}
%        \label{fig:Rank Level Unit Breakdown}    
%        }
%    \caption{Execution Flow of Membrane’s different architectures with elements as described in Sections 3.2 and 3.1 for subfigures (a) and (b), respectively.} %\ak{Note Q. This diagram will be modelled along the discussed "Wisconsin" style execution flow. Is it too simple and to be removed if there are space constraints? Or would it help in visually understanding the picture in one go? }}
%    \label{fig:exe_flow}
%    \vspace*{-.22in}
%\end{figure}

%\ks{Added this example for clarity but we can cut  it if needed for space.}

%\sout{\textbf{PIM-CPU Data Transfer.}
%The output of a predicate instruction is a vector of bits for the Bitmask Mode (or values for the Data Push Mode). To support that, the DRAM controller includes one 64B buffer per memory channel to cache the output bitmask and an additional 2KB FIFO to cache the values for Data Push Mode.\footnote{2KB because a 64B fully-dense mask can potentially retrieve 64*8=512 values. The worst case value bitwidth is 32 bits.} These buffers enable a decoupled mode of execution where subblocks of the output vector are produced by the PIM while subblocks buffered in the memory controller are being fetched by the CPU.} 

%\sout{These buffers are sufficient to decouple the CPU and PIM without stalls. In the data push mode, the amount of data being pushed to the CPU is  dependent on the selectivity of the query being executed, with more data being pushed for queries that exhibit high selectivity. In our analysis, the largest volume of data transferred in the SSB query suite was for query 3.1, with 152 MB of dictionary-encoded data values traveling across the memory bus. This equates to around 0.0004\% of the DRAM bandwidth, %\sout{so the memory interface is not longer a bottleneck} 
%hence, the memory interface is observed to not experience any bottlenecks in our evaluations.
%In bitmask mode, processing the bitmask overlaps with data retrieval from the memory locations. }

%\sout{ data retrieval from the DRAM memory location takes significantly longer  than processing the bitmask. }
%\ak{AK: can we replace the final the final part of the last sentence with - where the latter takes signficantly longer than the former.}
%In both modes, we observed that the memory controller has negligible overhead when compared to the overall query execution time. 

%\ak{The system integration of the PIM memory with the Host plays an important role in driving the architecture, usage and performance cherctarstics of the design. There is a need to make PIM-capable memory be compatible with the existing Host architecture without significantly modifying it while at the same time extending it to support the enhanced PIM-memory. Hence, many of the changes proposed were motivated by the desire to strike a fine balance between compatibility and extending the capabilities. The system integration is different for each variant of Membrane since their modes of operation differ significantly. }

%\ak{Membrane-V - This mode primarily operates on late materialisation philosophy where bitmaps for all the database records scanned are collected and processed in the final stage to materialize the result. Hence, collecting and transferring these bitmaps to the CPU is the main task of the system integration. Afer performing a scan operation, bitmaps are produced on a per-attribute basis. Hence, the memory controller directs the PIM memory to store each bitmap in certain reserved addresses or pages after each attribute scan operation. Once all the scans are completed, the CPU reads these bitmaps from the reserved addresses and processes them further to materialise the result. Modern operating systems and hardware utilise similar mechanism to reserve certain address spaces for various reasons such as debugging drivers, privelage sepration, memory mapping etc. Prior works such as Damon have also utilised this in the PIM context. }

%\ak{Membrane-H - In the V variant the scanning and retrieving bitmap operations are entirely driven and dictated by the CPU but the same may not hold true for the H variant where data that is filtered out needs to be "pushed" from the PIM memory rather than being read out or "pulled" from the CPU. Thus, there are significant changes that need to be introduced into the H variant to account for this. Direct Cache Approach where CPU consumes the data injected by the Network Card directly into caches is a motivation to our sytem design for this variant. DCA is a well studied and mechanism with extensive optimisations and implementations already available that one could leverage with minor modifications to extend it to support PIM capabilities. Another interesting direction was investigated in Memory Channel Networks [TODO citation] that again aimed at utilising a variant of DCA approach to enable Rank-level PIM processing. It treats each rank or DIMM to be a separate node with its own network addresses to communicate with except that the PHY layer consists of DDR interface rather than the conventional ethernet interface. Although this provides several valuable advantages especially related to offloading applications majorly written for distributed computing domain, we optimise the design to reflect our focus on the OLAP database workload. }

%\ak{Generally the memory is organised into several channels, DIMMs and ranks. While the channels are independent and can be accessed parallely, the DIMM and ranks within each channel share the same data and address buses and hence need to be accesssed in a concurrent manner. Our key idea here is that while the memory controller performs an access on a certain DIMM/rank, the next cacheline of data can be kept ready by the RLP/subarray units by performing a SCAN and Gather operation in another DIMM/rank. By performing this pipelining of operations between several ranks and DIMMs, the memory controller is always kept busy and at the same time hiding the latency related to the SCAN and Gather operations performed by the RLP and subarray-level PIM elements.}

%\ak{The memory controller after reading the cacheline worth of data usually transfers it to the CPU via a DMA engine by updating the TX descriptor. [AK - TODO] Need some elaboration here about the RX / TX rings }

%\textcolor{blue}{
%\sout{\textbf{FIFO Buffer Synchronization.}
%The HW
%The FIFO buffers adopt a latency-insensitive interface with the use of \emph{ready} and \emph{valid} bits: when the memory controller has filled up the buffer with data, it sets the valid bit to 1; and when the CPU has consumed the data, it sets the ready bit to 1 to let the memory controller know that it is ready to consume the next value. To enable the data push mode, there is also the \emph{done} bit, set by the memory controller to indicate when there is no more data to be consumed by the CPU.}
%The SW (or how do we expose the interface to the SW)
%\sout{To expose this latency-insensitive mechanism to the CPU, the program uses Membrane-buffer specific load instructions to read data from the buffers. In Bitmask Mode, the CPU can read a bit as long as the valid bit is set. In Data Push Mode, since the number of values to be read depends on the selectivity of the predicate, the CPU will continue reading values (if the valid bit is set and) until the done bit is set. To read or set the ready/valid/done bits, the CPU reads or modifies memory-mapped registers using regular loads and stores. This is similar to the approach in \cite{dca}, which is widely used, except that we utilize a FIFO buffer and register bits to synchronize instead of interrupts and read/writes to the cache.} 
%}
 
%FIFO buffers need to be addressable, memory controller sets valid bit every cacheline size block is loaded into buffers, CPU unsets the bit when it has consumed it. To enable this sync, the code looks like a for-loop containing a filter instruction, a fence instruction, and the aggregation operator body.
%The buffers adopt a latency-insensitive interface with the use of \emph{ready} and \emph{valid} bits: when the memory controller has filled up the buffer with data, it sets the valid bit to 1; and when the CPU has consumed all the data, it sets the ready bit to 1 to let the memory controller know that it can refill the buffer with fresh data. %(helena: This can be suboptimal because if read/valid bits work at the granularity of buffer size, then Membrane cannot start filling up the buffers until the CPU has consumed the whole 64B/2kB buffer data. Instead, we know that the CPU will consume this data using SSE instructions that work at 128-bit granularity. To leverage that, we can change the meaning of the valid/ready bits to valid 1 means there is at least one bit/record and instead of a ready bit having a counter that the CPU updates to let Membrane know how many records it has consumed.)

%helena: I think paragraphs 1 and 2 of this section already explain this:
%The DRAM controller translates Membrane ISA instructions into sequences of DRAM-specific commands. The controller for Membrane-V will break down predicate instructions into DRAM commands to broadcast the comparand, read-and-compare commands, and mask writes into the subarray and dedicated buffer. Membrane-H will transform the predicate instructions into subarray reads, ALU-like instructions %as shown in Table-\ref{tab:instruction buffer format}%, 
%and writes of the output. Note that both microarchitectures utilize the dedicated bookkeeping structures in the memory controller to generate the appropriate addresses at each command. Membrane load and store instructions will work similarly to traditional loads and stores, with the added column operand state, which will be read to move the data in the expected layout.

%helena: this is too much information and it does not relate to reviewers' concerns?:
%\ak{During query execution, the memory controller issues a series of read commands to process elements at the subarray level. In the bitmask-mode, we use a setup similar to \cite{jaffar} where the partial bitmasks are flushed and written to pre-determined memory locations periodically. The memory controller can later retrieve this information and send it to the CPU. In the data-push mode, every time an element evaluates to true, Membrane-H can pull \textcolor{red}{pull --$>$ set?} the \textit{push\_data\_h} (see~\ref{membrane-H control unit}) signal high to indicate to the memory controller to retrieve the data from the subarray via the global data lines and send it to the CPU \textcolor{red}{Not clear who does the send -- the memory controller?}. If the data element does not pass the selection predicate \textcolor{red}{check this sentence carefully}, no changes are made to the signal and the memory controller issues the next successive read command to iterate over the next columnar data. For Membrane-V, the memory controller needs to carry out an extra step of reading the bitmap generated and retrieving the data from the main memory before pushing it to the CPU. }

%\textbf{PIM-CPU Data Transfer.}
%\ak{The system integration of the PIM memory with the Host plays a key role in driving the architecture, usage, and performance characteristics of the design. There is a need to make PIM-capable memory compatible with the existing Host architecture without significantly modifying it while at the same time extending it to support the enhanced PIM-memory. Hence, many of the changes proposed were motivated by the desire to strike a fine balance between compatibility and extending the capabilities. The system integration is different for each variant of Membrane since their modes of operation differ significantly. }

%KEEP FOR REBUTTAL
%\subsection{Operation Modes}
%\label{sec:operation_modes}
%The system integration is different for each variant of Membrane since their modes of operation differ significantly. %Early Materialization and Late Materialization modes will referred to as EM and LM modes respectively, in further parts of the document.

%\ak{\sout{\subsection{Late Materialisation with Membrane-V}}
%\sout{Membrane-V is relatively simpler in terms of system integration where only three major phases of query execution are present. In the initial phase, the PIM processing elements associated with subarray bitlines operate on database records laid out vertically to perform a SCAN operation. The result of the SCAN operation is reprented again in the form of a bitmap. These bitmaps are written to specially reserved memory addresses for later retrieval. Once all the database records are scanned for the necassary attributes, then the CPU retrives the bitmaps and processes them for aggregate operations. Here the SIMD capabilities of the CPU can accelerate the processing of these bitmaps significantly and a copy of the WideTable stored in the main memory can be used to retrieve database records of interest. Once the aggregate operations are performed, the CPU can materialise the result to complete the query execution. }}

%\textbf{Membrane-V.} - This mode primarily operates on late materialization philosophy where
%\textbf{Late Materialization (LM) with Membrane-V} 
%Membrane-V is relatively simpler in terms of system integration where only three major phases of query execution are present. 
%In the initial phase (\ding{182} Figure~\ref{fig:Rank Level Unit Breakdown}), the PIM processing elements associated with subarray bitlines operate on database records laid out vertically to perform a scan operation, producing a bitmap for each row.  These bitmaps are written to reserved memory addresses for later retrieval (\ding{183} Figure~\ref{fig:Rank Level Unit Breakdown}). Once all the database records are scanned for the necessary attributes, then the CPU retrieves the bitmaps and uses them for subsequent aggregation operations (\ding{184} Figure~\ref{fig:Rank Level Unit Breakdown}).
%\sout{The SIMD capabilities of the CPU can accelerate the processing of these bitmaps significantly and a copy of the WideTable stored in the main memory can be used to retrieve database records of interest. Once the aggregate operations are performed, the CPU can materialise the result to complete the query execution. This Late Materialization Mode is associated with Membrane-V.
%\sout{Although it is possible to use SIMD instructions, either by using vector indexed loads or vector predication, to process these bitmasks and fetch the associated data, it is not strictly necessary.}

%The modifications to system integration aspect revolves around collecting and transferring the bitmaps to the CPU. After performing a scan operation, bitmaps are produced on a per-attribute basis. Hence, 
%The memory controller  directs the PIM  to store the bitmap  in reserved pages. Modern operating systems and hardware utilize similar mechanisms to reserve certain address spaces for several reasons such as debugging drivers, privilege separation, memory mapping etc. Prior works such as \cite{jaffar} have also utilized this in the PIM context. 

%\textbf{Membrane-H.} - While in V variant
%\textbf{Early Materialization (EM) with Membrane-H.} 
%In the scan phase, WideTable records containing prejoined attributes are activated into the row buffer and scanned by the subarray-level PE successively to perform the required predicate operation (\ding{182} Figure~\ref{fig:Filtering with Membrane-H Architecture}). The smaller-length bitmaps generated from this scan operation are transferred to reserved pages, which are then retrieved by the respective Rank-Level Unit (RLU).\footnote{Even though both V and H produce bitmasks to reserved pages, the RLU approach only works for the H variant, because the data to be fetched are in the same rank, enabling early materialization.  In the case of V, the data to be fetched are in a separate copy of the WideTable, which may require fetching from different ranks.} The RLU generates read offsets to select the data that needs to be transferred to CPU for materializing the result.  Due to the structured nature of storing database records following a certain layout, it is easier for the RLU to calculate the necessary offsets for the data to be read (\ding{183} Figure~\ref{fig:Filtering with Membrane-H Architecture}), compared to having each subarray PE do so.


%\sout{Once the offsets are inserted into the READ queue, the RLU waits for the Memory Controller to service its Rank. The Memory Controller (MC) related to each channel services  4 ranks among two DIMMs. The Controller reads a cache line worth of data from each of its ranks in a round robin format (\ding{184} Figure~\ref{fig:Filtering with Membrane-H Architecture}). When the MC selects a specific rank, its RLU issues the READ command for the offsets present in its READ queue and a cache line worth of data is transferred to the MC.
%In typical (non-PIM) operation, a READ command fetches a cache line worth of data, which contains other data from neighboring addresses apart from the data of interest. The RLU needs to add some header bytes to indicate which of the bytes in the cache line actually hold the data necessary. Usually the DDR specification defines the order in which the bytes are burst out and this information is exchanged with the MC during the initial setup and training phase when the system boots up. The RLU can make use of the same information in the modified setup in the context of Membrane. The header usually consists of 1 bit per byte of cache line to indicate whether it contains valid data, hence we end up with 56 byte payload and 7 byte header and 1 byte remaining for potential future use.}

%\textcolor{blue}{Once the offsets are inserted into the READ queue, the RLU associated with each of the rank performs a gather operations and buffers the data before being read out by the memory controller (MC). The MC services each of the ranks within a channel in a round robin format (\ding{184} Figure~\ref{fig:Filtering with Membrane-H Architecture}) and collects the buffered data to be sent to the CPU.} 
% Akhil First Draft on DCA  AKHIL, WHEN YOU ARE DONE DRAFTING THIS, PLEASE MOVE IT TO SECTION 4

With the RLU, gathering and packing the data is performed on the DIMM side of the memory bus and benefits from rank-level parallelism.  To simplify the task of fetching the data from the RLU, a mechanism such as Intel's DDIO~\cite{ddio} approach could be extended to allow the RLU to push data into the last-level cache. In this way, the memory controller does not need to wait for the RLU to have a block of data ready. DDIO involves using a descriptor table as a means of specifying physical addresses that the I/O devices can write to within the last-level cache, thereby avoiding expensive DMA transfers. Once an I/O device performs a write, it is indicated to the CPU by an interrupt mechanism or polling (which would be more appropriate for Membrane). The CPU in turn updates the descriptor table to receive the next READ request while processing the just-read data. 
We  extend this mechanism in the context of Membrane by provisioning additional PIM-specific descriptor tables, allowing the RLU
%PIM device 
to push data from its memory to the CPU's last-level cache at preconfigured addresses. %as demonstrated in Memory Channel Networks \cite{mcn-dimm} 
Furthermore, because multiple RLUs share the interface to the CPU, they can pipeline their writes to the CPU and hide delays at individual RLUs, e.g. because the data being gathered are sparse.
%Due to the predictable periodic intervals of transmission from PIM, \ks{Are we sure this is predictable? For sparse data, we don't know how many row accesses the RLU will need to make to gather a blob of data} any overhead suffered from the mechanism is hidden by simultaneously receiving the next cache line of data while buffering and transmitting the previous cache lines in a pipelined fashion. \ks{The preceding sentence is hard to follow. I can't understand the pipeline being described.} After the cache line is transferred from the PIM device to the CPU, %(\ding{185} Figure~\ref{fig:Filtering with Membrane-H Architecture}), 
%further aggregation and materialization operations are performed to completion. 
%and the results materialized early with this mode. 

%\hc{\textbf{Promote text below as a subsection inside Early Materialization?)}}

%\sout{While in the Late Materialization variant the scanning and retrieving bitmap operations were  driven  by the CPU, the same may not hold true for the H variant, where data that is selected based on a scan operation needs to be "pushed" from the PIM memory rather than being read out or "pulled" from CPU. Thus, there are significant changes that need to be introduced into the H variant to account for this. DCA or Direct Cache Access refers to the mechanism of inserting data directly into the cache by  IO devices such as network interface cards, from where CPU reads it for further processing. DCA has been widely implemented by major vendors over the past years, with various names such as Intel DDIO \cite{ddio} and ARM Cache Stashing \cite{arm-cache-stashing}. Several works such as (TODO - citations required) have studied the effects and optimization techniques related to DCA to seamlessly integrate it with the OS stack to get better performance. These mechanisms can be leveraged in the PIM context for pushing the data from the Membrane-H DIMM to the CPU. }
%\sout{Memory Channel Networks (MCN) \cite{mcn-dimm} proposes changes to the network subsystem to achieve this where DIMMs on a memory channel appear as independent nodes connected with an Ethernet link, except instead of the Ethernet PHY interface, it is the DDR interface. This has several benefits, because only minor modifications to the overall architecture are required to support transparent offloading of computation and retrieval of data from these PIM-capable DIMMs.} 

%\sout{Memory Channel Network (MCN) \cite{mcn-dimm} is one such prior work that proposes transperent offloading of computation and retrieval of data from PIM memory by making modifications to the network subsystem to support DCA. Our system integration builds on this mechanism to interface with Membrane-H and "push" data in periodic intervals to the CPU caches. Due to the predictable periodic intervals of transmission from PIM, any overhead suffered from the mechanism is hidden by simultaneously reciveing the next cacheline of data while bufferring and transmitting the previous cache lines in a pipelined fashion.}
%\sout{Our system integration employs a similar mechanism to receive data from the RLP processor and insert it into the CPU caches for further processing. Furthermore, since the Memory Controller (MC) sends data in periodic intervals from PIM memory into the CPU caches, we could hide any overhead latencies incurred by the mechanism by simultaneously receiving the next cache line of data while buffering and transmitting the previous cache line in a pipelined fashion. As the CPU receives each cache line of data, it cab starts processing it.}

%\sout{The overhead related to performing a scan on the subarrays and the bitmaps processing by the RLP can be hidden by pipelining the operations. As shown in the figure - ??, as the MC is performing a READ on a specific rank, other ranks could perform the scan and gather operation necassary and be ready with offsets to fill the data for the next cacheline. In some of the scenarios when the RLP is not ready with the data but the MC happens to service its ranks, the RLP can send out cacheline full of NULL or zero values and indicate the same in the header portion of the cacheline. In other scenarios, more than one cacheline is needed to transmit data related to results of a bitmap, and the RLP might need to wait and do multiple transmissions with the MC. In this manner the flow control between the MC and the RLP is achieved. }

%TODO(add text that walks the reader over a Figure describing the execution flow for V and H).

%\ak{{\subsection{Early Materialisation with Membrane-H}}
%\sout{As described in the Architecture section about the details of the Membrane-H, the overall query execution is broken down into 4-stages and pipelined to hide latencies related to each stage. Consider execution of SSB Q1.1}}
%SELECT SUM(lo_extendedprice*lo_discount) AS revenue 
%FROM lineorder, ddate
%WHERE lo_orderdate = d_datekey
%  AND d_year = 1993
%  AND lo_discount BETWEEN 1 AND 3
%  AND lo_quantity < 25;

%\sout{In the above example, the the WideTable already has the prejoined database attributes stored in each of the subarrays. In the Scan Phase, subarray rows containing d\_year, lo\_discount and lo\_quantity are brought into the row buffer and scanned by the subarray-level PE to perform the required predicate operations successively on each of the database attributes. After scanning database records for each attribute, a bitmap is constructed and sent to the Rank-Level Processor. For the above mentioned query 3 separate bitmaps are constructed for each of the database attributes and the size of each bitmap is related to how many database records can fit into a row buffer or page. Based on our analysis of SSB dataset usually less than 256 database records can fit into a single 8 KB page depending on the data layouts, hence a bitmap of approximate length 256-bits or lower is constructed for each attribute scan. }

%\ak{\sout{These seperate bitmaps are collected in the Rank-Level Processor (RLP) and an AND operation is performed to indicate which of the database records evaluated to true for all attribute scans. After resolving the bitmap, the RLP generates offsets to fetch lo\_extendedprice and lo\_discount for database records that evaluated to true and inserts these memory addresses into the READ buffer. Due to the structured nature of storing database records following a certain layout, it is easier for the RLP to calculate the necassary offsets to READ. }}

%\ak{\sout{Once the offsets are inserted into the READ queue, the RLP waits for the Memory Controller to service its Rank. The Memory Controller (MC) related to each channel services is further split into 4 ranks amongst two DIMMs each. The Controller reads a cacheline worth of data form each of its ranks in a round robin format. When the MC selects a specific rank, its RLP issues the READ command for the offsets present in its READ queue and a cacheline worth of data is said to flow into the MC. Usually when a READ command is issued a cacheline worth of data is burst into the MC which contains other data from neighbouring addresses apart from the data of interest. The RLP needs to add some header bytes to indicate which of the bytes in the cacheline actually hold the data necassary. Usually the DDR specfication holds order in which the bytes are burst out and this information is exchanged with the MC during the initial setup and training phase when the system boots up. The RLP can make use of the same information in the modified setup in the context of Membrane. The header usually conists of 1 bit per byte of cacheline to indicate whether its a valid data or not, hence we end up with 56 byte payload and 7 byte header and 1 byte remaining that could be utilised for any other purposes. }}

%\ak{\sout{The overhead related to performing a SCAN on the subarrays and the bitmaps processing by the RLP can be hidden by pipelining the operations. As shown in the figure - ??, as the MC is performing a READ on a specific rank, other ranks could perform the SCAN and GATHER operation necassary and be ready with offsets to fill the data for the next cacheline. In some of the scenarios when the RLP is not ready with the data but the MC happens to service its ranks, the RLP can send out cacheline full of NULL or zero values and indicate the same in the header portion of the cacheline. In other scenarios, more than one cacheline is needed to transmit data related to results of a bitmap, and the RLP might need to wait and do multiple transmissions with the MC. In this manner the flow control between the MC and the RLP is achieved. }}

%\ak{\sout{Once the cacheline reaches the MC, it needs to travel up to CPU caches and we employ a DCA-style mechanism that has been discussed in the prior section.}} %DCA or Direct Cache Access refers to mechanism of inserting data directly into the cache (usually LLC) by the IO devices such as the NICs from where the CPU reads it for further processing. DCA has been widely implemented in several chips of major vendors over the past several years with various names such as DDIO by Intel and Cache Stashing by Arm. Several works such as {TODO - citations required} have studied the effects and optmisation techniques related DCA to seamlessly integrate it with the OS stack and extract the maximum performance. These mechanisms can be leveraged in our PIM setting for pushing the data from the PIM to the CPU. MCN approach proposes changes to network subsytem to achieve this where DIMMs on a memory channel appear as independent nodes connected with an ethernet link except instead of ethernet PHY layer, it is the DDR layer. This has several benefits as minor modifications to the overall architecture are required to support transperent offloading of computation and retrieval of data from these PIM-capable DIMMs. Our system integration employs similar mechanism to recieve data from the RLP processor and insert it into the CPU caches for further processing. Furthermore since the MC sends data in periodic intervals into the CPU caches, we could hide any overhead latencies incurred by this mechanism by recieving the next cacheline of data while bufferring and transmitting the previous cacheline in a pipelined fashion.}

%\ak{\sout{Figure ?? shows overview of integrating the DCA mechanism to push data from the MC to the CPU. The descriptor tables usually contain addresses for the MC to write into. Once the data is recieved in the CPU caches, the application program could pick it and perform the necassary aggregate and post-processing operations to materialise the results. }}

%\ak{\sout{\subsection{Late Materialisation with Membrane-V}}
%\sout{Membrane-V is relatively simpler in terms of system integration where only three major phases of query execution are present. In the initial phase, the PIM processing elements associated with subarray bitlines operate on database records laid out vertically to perform a SCAN operation. The result of the SCAN operation is reprented again in the form of a bitmap. These bitmaps are written to specially reserved memory addresses for later retrieval. Once all the database records are scanned for the necassary attributes, then the CPU retrives the bitmaps and processes them for aggregate operations. Here the SIMD capabilities of the CPU can accelerate the processing of these bitmaps significantly and a copy of the WideTable stored in the main memory can be used to retrieve database records of interest. Once the aggregate operations are performed, the CPU can materialise the result to complete the query execution. }}



==> Membrane/Sections/Sys_Integration_v5.tex <==
\section{System Integration (NEW) - To be filled in.}

%\hl{
%\textbf{Interleaving} poses a problem for performing PIM on words larger than the native burst size, because neighboring bytes are in different DRAM chips. This  can be addressed in several ways. The Compute Slices could produce partial results by processing the local data available, even though these are not full words. Later, these partial results are combined to form a single representative result, but this becomes challenging for range queries. One could simply change the interleaving so that entire words are kept together, but without other changes, this makes traditional load/store inefficient, because cache-line fetch can no longer leverage the full bandwidth of the rank. Our solution is therefore to modify the address interleaving so that full words are kept together; i.e., interleaving is now at 64 bits rather than the burst width. We simply need to add a {\em De-interleaving Unit (DU)} with a cache-line-wide buffer that resides in the memory controller to assemble the cache line being read, or to feed the appropriate bytes for a read. Now a rank wide read or write fetches or writes the appropriate chunk (e.g., a byte for x8) of each word in the cache line. For example, the first read for a cache line would get the 0th byte of each word, the next read would get the 1st byte, then the 2nd byte, and so on.  In this way a cache line access takes the same amount of time.

%\textbf{PIM Pages.} PIM is only cost-effective when operating on a sufficiently large volume of data. At the same time, the design is simplified when one or more entire {\em logical rows}, interleaved across all channels, ranks, and banks, are the minimum unit of PIM operation. This ensures that the full channel-, rank-, and (for AB mode) bank-level parallelism can be utilized. This also maps well to operating system support for superpages.  

%A {\em PIM page} is therefore the \hc{enforced} minimum unit of allocation and consists of one or more native superpages, and its size will depend on the system’s configuration, so that the PIM page fills at least one entire system-wide \hc{logical?} row.  For a large memory system this will require multiple contiguous superpages, e.g., for an 8-channel, 4 ranks/channel system with DDR4\_8Gb\_x8\_2933 DRAM chip configuration taken from \cite{dramsim3}, a PIM page is 4 MByte, requiring two 2 Mbyte superpages on an x86-64 system.   For a smaller system, a single superpage will suffice, and it might occupy several logical rows.  This means that that when building a system to use Membrane memory, the memory system should configure memory channels in powers of 2.

%Using superpages allows us to allocate PIM data and schedule PIM operations, manage interleaving, and perform virtual-to-physical translation/protection at a superpage granularity, and avoid hundreds or thousands of TLB lookups per PIM page.  Note that PIM pages do not need require any particular placement in memory or relative to each other, especially for bank- and rank-level PIM.  In the case of subarray-level PIM,  for performance optimization, it is preferable to place PIM pages in or as close as possible to the subarrays with Compute Slices, to minimize LISA hops.  This suggests that, for subarray-level PIM (which we eventually show is not needed), the memory allocator would want to reserve space in the CS-enabled subarrays and its neighbors for PIM allocations. 

%\textbf{CPU - PIM Synchronization.} Each PIM command is performed at the granularity of a PIM page. During PIM processing of a page, the entire memory system is stalled. In between PIM pages, regular CPU loads/stores and I/O DMAs can proceed.  \ks{What is the latency to PIM one page in SB?} \ak{5.90 second per columnar scan in SB mode. }

%\textbf{PIM Configuration.} \hc{Is this section alluding to a memory-mapped programming model? If so, should Fig. 5 should have a logic block monitoring the PIMCONF addresses and triggering the PCG to request translations from the TLB, etc.} Aquabolt proposes a set of reserved memory addresses that can be written to, in order to configure the modes of operation for PIM execution and to specify the instructions to be executed by the PIM subsystem. These addresses can be easily accessed and configured by the Host CPU using a simple DRAM write command, allowing for simpler control of the PIM execution units. By writing into a special register, the PIM mode of execution can be toggled on or off, and instructions and operands can be specified for execution. The reserved memory space for this purpose is referred to as PIMCONF in the address space and can be accessed by userspace programs without needing to switch to kernel space every time a PIM execution is invoked, reducing overhead. We adopt a similar mechanism for Membrane. 

%\textbf{Virtual Memory.} The operating system must support a {\em pim\_malloc()} system call that allocates the desired amount of contiguous virtual address space and maps this to one or more PIM pages (note that the allocated PIM pages do not need to be contiguous in physical address space), and for subarray-level PIM, places them in or as close as possible to a Compute-Slice-enabled subarray. This means that when first loading an in-memory database for PIM, the application will allocate the memory for the database, and also for one bitmap array, using pim\_malloc(). These pages should be allocated read-only.  To differentiate between the conventional pages and PIM-capable pages, we propose a bit in the page tables and within the TLB  indicating whether a superpage is PIM-capable or not. 

%Note that we assume that the database WideTable is read-only, which avoids the need to worry about coherence between the CPU and DRAM, cache flushes, etc. Furthermore, any data read from the database in the Materialization stage cannot be modified in place by the subsequent Aggregation stage, to avoid corrupting the table.

%The bitmap produced by a Filter operation must also be cacheable, to leverage spatial locality in fetching the bitmap. The bitmap does need to be flushed at the end of a query, so that a subsequent query can write a fresh bitmap without worrying about coherence with the previous version in the cache. The bitmap is small (approx 2 MB per rank in our workload listed in section-\ref{sec:methodology} for a given \ks{Give size in MB}, and the CPU will not modify it, so flushing this does not require writebacks to memory. This means the cache flush for the bitmap can be done in parallel with the next Filter operation and the cache flush time can be completely hidden.
%}

\textbf{PIM Pages.} PIM is only cost-effective when operating on a sufficiently large volume of data. At the same time, the design is simplified when one or more entire logical rows, interleaved across all channels, ranks, and banks, are the minimum unit of PIM operation. This ensures that the full channel-, rank-, and (for AB mode) bank-level parallelism can be utilized. This also maps well to operating system support for superpages.

A PIM page is therefore the \hc{enforced} minimum unit of allocation and consists of one or more native superpages, and its size will depend on the system’s configuration, so that the PIM page fills at least one entire system-wide \hc{logical?} row.  For a large memory system this will require multiple contiguous superpages, e.g., for an 8-channel, 4 ranks/channel system with DDR4\_8Gb\_x8\_2933 DRAM chip configuration taken from \cite{dramsim3}, a PIM page is 4 MByte, requiring two 2 Mbyte superpages on an x86-64 system.   For a smaller system, a single superpage will suffice, and it might occupy several logical rows.  This means that that when building a system to use Membrane memory, the memory system should configure memory channels in powers of 2.

Using superpages allows us to allocate PIM data and schedule PIM operations, manage interleaving, and perform virtual-to-physical translation/protection at a superpage granularity, and avoid hundreds or thousands of TLB lookups per PIM page.  Note that PIM pages do not need require any particular placement in memory or relative to each other, especially for bank- and rank-level PIM.  In the case of subarray-level PIM,  for performance optimization, it is preferable to place PIM pages in or as close as possible to the subarrays with Compute Slices, to minimize LISA hops.  This suggests that, for subarray-level PIM (which we eventually show is not needed), the memory allocator would want to reserve space in the CS-enabled subarrays and its neighbors for PIM allocations.

==> Membrane/Sections/Sys_Integration_ver4.tex <==
\section{System-Level Integration}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Membrane/Sys_Int_2_Figs/04_PIM_System_Integ.pdf}
    \caption{PIM System Integration}
    \label{fig:system_integration}
\end{figure}

In integrating the different PIM architectures from the preceding section into the system, we seek to minimizes changes to the CPU and software. Several works, such as MCN, Mutlu's PEI ISCA 2015 work, and SIMDRAM, have proposed various system integration mechanisms. We also find successful real-world implementations, such as Samsung AxDIMM, Aquabolt, and UPMEM, that have integrated PIM architectures with existing systems. \ks{Need citations for all of these.} \ak{We aim to build up on the existing integration mechanisms and iterate upon them to integrate Membrane's PIM architecture with the Host system in the context of database workloads. }
%Since the primary objective of this paper is to explore query execution with PIM architectures at each level of the DRAM hierarchy, we propose to build upon existing system integration mechanisms with a conservative set of assumptions to integrate Membrane PIM architectures.

\textbf{PIM Pages.} PIM is only cost-effective when operating on a sufficiently large volume of data. At the same time, the design is simplified when one or more entire {\em logical rows}, interleaved across all channels, ranks, and banks, are the minimum unit of PIM operation. This ensures that the full channel-, rank-, and (for AB mode) bank-level parallelism can be utilized. This also maps well to operating system support for superpages.  

A {\em PIM page} is therefore the \hc{enforced} minimum unit of allocation and consists of one or more native superpages, and its size will depend on the system’s configuration, so that the PIM page fills at least one entire system-wide \hc{logical?} row.  For a large memory system this will require multiple contiguous superpages, e.g., for an 8-channel, 4 ranks/channel system with DDR4\_8Gb\_x8\_2933 DRAM chip configuration taken from \cite{dramsim3}, a PIM page is 4 MByte, requiring two 2 Mbyte superpages on an x86-64 system.   For a smaller system, a single superpage will suffice, and it might occupy several logical rows.  This means that that when building a system to use Membrane memory, the memory system should configure memory channels in powers of 2.

Using superpages allows us to allocate PIM data and schedule PIM operations, manage interleaving, and perform virtual-to-physical translation/protection at a superpage granularity, and avoid hundreds or thousands of TLB lookups per PIM page.  Note that PIM pages do not need require any particular placement in memory or relative to each other, especially for bank- and rank-level PIM.  In the case of subarray-level PIM,  for performance optimization, it is preferable to place PIM pages in or as close as possible to the subarrays with Compute Slices, to minimize LISA hops.  This suggests that, for subarray-level PIM (which we eventually show is not needed), the memory allocator would want to reserve space in the CS-enabled subarrays and its neighbors for PIM allocations. 

%, by placing the input data into a page. In single bank-mode, we can also take advantage of the rank-level parallelism available across many channels, by spreading a page in SB mode across a single bank in all available rows. If the page size does not match the page sizes supported by the host, we could pad the existing pages with zeroes and make note of the same. We have proposed PCG further down below to be used for these meta data operations.
%Since we are introducing the ability to use All-Bank mode, we suggest that the page size should be set according to the row-buffers activated across all the banks and ranks, to take advantage of the parallelism afforded by this mode.

%In AB mode, a page is again spread across all the ranks, but this time with all the available banks within a rank holding a portion of the page. We recommend that page sizes be set according to the Membrane modes (ABAR or SBAR) that are being used. The page interleaving has potential implications on other workloads, and we acknowledge the same. We envision systems utilizing Membrane PIM accelerators to be specially configured for maximum database performance.
	
\textbf{Virtual Memory.} The operating system must support a {\em pim\_malloc()} system call that allocates the desired amount of contiguous virtual address space and maps this to one or more PIM pages (note that the allocated PIM pages do not need to be contiguous in physical address space), and for subarray-level PIM, places them in or as close as possible to a Compute-Slice-enabled subarray. This means that when first loading an in-memory database for PIM, the application will allocate the memory for the database, and also for one bitmap array, using pim\_malloc(). These pages should be allocated read-only.  To differentiate between the conventional pages and PIM-capable pages, we propose a bit in the page tables and within the TLB  indicating whether a superpage is PIM-capable or not. 
%We also suggest that the data residing in PIM-capable pages be non-cacheable. This is because, if any PIM data is cached within the available cache levels, it needs to be flushed before starting a PIM operation. However, since we operate on an OLAP database that is not frequently updated, the CPU only requires the filtered data to arrive at its caches to perform the final aggregation and result materialization step. Also, making the PIM-capable pages non-cacheable relieves us of further complexity associated with flushing PIM-capable cachelines before scheduling a PIM operation.

Note that we assume that the database WideTable is read-only, which avoids the need to worry about coherence between the CPU and DRAM, cache flushes, etc. Furthermore, any data read from the database in the Materialization stage cannot be modified in place by the subsequent Aggregation stage, to avoid corrupting the table.

The bitmap produced by a Filter operation must also be cacheable, to leverage spatial locality in fetching the bitmap. The bitmap does need to be flushed at the end of a query, so that a subsequent query can write a fresh bitmap without worrying about coherence with the previous version in the cache. The bitmap is small (approx 2 MB per rank in our workload listed in section-\ref{sec:methodology} for a given \ks{Give size in MB}, and the CPU will not modify it, so flushing this does not require writebacks to memory. This means the cache flush for the bitmap can be done in parallel with the next Filter operation and the cache flush time can be completely hidden.


\textbf{PIM Command Generator (PCG) Unit.} \hc{Add table with PCG ISA spec: pim\_malloc(), pim\_filter(), pim\_write(), pim\_free()...} The PCG unit is analogous to Intel's Data Streaming Accelerator and Analytics Accelerator \cite{intel-iaa}.  It offloads the PIM orchestration from the CPU and also coordinates the PIM operations across memory controllers and channels. The operating system must support a {\em pim\_filter()} command that has the arguments to provide the context for a columnar scan on the PIM memory. Specifically it requires the start and end addresses of the column to be scanned, the number of elements, the values to compare against and comparison operation to perform on the elements of a column (less than/equality/not equal to) as arguments of the pim\_filter() call.The OS can parse this function call and offload the operation to the PCG. Note that the Intel DSA provides user-level drivers to ensure that userspace programs can invoke the hardware without expensive context switch to kernel space. And since, we propose the PCG too along the DSA lines, we aim to avoid these overheads simlarly.  


% has multiple purposes depending on the Membrane architecture used. At the subarray level, the PCG is involved in orchestrating the LISA mechanism. To perform the LISA hops, it requires the physical address of the source row in order to map data and issue the necessary commands. Therefore, the PCG unit is designed to calculate the subarray row's location based on the physical memory address decoded from the TLB, and introduce a series of LISA hop commands into the memory controller to transfer the data into the Compute Slice.

In addition to its role in the LISA mechanism, the PCG provides a useful abstraction for the CPU to offload PIM execution and orchestration. The Host CPU operates on the virtual address space, unaware of the physical location of the input data. However, metadata such as the physical location, page size, and offsets are necessary for managing and scheduling PIM operations. For this reason, the PCG has access to the Translation Lookaside Buffer (TLB) to perform address translations.

%%ak{AK - Note sure about including this following para}
%We proposed the PCG based on Intel's DSA (Data Streaming Accelerator), which primarily issues a series of memory commands to relieve the CPU of trivial data copying and minor processing operations (such as CRC, fill, and memcpy). Intel Analytics Accelerator (IAA) is built on top of DSA to execute database filtering operations, which Membrane aims to perform within the memory, rather than accessing the data across the memory bus. A key difference between Intel's DSA (or IAA) and PCG is that the former operates on virtual addresses while the latter operates on physical addresses.

\textbf{CPU - PIM Synchronization.} Each PIM command is performed at the granularity of a PIM page. During PIM processing of a page, the entire memory system is stalled. In between PIM pages, regular CPU loads/stores and I/O DMAs can proceed.  \ks{What is the latency to PIM one page in SB?} \ak{5.90 second per columnar scan in SB mode. }

%In our proposed system integration scheme, we suggest that while the PIM operations are ongoing, any access to the DRAM memory system must be blocked. This is necessary because regardless of whether Membrane is operating in SBAR or ABAR mode, all the ranks are utilized in parallel to accelerate the scan kernel. Consequently, any CPU access must be blocked until the PIM commands are completed. This could potentially affect other applications, so we recommend that any system adopting Membrane should be optimized for database-specific workloads. In our evaluations, PIM operations for executing a query lasted for less than 10 ms under an 8-channel configuration operating on scale factor-100 datasets.

\textbf{PIM Configuration.} \hc{Is this section alluding to a memory-mapped programming model? If so, should Fig. 5 should have a logic block monitoring the PIMCONF addresses and triggering the PCG to request translations from the TLB, etc.} Aquabolt proposes a set of reserved memory addresses that can be written to, in order to configure the modes of operation for PIM execution and to specify the instructions to be executed by the PIM subsystem. These addresses can be easily accessed and configured by the Host CPU using a simple DRAM write command, allowing for simpler control of the PIM execution units. By writing into a special register, the PIM mode of execution can be toggled on or off, and instructions and operands can be specified for execution. The reserved memory space for this purpose is referred to as PIMCONF in the address space and can be accessed by userspace programs without needing to switch to kernel space every time a PIM execution is invoked, reducing overhead. We adopt a similar mechanism for Membrane. 

==> Membrane/Sections/System.tex <==
% system integration %

% System integration pending which modes of operation we choose to showcase.
% 1- Membrane + CPU
% 2- Membrane + Main memory + CPU (Membrane and memory interact via CPU)
% 3- Membrane-Main memory (via DMA) + CPU

% Two levels of abstraction used for system integration in any case:
% a) CAM ISA: exposed to DBMS designer to utilize PIM operations (i.e., selection, aggregation), unaware of microarchitectural details (it works for both Fulcrum and Sieve).
% b) DRAM++ microcode: microarchitecture specific commands, different for Sieve and Fulcrum.

% More details:
% CAM ISA: Is composed of three types of instructions (include table): 
%     - predicates: equality, inequality predicates: they broadcast predicate values to subarrays/PIM PEs (Sieve/Fulcrum), execute predicate, retrieve masks into special buffer inside the memory controller.
%     - (pre)aggregations, (pre)sorting: coarsely prepare data for a finer-grain CPU processing.
%     - configuration: helps generate sequences of addresses for subsequent commands.
    
% DRAM++ microcode: It can be produced at different levels of the microarchitecture. For now let's assume it's generated by the memory controller. 
% CAM ISA Configuration instructions- Two options:
% 1) unstructured layout: configuration instructions set: start address, data type (i.e., bytewidth), column length (record ID count). Subsequent predicate instructions are applied to all addresses within range: [start_addr:start_addr+bytewidth*length-1].
% 2) RISC-V vector-like layout: use standard configuration RISC-V instructions (vsetvl, vsetvli) and vector register name abstractions to map PIM locations to database columns. For example, vector register v1 stores d_year, so v1_start_addr, Control Status Registers (CSRs) v1_type, v1_vl contain the start address, data type (uint32_t or whatever compressed value needed), and size of d_year's size (6M in SF1) as vector length. Another way to do this which makes it more efficient is to group columns with the same length/type share CSRs. However, start addresses still need to be stored separately by vector register name. This is similar to traditional virtualization, we may need a virtual page table and TLB-like structure if it is too complex.

% In order for 2) to work, we would need to be able to:
% 1- set configuration flag to say that vector instructions now refer to MemBrain
% 2- vlw.v (loads) now refer to moving data from DRAM to DRAMPIM in the appropriate layout (V or H)
% 3- express predicates using RISC-V vector instructions (like Castle)- done.
% Challenge: each DB column may have different bitwidths and needs to be layed out very carefully for each microarchitecture. How do we express irregularity- can we group the layout of columns in at most 4-8 categories (rather than 15)?

%\vspace*{-0.1in}
\section{System Integration} \label{sec:system integration}
%\vspace*{-0.05in}
%Membrane's system integration consists of two levels of abstraction. First, we create a small set of Membrane-specific ISA instructions to expose the PIM functionalities that can be expressed by a DBMS developer. Second, we add logic in the DRAM controller to further decompose these new ISA instructions into DRAM commands specific to each Membrane (V/H) architecture. 

Membrane's system integration consists of two levels of abstraction. First, a small set of Membrane-specific ISA instructions expose the PIM functionalities that can be used by a programmer. Second, logic in the DRAM controller is used to further decompose these new ISA instructions to DRAM-specific commands for each Membrane (V/H) architecture. 

\textbf{Membrane ISA.}
There are three main types of Membrane ISA instructions: \emph{predicate}, \emph{data movement}, and \emph{configuration} instructions. Predicate instructions include equality and inequality flavors and take the comparand value, the type of predicate (e.g., equal, not equal, less than or equal, greater than or equal, between, etc.), and the target column to which to apply the predicate. Data movement instructions are typically used offline by the DBMS to orchestrate loading the WideTable into the PIM. (Since generating the WideTable is considered a fixed cost that is paid once, we decided not to add dedicated hardware to accelerate it.)

In order to maintain a reasonably user-friendly interface of the Membrane ISA instructions and to keep the instructions' encoding lightweight, we added eight column-operand names $c_0-c_7$ that can be utilized by the PIM instructions.\footnote{When a query operates on more than 8 columns, the query is divided into multiple sub-queries, each with at most 8 columns, and executed separately.} Similar to existing vector-length agnostic ISAs which maintain the state of their vector register names using Control Status Registers~\cite{waterman14}, we augment the DRAM controller with bookkeeping logic to keep track of the start address, size, layout, and bitwidth of each column operand. Then, data movement and predicate instructions addressing a specific column operand will read these data structures to generate addresses for the required DRAM commands. 

The way that a DBMS would utilize the Membrane instructions is as follows. 1) Use configuration instructions to map database columns used in the query to column names: $c_0-c_7$. 2) Use data movement instructions to load the WideTable columns into Membrane. 3) Call Membrane predicate instructions as part of the query execution to execute the selection operators in Membrane. For example, suppose we want to filter on d\_year and return lo\_date. We would set d\_year’s length, bitwidth, data layout, start address with a configuration instruction and map it to c\_0, and do the same with lo\_date and map it to c\_1.  Finally, we would execute a predicate instruction on c\_0 and project the masks on c\_1. %\ks{Added this example for clarity but we can cut  it if needed for space.}

\sout{\textbf{PIM-CPU Data Transfer.}
The output of a predicate instruction is a vector of bits for the Bitmask Mode (or values for the Data Push Mode). To support that, the DRAM controller includes one 64B buffer per memory channel to cache the output bitmask and an additional 2KB FIFO to cache the values for Data Push Mode.\footnote{2KB because a 64B fully-dense mask can potentially retrieve 64*8=512 values. The worst case value bitwidth is 32 bits.} These buffers enable a decoupled mode of execution where subblocks of the output vector are produced by the PIM while subblocks buffered in the memory controller are being fetched by the CPU.} 

\sout{These buffers are sufficient to decouple the CPU and PIM without stalls. In the data push mode, the amount of data being pushed to the CPU is  dependent on the selectivity of the query being executed, with more data being pushed for queries that exhibit high selectivity. In our analysis, the largest volume of data transferred in the SSB query suite was for query 3.1, with 152 MB of dictionary-encoded data values traveling across the memory bus. This equates to around 0.0004\% of the DRAM bandwidth, %\sout{so the memory interface is not longer a bottleneck} 
hence, the memory interface is observed to not experience any bottlenecks in our evaluations.
In bitmask mode, processing the bitmask overlaps with data retrieval from the memory locations. }

%\sout{ data retrieval from the DRAM memory location takes significantly longer  than processing the bitmask. }
%\ak{AK: can we replace the final the final part of the last sentence with - where the latter takes signficantly longer than the former.}
%In both modes, we observed that the memory controller has negligible overhead when compared to the overall query execution time. 

%\ak{The system integration of the PIM memory with the Host plays an important role in driving the architecture, usage and performance cherctarstics of the design. There is a need to make PIM-capable memory be compatible with the existing Host architecture without significantly modifying it while at the same time extending it to support the enhanced PIM-memory. Hence, many of the changes proposed were motivated by the desire to strike a fine balance between compatibility and extending the capabilities. The system integration is different for each variant of Membrane since their modes of operation differ significantly. }

%\ak{Membrane-V - This mode primarily operates on late materialisation philosophy where bitmaps for all the database records scanned are collected and processed in the final stage to materialize the result. Hence, collecting and transferring these bitmaps to the CPU is the main task of the system integration. Afer performing a scan operation, bitmaps are produced on a per-attribute basis. Hence, the memory controller directs the PIM memory to store each bitmap in certain reserved addresses or pages after each attribute scan operation. Once all the scans are completed, the CPU reads these bitmaps from the reserved addresses and processes them further to materialise the result. Modern operating systems and hardware utilise similar mechanism to reserve certain address spaces for various reasons such as debugging drivers, privelage sepration, memory mapping etc. Prior works such as Damon have also utilised this in the PIM context. }

%\ak{Membrane-H - In the V variant the scanning and retrieving bitmap operations are entirely driven and dictated by the CPU but the same may not hold true for the H variant where data that is filtered out needs to be "pushed" from the PIM memory rather than being read out or "pulled" from the CPU. Thus, there are significant changes that need to be introduced into the H variant to account for this. Direct Cache Approach where CPU consumes the data injected by the Network Card directly into caches is a motivation to our sytem design for this variant. DCA is a well studied and mechanism with extensive optimisations and implementations already available that one could leverage with minor modifications to extend it to support PIM capabilities. Another interesting direction was investigated in Memory Channel Networks [TODO citation] that again aimed at utilising a variant of DCA approach to enable Rank-level PIM processing. It treats each rank or DIMM to be a separate node with its own network addresses to communicate with except that the PHY layer consists of DDR interface rather than the conventional ethernet interface. Although this provides several valuable advantages especially related to offloading applications majorly written for distributed computing domain, we optimise the design to reflect our focus on the OLAP database workload. }

%\ak{Generally the memory is organised into several channels, DIMMs and ranks. While the channels are independent and can be accessed parallely, the DIMM and ranks within each channel share the same data and address buses and hence need to be accesssed in a concurrent manner. Our key idea here is that while the memory controller performs an access on a certain DIMM/rank, the next cacheline of data can be kept ready by the RLP/subarray units by performing a SCAN and Gather operation in another DIMM/rank. By performing this pipelining of operations between several ranks and DIMMs, the memory controller is always kept busy and at the same time hiding the latency related to the SCAN and Gather operations performed by the RLP and subarray-level PIM elements.}

%\ak{The memory controller after reading the cacheline worth of data usually transfers it to the CPU via a DMA engine by updating the TX descriptor. [AK - TODO] Need some elaboration here about the RX / TX rings }

%\textcolor{blue}{
\sout{\textbf{FIFO Buffer Synchronization.}
%The HW
The FIFO buffers adopt a latency-insensitive interface with the use of \emph{ready} and \emph{valid} bits: when the memory controller has filled up the buffer with data, it sets the valid bit to 1; and when the CPU has consumed the data, it sets the ready bit to 1 to let the memory controller know that it is ready to consume the next value. To enable the data push mode, there is also the \emph{done} bit, set by the memory controller to indicate when there is no more data to be consumed by the CPU.}
%The SW (or how do we expose the interface to the SW)
\sout{To expose this latency-insensitive mechanism to the CPU, the program uses Membrane-buffer specific load instructions to read data from the buffers. In Bitmask Mode, the CPU can read a bit as long as the valid bit is set. In Data Push Mode, since the number of values to be read depends on the selectivity of the predicate, the CPU will continue reading values (if the valid bit is set and) until the done bit is set. To read or set the ready/valid/done bits, the CPU reads or modifies memory-mapped registers using regular loads and stores. This is similar to the approach in \cite{dca}, which is widely used, except that we utilize a FIFO buffer and register bits to synchronize instead of interrupts and read/writes to the cache.} 
%}
 
%FIFO buffers need to be addressable, memory controller sets valid bit every cacheline size block is loaded into buffers, CPU unsets the bit when it has consumed it. To enable this sync, the code looks like a for-loop containing a filter instruction, a fence instruction, and the aggregation operator body.
%The buffers adopt a latency-insensitive interface with the use of \emph{ready} and \emph{valid} bits: when the memory controller has filled up the buffer with data, it sets the valid bit to 1; and when the CPU has consumed all the data, it sets the ready bit to 1 to let the memory controller know that it can refill the buffer with fresh data. %(helena: This can be suboptimal because if read/valid bits work at the granularity of buffer size, then Membrane cannot start filling up the buffers until the CPU has consumed the whole 64B/2kB buffer data. Instead, we know that the CPU will consume this data using SSE instructions that work at 128-bit granularity. To leverage that, we can change the meaning of the valid/ready bits to valid 1 means there is at least one bit/record and instead of a ready bit having a counter that the CPU updates to let Membrane know how many records it has consumed.)

%helena: I think paragraphs 1 and 2 of this section already explain this:
%The DRAM controller translates Membrane ISA instructions into sequences of DRAM-specific commands. The controller for Membrane-V will break down predicate instructions into DRAM commands to broadcast the comparand, read-and-compare commands, and mask writes into the subarray and dedicated buffer. Membrane-H will transform the predicate instructions into subarray reads, ALU-like instructions %as shown in Table-\ref{tab:instruction buffer format}%, 
%and writes of the output. Note that both microarchitectures utilize the dedicated bookkeeping structures in the memory controller to generate the appropriate addresses at each command. Membrane load and store instructions will work similarly to traditional loads and stores, with the added column operand state, which will be read to move the data in the expected layout.

%helena: this is too much information and it does not relate to reviewers' concerns?:
%\ak{During query execution, the memory controller issues a series of read commands to process elements at the subarray level. In the bitmask-mode, we use a setup similar to \cite{jaffar} where the partial bitmasks are flushed and written to pre-determined memory locations periodically. The memory controller can later retrieve this information and send it to the CPU. In the data-push mode, every time an element evaluates to true, Membrane-H can pull \textcolor{red}{pull --$>$ set?} the \textit{push\_data\_h} (see~\ref{membrane-H control unit}) signal high to indicate to the memory controller to retrieve the data from the subarray via the global data lines and send it to the CPU \textcolor{red}{Not clear who does the send -- the memory controller?}. If the data element does not pass the selection predicate \textcolor{red}{check this sentence carefully}, no changes are made to the signal and the memory controller issues the next successive read command to iterate over the next columnar data. For Membrane-V, the memory controller needs to carry out an extra step of reading the bitmap generated and retrieving the data from the main memory before pushing it to the CPU. }

\ak{\textbf{PIM-CPU Data Transfer.}
The system integration of the PIM memory with the Host plays a key role in driving the architecture, usage, and performance characteristics of the design. There is a need to make PIM-capable memory compatible with the existing Host architecture without significantly modifying it while at the same time extending it to support the enhanced PIM-memory. Hence, many of the changes proposed were motivated by the desire to strike a fine balance between compatibility and extending the capabilities. The system integration is different for each variant of Membrane since their modes of operation differ significantly. }

\ak{\textbf{Membrane-V.} - This mode primarily operates on late materialization philosophy where bitmaps for all the database records scanned are collected and processed in the final stage to materialize the result. Hence, collecting and transferring these bitmaps to the CPU is the main task of the system integration. After performing a scan operation, bitmaps are produced on a per-attribute basis. Hence, the memory controller directs the PIM memory to store each bitmap in certain reserved addresses or pages after each attribute scan operation. Once all the scans are completed, the CPU reads these bitmaps from the reserved addresses and processes them further to materialize the result. Modern operating systems and hardware utilize similar mechanisms to reserve certain address spaces for several reasons such as debugging drivers, privilege separation, memory mapping etc. Prior works such as \cite{jaffar} have also utilized this in the PIM context. }

\ak{\textbf{Membrane-H.} - While in V variant, the scanning and retrieving bitmap operations were entirely driven and dictated by CPU, the same may not hold true for the H variant where data that is filtered  after SCAN operation needs to be "pushed" from the PIM memory rather than being read out or "pulled" from CPU. Thus, there are significant changes that need to be introduced into the H variant to account for this. DCA or Direct Cache Access refers to the mechanism of inserting data directly into the cache by the IO devices such as network interface cards (NICs), from where the CPU reads it for further processing. DCA has been widely implemented by major vendors over the past years with various names such as Intel DDIO \cite{ddio} and Cache Stashing by Arm \cite{arm-cache-stashing}. Several works such as (TODO - citations required) have studied the effects and optimization techniques related DCA to seamlessly integrate it with the OS stack to get better performance. These mechanisms can be leveraged in the PIM context for pushing the data from the Membrane-H DIMM to the CPU. Memory Channel Networks (MCN) \cite{mcn-dimm} proposes changes to network subsystem to achieve this where DIMMs on a memory channel appear as independent nodes connected with an ethernet link except instead of ethernet PHY interface, it is the DDR interface. This has several benefits as minor modifications to the overall architecture are required to support transparent offloading of computation and retrieval of data from these PIM-capable DIMMs. Our system integration employs a similar mechanism to receive data from the RLP processor and insert it into the CPU caches for further processing. Furthermore, since the Memory Controller (MC) sends data in periodic intervals from PIM memory into the CPU caches, we could hide any overhead latencies incurred by the mechanism by simulatenously receiving next cacheline of data while buffering and transmitting the previous cacheline in a pipelined fashion.}

==> Membrane/Sections/scratch_intro.tex <==
\section{INTRODUCTION}
\begin{INTRODUCTION}
Database Management Systems are software systems that enables users to define, create, maintain and control access to the database. These database tend to hold large quantities of data which leads to DBMS becoming ever more complex and support various features. Database as a discipline has been studied extensively over several decades and has been optimised to always provide the highest performance possible. By some estimates, database workloads tend to be one of the two most important and extensively used workloads in the datacentre industry apart from Machine Learning. Hence, due to its widespread usage, accelerating database workloads provides tremendous benefits both in terms of increasing revenue to the cloud customers and also reducing the execution times for the end-users. 

Due to the slowing down of the Moore's Law and the impact of memory wall, moving vast amounts of data between the memory and processor tends to be expensive, both in terms of time and energy which always eats into the performance. {citation needed} shows that the cost of moving the data is several orders of magnitude higher than the cost of computation itself. Thus, cutting down the expensive data movements would yield immense benefits both in terms of performance and reduced energy consumption. 

Processing-in-Memory or Near Data Architectures have turned out to one of the possible solutions to overcome the effects of this Von Neumann bottleneck. They involve providing compute capability to the memory itself or placing compute elements as close to the memory as possible. Several such architectures { citation needed } have been proposed that could be utilized to accelerate and process a wide array of kernels. However, our work primarily focuses on accelerating database workloads precisely and looking at the end to end query processing pipeline. Our key insights that inspired our work are elaborated in the succeeding paragraphs. 

Firstly, DRAM is becoming an ubiquitous device which has several useful characteristics such as speed, capacity and its proven performance. The cost of DRAM is also continuously decreasing, while the capacity tends to increase with each succeeding generation. Hence, the database workloads have taken advantage of these characteristics and moved away from the disk-based database systems to in-memory-based database systems. Hence, from a performance perspective, DRAM is a very strong contender that offers several advantages when compared to Flash or disk-based systems. 

Secondly, processing-in-memory architectures offers immense parallelism and bandwidth. These can be very useful in overcoming effects of Von Neumann bottleneck. Placing compute elements closer to the data also helps in ensuring the expensive costs such as energy and time associated with moving massive amounts of data between the memory and CPU. 

Thirdly, although several previous works { citation needed}, have proposed Processing-In-Memory architectures to solve a variety of workloads, { To PIM or not to PIM } indicates that Database workloads in particular are one of the best placed workloads that is designed to take maximum advantage of the benefits offered by the Processing In Memory Architecture. This is because although Processing-In-Memory offers massive bandwidth and parallelism, not every workload is designed to derive maximum benefit of such features. This is because of the nature of the kernels and the algorithms that implement the execution of these kernels. Some workloads tend to be memory bound and some compute bound. Although, it is intuitive to observe that all memory-bound workloads tend to favour PIM architectures, previous studies {citation needed} have indicated that random memory accesses of a workload can degrade the performance of PIM architectures immensely. Also, due to the light weight nature of the compute elements placed within the PIM architecture, the workloads need to have a lower computational intensity per memory access to win over the CPUs. Thus, any workload with lower computational intensity and non-random memory access patterns naturally favour the PIM architecture generally. Database applications exhibit these characteristics thereby enabling a PIM architecture to accelerate this application massively. 

Fourthly, with several advancements and optimizations studied over decades of research in accelerating database applications, we draw upon a large body of previously researched ideas and revisit them in the context of the Processing in Memory to suitably adapt the workload to the architecture's strong suites. We have drawn ideas from WideTable paper published in 2014 and Data Morphing paper published in 2002 which bear immense significance on this work and thereby reinforcing the need for revisiting certain fundamental assumptions and old ideas in light of the slowing down of Moore's Law. 
\end{INTRODUCTION}
